Two-Commodity Flow is Equivalent to Linear Programming under Nearly-Linear Time Reductions

We give a nearly-linear time reduction that encodes any linear program as a 2-commodity flow problem with only a small blow-up in size. Under mild assumptions similar to those employed by modern fast solvers for linear programs, our reduction causes only a polylogarithmic multiplicative increase in the size of the program and runs in nearly-linear time. Our reduction applies to high-accuracy approximation algorithms and exact algorithms. Given an approximate solution to the 2-commodity flow problem, we can extract a solution to the linear program in linear time with only a polynomial factor increase in the error. This implies that any algorithm that solves the 2-commodity flow problem can solve linear programs in essentially the same time. Given a directed graph with edge capacities and two source-sink pairs, the goal of the 2-commodity flow problem is to maximize the sum of the flows routed between the two source-sink pairs subject to edge capacities and flow conservation. A 2-commodity flow can be directly written as a linear program, and thus we establish a nearly-tight equivalence between these two classes of problems. Our proof follows the outline of Itai's polynomial-time reduction of a linear program to a 2-commodity flow problem (JACM'78). Itai's reduction shows that exactly solving 2-commodity flow and exactly solving linear programming are polynomial-time equivalent. We improve Itai's reduction to nearly preserve the problem representation size in each step. In addition, we establish an error bound for approximately solving each intermediate problem in the reduction, and show that the accumulated error is polynomially bounded. We remark that our reduction does not run in strongly polynomial time and that it is open whether 2-commodity flow and linear programming are equivalent in strongly polynomial time.

==> proofs.tex <==
%!TEX root = main.tex



\section{Proof details}
\label{sect: proof}
The chain of reductions from \textsc{lp(a)} to \textsc{2cf(a)} consists of nine steps.
In each step, we analyze the reduction from some problem A to some problem B in both the exact case and the approximate case.
In the exact case, we start with describing a nearly-linear-time method of reducing A to B, and a nearly-linear-time method of mapping a solution of B back to a solution of A. Then, we prove the correctness of the reduction method in the forward direction, that is if A has a solution then B has a solution. 
In addition, we provide a fine-grained analysis of the size of B given the size of A.
 
In the approximate case, we formally define approximately solving
each problem in
the first place, specifying bounds on various different types of error.
We always use the same reduction method from problem A to problem B in the
exact and approximate cases.
Thus the conclusion that problem B has a feasible solution when
problem A has a feasible solution also applies in the approximate
case.

We also always use a solution map back for the approximate case that
agrees with the exact case when there is no error. 
Crucially, we conduct an error analysis. That is given an approximate solution to B and its error parameters (by abusing notations, we use $\epsilon^B$ to denote), we map it back to an approximate solution to A and measure its error $\tau^A$ with respect to $\epsilon^B$. In other words, we can reduce an approximate version of A with error parameters $\epsilon^A\geq \tau^A$ to an approximate version of B with error parameters $\epsilon^B$. 
Note that the correctness of the reduction method in the backward
direction for the exact case follows from the approximate case analysis by setting all error parameters to zero, which completes the proof of correctness.







%reduction method from and the solution , and then state a lemma, which indicates such a reduction approach can reduce a problem instance to an instance of its following problem in (nearly-)linear time with the problem size increased polynomially. Moreover, if we set the problem error of the latter instance properly, then a solution of the latter instance can be mapped back to a solution of the former instance in linear time.
%
%The proof of each subsection is divided into two parts. In the first part, we track the change of problem size and estimate the reduction time. In the second part, we describe the method of solution mapping and estimate the solution mapping time, and then track the change of problem error. We use letter $\epsilon$ to denote the error target set in the instance, and use letter $\tau$ to denote the error that we can achieve by mapping the solution back. It is a valid solution mapping if we can show that, for the former instance, the error that we achieve is less than the error target.
%The chain of reductions from \textsc{lp(a)} to \textsc{2cf(a)} consists of nine steps.
%In each step, we start with describing the reduction approach, and then state a lemma, which indicates such a reduction approach can reduce a problem instance to an instance of its following problem in (nearly-)linear time with the problem size increased polynomially. Moreover, if we set the problem error of the latter instance properly, then a solution of the latter instance can be mapped back to a solution of the former instance in linear time.
%
%The proof of each subsection is divided into two parts. In the first part, we track the change of problem size and estimate the reduction time. In the second part, we describe the method of solution mapping and estimate the solution mapping time, and then track the change of problem error. We use letter $\epsilon$ to denote the error target set in the instance, and use letter $\tau$ to denote the error that we can achieve by mapping the solution back. It is a valid solution mapping if we can show that, for the former instance, the error that we achieve is less than the error target.

%\ming{check reduction time and solution mapping time}

\subsection{LP(A) to LEN(A)}
\label{sect: lpa-lena}
\subsubsection{LP to LEN}
We show the reduction from an \textsc{lp} instance $(\AA,\bb,\cc,K,R)$
to an \textsc{len} instance $(\AAtil,\bbtil,\Rtil)$.
% $(\AA, \bb, \cc, K, R, \eps^{lp})$
% to an LENA instance $(\AAtil, \bbtil, \Rtil, \eps^{le})$.
% Given an LP instance 
The \textsc{lp} instance has the following form:
\begin{equation}
	\label{eq: lp}
	\begin{aligned}
		\cc^\top\xx\geq K\\
		\AA\xx\leq\bb\\
		\xx\geq\boldsymbol{0}\\
	\end{aligned}
\end{equation}
% where $\AA\in\Z^{m\times n}, \bb\in \Z^m, \cc\in \Z^n$, and $K\in \Z$,
To reduce it to an \textsc{len} instance,
% it can be reduced to an LEN instance by 
we introduce slack variables $\alpha$ and $\ss$:
\begin{equation}
	\label{eq: len}
	\begin{aligned}
		\begin{pmatrix}
			\cc^\top&\boldsymbol{0}&-1\\
			\AA&\II&\boldsymbol{0}
		\end{pmatrix}\begin{pmatrix}
			\xx\\
			\ss\\
			\alpha
		\end{pmatrix}&=\begin{pmatrix}
			K\\
			\bb
		\end{pmatrix}\\
		\begin{pmatrix}
			\xx\\
			\ss\\
			\alpha
		\end{pmatrix}&\geq\boldsymbol{0}
	\end{aligned}
\end{equation}
Setting
\[\tilde{\AA}=\begin{pmatrix}
	\cc^\top&\boldsymbol{0}&-1\\
	\AA&\II&\boldsymbol{0}
\end{pmatrix}, \qquad \tilde{\xx}=\begin{pmatrix}
	\xx\\
	\ss\\
	\alpha
\end{pmatrix},\qquad \tilde{\bb}=\begin{pmatrix}
	K\\
	\bb
\end{pmatrix},\]
% then the LP is reduced to an LEN $\tilde{\AA}\tilde{\xx}=\tilde{\bb}$. 
we get an \textsc{len} instance $(\AAtil, \bbtil, \Rtil)$
where $\Rtil = \max\{1, \max\{ \norm{\xxtil}_1: \AAtil \xxtil = \bbtil, \xxtil \ge \bf{0} \}\}$.
% $\tilde{\AA}\tilde{\xx}=\tilde{\bb}$.

If an \textsc{len} solver returns $\xxtil = (\xx^\top, \ss^\top, \alpha)^\top$ for the \textsc{len} instance $(\AAtil, \bbtil, \Rtil)$, 
then we return $\xx$ for the \textsc{lp} instance $(\AA, \bb, \cc, K,R)$;
if the \textsc{len} solver returns ``infeasible'' for the \textsc{len} instance, 
then we return ``infeasible'' for the \textsc{lp} instance.

% If we are given a solution $\xxtil = $ to LEN $(\AAtil, \bbtil, \Rtil)$
% LP $(\AA, \bb, \cc, K,R)$, 
% then 


\begin{lemma}[\textsc{lp} to \textsc{len}]
	\label{lm: lp-len}
	% Reducing from an LP instance $(\AA,\bb,\cc,K,R)$ to an LEN instance $(\AAtil, \bbtil, \tilde{R})$ can be performed in time $O(\nnz(\AAtil))$.
	Given an \textsc{lp} instance $(\AA,\bb,\cc,K, R)$ where $\AA\in\Z^{m\times n}, \bb \in \mathbb{Z}^m, \cc \in \mathbb{Z}^n, K \in \mathbb{Z}$, we can construct, in $O(\nnz(\AA))$ time, an \textsc{len} instance $(\tilde{\AA},\tilde{\bb}, \tilde{R})$ 
	where $\tilde{\AA}\in \Z^{\tilde{m}\times\tilde{n}}, \bbtil \in \mathbb{Z}^{\tilde{m}}$ 
	such that 
	\[\tilde{n}= n+m+1,~~\tilde{m}=m+1,~~\nnz(\tilde{\AA})\leq 4\nnz(\AA),\]
	\[
	% \tilde{R}= 5(m+n)RX(\AA,\bb,\cc,K),~~
	\tilde{R}= 5mRX(\AA,\bb,\cc,K),~~
        X(\tilde{\AA},\tilde{\bb})=X(\AA,\bb,\cc,K)\geq 1, \]
        and if the \textsc{lp} instance has a solution, then the \textsc{len} instance
        has a solution.
    %     Furthermore, if $\tilde{\xx}$ is a solution to the LEN instance, 
	% then in time $O(n)$, we can compute a solution $\xx$ to the LP instance.
%	Given an LP instance $(\AA,\bb,\cc,K,R)$, we can reduce it to an LEN instance $(\AAtil, \bbtil, \tilde{R})$
%	in time $O(\nnz(\AAtil))$ such that a solution to LEN $(\AAtil, \bbtil, \tilde{R})$ can be 
%	mapped back to a solution to LP $(\AA,\bb,\cc,K,R)$ in time $O(n)$, where $n$ is the number of variables in 
%	the LP $(\AA,\bb,\cc,K,R)$.
\end{lemma}	
\begin{proof}
	\ming{is it ok to prove in this order?}\peng{I think this is the right order}
	Based on the reduction method described above, if $\xx$ is a solution to the \textsc{lp} instance as shown in Eq. \eqref{eq: lp}, 
	we can derive a solution $\xxtil=(\xx^\top, \ss^\top, \alpha)^\top$ to the \textsc{len} instance as shown in Eq. \eqref{eq: len}, by setting
	\[\ss=\bb-\AA\xx, \qquad \alpha = \cc^\top\xx-K.\]
	Thus, if the \textsc{lp} instance has a solution, then the \textsc{len} instance
	has a solution.
	\ming{remove comments if we want the other direction}
%	In the other direction, if $\xxtil=(\xx^\top, \ss^\top, \alpha)^\top$ solves the \textsc{len} instance as shown in Eq. \eqref{eq: len}, then $\xx$ solves the \textsc{lp} instance Eq. \eqref{eq: lp}. 

	Given the size of the \textsc{lp} instance with $n$ variables, $m$ linear constraints, and $\nnz(\AA)$ nonzero entries, we observe the size of the reduced \textsc{len} instance as following:
	\begin{enumerate}
		\item $\tilde{n}$ variables, where
		\[\tilde{n}=n+m+1.\]
		\item $\tilde{m}$ linear constraints, where
		\[\tilde{m}=m+1.\]
		\item $\nnz(\tilde{\AA})$ nonzeros, where
		\begin{equation}
			\label{eq: len-R}
			\nnz(\tilde{\AA})=\nnz(\AA)+\nnz(\cc)+m+1\leq 4\nnz(\AA),
		\end{equation}
		where we use $\nnz(\AA)\geq m,n\geq 1$, and $\nnz(\cc)\leq n$.
		\item $\tilde{R} = \max\{1, \max\{\norm{\tilde{\xx}}_1: \AAtil \xxtil = \bbtil, \xxtil \ge \bf{0} \} \}$, the radius of polytope in $\ell_1$ norm.
		Our goal is to upper bound $\norm{\xxtil}_1$ for every feasible solution to the \textsc{len} instance.
		By definition and the triangle inequality, 
		$$\norm{\tilde{\xx}}_1 =\norm{\xx}_1+\alpha+\norm{\ss}_1.$$
		Note $\norm{\xx}_1 \le R$, the polytope radius in the \textsc{lp} instance.
		% The bound of each variable $\xx(j)$ in \textsc{lp} equals to that of itself in \textsc{len}. In addition, we have 
		% \[\alpha=
		% \cc^\top\xx-K\leq \norm{\cc}_1\norm{\xx}_1+|K|\leq n\norm{\cc}_{max}R+|K|,\]
		In addition,
		\[\alpha=
		\cc^\top\xx-K\leq \norm{\cc}_{max}\norm{\xx}_1+|K|\leq \norm{\cc}_{max}R+|K|,\]
		and
		\[\norm{\ss}_1= \norm{\AA\xx-\bb}_1\leq \norm{\AA\xx}_1+\norm{\bb}_1\leq m\norm{\AA}_{max}\norm{\xx}_1+\norm{\bb}_{1}\leq m(\norm{\AA}_{max}R+\norm{\bb}_{max}).\]
		Therefore, we have
		\begin{align*}
			\norm{\tilde{\xx}}_1
			% &=\norm{\xx}_1+\alpha+\norm{\ss}_1\\
			&\leq R+|K|+\norm{\cc}_{max}R+m(\norm{\AA}_{max}R+\norm{\bb}_{max})\\
			&\leq mR(1+|K|+\norm{\cc}_{max}+\norm{\AA}_{max}+\norm{\bb}_{max}) && \text{Because $R\geq 1$}\\
			&\leq 5mRX(\AA,\bb,\cc,K). 
		\end{align*}
		% \begin{align*}
		% 	\norm{\tilde{\xx}}_1&=\norm{\xx}_1+\alpha+\norm{\ss}_1\\
		% 	&\leq R+|K|+n\norm{\cc}_{max}R+m(\norm{\AA}_{max}R+\norm{\bb}_{max})\\
		% 	&\leq (m+n)R(1+|K|+\norm{\cc}_{max}+\norm{\AA}_{max}+\norm{\bb}_{max}) && \text{Because $R\geq 1$}\\
		% 	&\leq 5(m+n)RX(\AA,\bb,\cc,K). 
		% \end{align*}
		Hence, it suffices to set
		% \[\tilde{R}=5(m+n)RX(\AA,\bb,\cc,K). \]
		\[\tilde{R}=5mRX(\AA,\bb,\cc,K). \]
		\item $X(\tilde{\AA},\tilde{\bb})=X(\AA,\bb,\cc,K)$ because \[\norm{\tilde{\AA}}_{max}=\max \left\{\norm{\AA}_{max}, \norm{\cc}_{max}, 1\right\}=\max \left\{\norm{\AA}_{max}, \norm{\cc}_{max}\right\},\]
		and
		\[\norm{\tilde{\bb}}_{max}=\max\left\{|K|, \norm{\bb}_{max}\right\}.\]
	\end{enumerate}
%	Moreover, we can apply the observation that $\nnz(\AAtil)\leq 4\nnz(\AA)$ to Claim \ref{cl: lp-len-time}, and conclude that the reduction can be performed in time $O\left(\nnz(\AA)\right)$.
	
	To estimate the reduction time, as it takes $O\left(\nnz(\tilde{\AA})\right)$ time to construct $\tilde{\AA}$, and $O\left(\nnz(\tilde{\bb})\right)$ time to construct $\tilde{\bb}$, thus the reduction takes time
	\begin{align*}
		O\left(\nnz(\AAtil)+\nnz(\bbtil)\right)&=O\left(\nnz(\AAtil)\right) && \text{Because $\nnz(\bbtil)\leq m\leq \nnz(\AAtil)$}\\
		&=O\left(\nnz(\AA)\right).  && \text{By Eq. \eqref{eq: len-R}}
	\end{align*}
	
%	In terms of the solution mapping time, as it takes constant time to set the value of each entry of $\xx$ by mapping back trivially, and the size of $\xx$ is $n$, thus the solution mapping takes $O(n)$ time.
	%	In a reverse direction, we show the solution mapping rule from a solution $\tilde{\xx}$ of an LEN instance to a solution $\xx$ of an LP instance. 
	%Given $\tilde{\xx}=(\xx^\top,\ss^\top,\alpha)^\top$, we can discard those entries of slack variables $\ss,\alpha$, and map back trivially for those entries of $\xx$. 
%	In a reverse direction, we show the solution mapping rule from a solution $\tilde{\xx}$ of an LEN instance to a solution $\xx$ of an LP instance. 
%Given $\tilde{\xx}=(\xx^\top,\ss^\top,\alpha)^\top$, we can discard those entries of slack variables $\ss,\alpha$, and map back trivially for those entries of $\xx$. 
%As it takes constant time to set the value of each entry of $\xx$, and the size of $\xx$ is $n$, such a mapping rule can be performed in time $O(n)$, as shown in the following claim.
% \begin{claim}
% 	\label{cl: len-lp-time}
% 	Mapping a solution $\xxtil$ of an LEN instance $(\AAtil, \bbtil, \tilde{R})$ back to a solution $\xx$ of an LP instance $(\AA,\bb,\cc,K,R)$ can be performed in time $O(n)$.
% \end{claim}	

\end{proof}


\subsubsection{LPA to LENA}
The above lemma shows the reduction between exactly solving an \textsc{lp} instance and exactly solving an \textsc{len} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.
First of all, we give a definition of the approximate version of \textsc{len}.

\begin{definition}[LEN Approximate Problem (\textsc{lena})]
	\label{def: lena-new}
	An \textsc{lena} instance is given by an \textsc{len} instance $(\AA,\bb, R)$ as in Definition \ref{def: len} and an error parameter $\eps\in[0,1]$, which we collect in a tuple $(\AA,\bb,R,\epsilon)$. We say an algorithm solves the \textsc{lena} problem, if, given any \textsc{lena} instance, it returns a vector $\xx\geq \boldsymbol{0}$ such that
	\begin{align*}
		\abs{\AA\xx-\bb}\leq \eps \vecone,
	\end{align*}
	where $\abs{\cdot}$ is entrywise absolute value and $\vecone$ is the all-1 vector, or it correctly declares that the associated \textsc{len} instance is infeasible.
	%	under the assumption that the polytope has diameter $R$ in $\ell_1$ norm, i.e., for any $\xx\geq\boldsymbol{0}$ with $\abs{\AA\xx- \bb}\leq \boldsymbol{\epsilon}$, we have $\norm{\xx}_1\leq R$.
\end{definition}

\begin{remark*}
	We use an additive error in \textsc{lena} so that it is consistent with 
	the additive error used in  \textsc{lp}. Note this is different
	from an multiplicative error, which is also commonly used in solving 
	systems of linear equations.
	% The error for \textsc{lena} is an additive error, 
	% which is different from the multiplicative error commonly used in approximately solving 
	% systems of linear equations.
\end{remark*}	


%\ming{explain both reduction and solution mapping method here?}
\vspace{8pt}
We use the same reduction method in the exact case to reduce an \textsc{lpa} instance to an \textsc{lena} instance. Furthermore, if an \textsc{lena} solver returns $\xxtil = (\xx^\top, \ss^\top, \alpha)^\top$ for the \textsc{lena} instance $(\AAtil, \bbtil, \Rtil, \epsilon^{le})$, 
then we return $\xx$ for the \textsc{lpa} instance $(\AA, \bb, \cc, K,R, \epsilon^{lp})$;
if the \textsc{lena} solver returns ``infeasible'' for the \textsc{lena} instance, 
then we return ``infeasible'' for the \textsc{lpa} instance.


\begin{lemma}[\textsc{lpa} to \textsc{lena}]
	\label{lm: lpa-lena}
	Given an \textsc{lpa} instance $(\AA,\bb,\cc,K, R, \epsilon^{lp})$ where $\AA\in\Z^{m\times n}, \bb \in \mathbb{Z}^m, \cc \in \mathbb{Z}^n, K \in \mathbb{Z}$,
	% , such that 
	% \[\epsilon^{lp}=\epsilon_1^{lp}\cdot nX(\AA,\bb,\cc,K)+\epsilon_2^{lp}X(\AA,\bb,\cc,K)+\epsilon_3^{lp},\]
	we can construct, in $O(\nnz(\AA))$ time, an \textsc{lena} instance $(\tilde{\AA},\tilde{\bb}, \tilde{R}, \epsilon^{le})$ 
	%such that the dimensions of $\AAtil$ are $(m+1) \times (n+m+1)$,
	where $\tilde{\AA}\in \Z^{\tilde{m}\times\tilde{n}}, \bbtil \in \mathbb{Z}^{\tilde{m}}$ 
	such that 
	\[\tilde{n}= n+m+1,~~\tilde{m}=m+1,~~\nnz(\tilde{\AA})\leq 4\nnz(\AA),\]
	\[
	% \tilde{R}= 5(m+n)RX(\AA,\bb,\cc,K),
	\tilde{R}= 5mRX(\AA,\bb,\cc,K),
	~~ X(\tilde{\AA},\tilde{\bb})=X(\AA,\bb,\cc,K), \]
      \[\eps^{le} = \eps^{lp}.\]
        If the \textsc{lp} instance $(\AA,\bb,\cc,K, R)$ has a solution, then
        the \textsc{len} instance $(\tilde{\AA},\tilde{\bb},
        \tilde{R})$ has a solution.
        Furthermore, if $\tilde{\xx}$ is a solution to the \textsc{lena} instance, 
	then in time $O(n)$, 
	we can compute a solution $\xx$ to the \textsc{lpa} instance.
\end{lemma}	

% \begin{lemma}[\textsc{lpa} to \textsc{lena}]
% 	\label{lm: lpa-lena}
% 	Given an \textsc{lpa} instance $(\AA,\bb,\cc,K, R, \epsilon^{lp}), \AA\in\Z^{m\times n}$, such that 
% 	\[\epsilon^{lp}=\epsilon_1^{lp}\cdot nX(\AA,\bb,\cc,K)+\epsilon_2^{lp}X(\AA,\bb,\cc,K)+\epsilon_3^{lp},\]
% 	we can compute an \textsc{lena} instance $(\tilde{\AA},\tilde{\bb}, \tilde{R}, \boldsymbol{\epsilon}^{le}), \tilde{\AA}\in \Z^{\tilde{m}\times\tilde{n}}$ such that 
% 	\[\boldsymbol{\epsilon}^{le}(i)=\epsilon_1^{le}\norm{\tilde{\aa}_i}_1+\epsilon_2^{le}X(\tilde{\AA},\tilde{\bb})\]
% 	in time $O(\nnz(\AA))$, with
% 	\[\tilde{n}\leq n+m+1,~~\tilde{m}=m+1,~~  \nnz(\tilde{\AA})\leq 4\nnz(\AA),\]
% 	\[\tilde{R}\leq 5(m+n)RX(\AA,\bb,\cc,K),~~ X(\tilde{\AA},\tilde{\bb})=X(\AA,\bb,\cc,K),\]
% 	and
% 	\begin{align*}
% 		\epsilon_1^{le}&=\min\{\epsilon_1^{lp},\epsilon_3^{lp}\},\\
% 		\epsilon_2^{le}&=\epsilon_2^{lp}.
% 	\end{align*}
% 	If $\tilde{\xx}$ solves the \textsc{lena} instance, then in time $O(n)$, we can compute $\xx$ that solve the \textsc{lpa} instance.

% %	Given an \textsc{lpa} instance $(\AA,\bb,\cc,K, \epsilon^{lp}), \AA\in\Z^{m\times n}$, it can be reduced to an \textsc{lena} instance $(\tilde{\AA},\tilde{\bb}, \boldsymbol{\epsilon}^{le}), \tilde{\AA}\in \Z^{\tilde{m}\times\tilde{n}}$ in constant time, such that 
% %	\[\tilde{m}=O(m),~~ \tilde{n}=O(m+n),~~ \nnz(\tilde{\AA})=O(\nnz(\AA)).\]
% %	%	\[\tilde{m}=m+1,\qquad \tilde{n}=m+n+1,\qquad \nnz(\tilde{\AA})=\nnz(\AA)+\nnz(\cc)+n+1.\]
% %	If there is an \textsc{lena} solver with error $\boldsymbol{\epsilon}^{le}_i=\epsilon_1^{le}\norm{\tilde{\aa}_i}_1+\epsilon_2^{le}X(\tilde{\AA},\tilde{\bb})$ for the $i$th linear equation, then it can be translated into an \textsc{lpa} solver with error \[\epsilon^{lp}=\left(\epsilon_1^{lp}\nnz(\AA)+\epsilon_2^{lp}\right)X(\AA,\bb,\cc,K)+\epsilon_3^{lp},\] 
% %	where $\epsilon_1^{lp}=\epsilon_1^{le}, \epsilon_2^{lp}=\epsilon_2^{le}, \epsilon_3^{lp}=\epsilon_1^{le}$.
% \end{lemma}	
\begin{proof}	
	Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: lp-len} also apply here, including the reduction time, problem size, and that the \textsc{len} instance has a feasible solution when the \textsc{lp} instance has one. 
	It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to the \textsc{lena} instance back to an approximate solution to the \textsc{lpa} instance.
	
	Based on the solution mapping method described above, given a solution $\tilde{\xx}$, we discard those entries of $\ss$ and $\alpha$, and map back trivially for those entries of $\xx$. 
	As it takes constant time to set the value of each entry of $\xx$ by mapping back trivially, and the size of $\xx$ is $n$, thus the solution mapping takes $O(n)$ time.
	
	Now, we conduct error analysis. If $\tilde{\xx}= (\xx^\top, \ss^\top, \alpha)^\top$ is a solution to the \textsc{lena} instance, then by Definition \ref{def: lena-new}, $\xxtil$ satisfies 
	\begin{align*}
		\abs{\cc^\top\xx-\alpha-K}&\leq \eps^{le},\\
		\abs{\AA\xx+\ss-\bb}&\leq \eps^{le}\vecone.
	\end{align*}
	
	Taking one direction of the absolution value, we obtain
	\begin{align*}
		\cc^\top\xx&\geq \alpha +  K-\eps^{le} \ge  K-\eps^{le},\\
		\AA\xx&\leq -\ss + \bb+\eps^{le}\vecone \le  \bb+\eps^{le}\vecone,
	\end{align*}
	% where we use the nonnegativity of slack variables, i.e., $\alpha\geq0, \ss\geq \boldsymbol{0}$.
	
	As we set in the reduction that $\eps^{le}=\eps^{lp}$, then we have
	\begin{equation*}
		\label{eq: lpa}
		\begin{aligned}
			\cc^\top\xx&\geq K-\eps^{lp},\\
			\AA\xx&\leq \bb+\eps^{lp}\vecone,
		\end{aligned}
	\end{equation*}
	which indicates that $\xx$ is a solution to the \textsc{lpa} instance by Definition \ref{def: lpa}.
		%		Applying the error of \textsc{lena} solver to the equation $\cc^\top\xx-\alpha=K$, we get
		%		\begin{align*}
		%			\abs{\cc^\top\xx-\alpha-K}&\leq \epsilon_1^{le}(\norm{\cc}_1+1)+\epsilon_2^{le}X(\tilde{\AA},\tilde{\bb})\\
		%			&=\epsilon_1^{le}\norm{\cc}_1+\epsilon_2^{le}X(\AA,\bb,\cc,K)+\epsilon_1^{le}.
		%		\end{align*}
		%		
		%		Thus, we can lower bound $\cc^\top\xx$ by
		%		\begin{equation*}
		%			\cc^\top\xx\geq K-\underbrace{\left(\epsilon_1^{le}\norm{\cc}_1+\epsilon_2^{le}X(\AA,\bb,\cc,K)+\epsilon_1^{le}\right)}_{\tau^{lp}},
		%		\end{equation*}
		%		where we use $\alpha\geq 0$.
		%		As we set in the reduction that $\epsilon_1^{le}=\min\{\epsilon_1^{lp},\epsilon_3^{lp}\},
		%		\epsilon_2^{le}=\epsilon_2^{lp}$, then we have
		%		\begin{align*}
		%			\tau^{lp}&\leq \epsilon^{lp}_1\norm{\cc}_1+\epsilon_2^{lp}X(\AA,\bb,\cc,K)+\epsilon_3^{lp}\\
		%			&\leq \epsilon^{lp}_1\cdot nX(\AA,\bb,\cc,K)+\epsilon_2^{lp}X(\AA,\bb,\cc,K)+\epsilon_3^{lp}\\
		%			&\leq \epsilon^{lp}.
		%		\end{align*}
		%		
		%		Similarly, we applying the error of \textsc{lena} solver to the equation $\aa_i^\top\xx+\ss(i)=\bb(i)$, we get
		%		\begin{align*}
		%			\abs{\aa_i^\top\xx+\ss(i)-\bb(i)}&\leq \epsilon_1^{le}(\norm{\aa_i}_1+1)+\epsilon_2^{le}X(\tilde{\AA},\tilde{\bb})\\
		%			&=\epsilon_1^{le}\norm{\aa_i}_1+\epsilon_2^{le}X(\AA,\bb,\cc,K)+\epsilon_1^{le}.
		%		\end{align*}
		%		Thus, we can upper bound all $\aa_i^\top\xx, i\in[m]$ by
		%		\begin{equation*}
		%			\aa_i^\top\xx\leq \bb(i)+\underbrace{\left(\epsilon_1^{le}\norm{\aa_i}_1+\epsilon_2^{le}X(\AA,\bb,\cc,K)+\epsilon_1^{le}\right)}_{\bar{\tau}^{lp}},
		%		\end{equation*}
		%		where we use $\ss(i)\geq0$.
		%		As we set in the reduction that $\epsilon_1^{le}=\min\{\epsilon_1^{lp},\epsilon_3^{lp}\},
		%		\epsilon_2^{le}=\epsilon_2^{lp}$, then for any $i\in[m]$, we have
		%		\begin{align*}
		%			\bar{\tau}^{lp}&\leq \epsilon_1^{lp}\norm{\aa_i}_1+\epsilon_2^{lp}X(\AA,\bb,\cc,K)+\epsilon_3^{lp}\\
		%%			&\leq \epsilon_1^{lp}\norm{\AA}_{\infty}+\epsilon_2^{lp}X(\AA,\bb,\cc,K)+\epsilon_3^{lp}\\
		%			&\leq\epsilon_1^{lp}\cdot nX(\AA,\bb,\cc,K)+\epsilon_2^{lp}X(\AA,\bb,\cc,K)+\epsilon_3^{lp} \\
		%			&=\epsilon^{lp}.
		%		\end{align*}
		%		Therefore, if $\tilde{\xx}$ solves the \textsc{lena} instance with the error $\epsilon_1^{le}, \epsilon_2^{le}$ as set in the reduction, we can map it back to $\xx$ that solves the \textsc{lpa} instance with error $\epsilon^{lp}$.
\end{proof}

\subsection{LEN(A) to $2$-LEN(A)}
\label{sect: lena-2lena}
\subsubsection{LEN to 2-LEN}
We show the reduction from an \textsc{len} instance $(\AAtil, \bbtil, \Rtil)$ to a \textsc{2-len} instance $(\bar{\AA},\bar{\bb}, \bar{R},2)$. 
The \textsc{len} instance has the following form:
\begin{align*}
	\AAtil\xxtil=\bbtil,
\end{align*}
where $\AAtil\in\Z^{\tilde{m}\times\tilde{n}}, \bbtil\in\Z^{\tilde{m}}$. 
To reduce it to a \textsc{2-len} instance, we utilize a technique called \textit{bitwise decomposition}. 

\ming{describe bitwise decomposition formally. need check}

\begin{algorithm}
	\caption{\textsc{BinaryRepresentation}}
	\label{algo: bitwise-decomposition}
	\KwIn{$z\in \Z$}
	\KwOut{$L$ is a list of power of 2 such that $z=s(z)\sum_{l\in L} 2^{l}$, where $s(z)$ returns the sign of $z$.}
	$r\leftarrow |z|$\;
	$L\leftarrow []$\;
	\For{$r>0$}{
		$L$.append($\floor{\log_2 r}$)\;
		$r\leftarrow r-2^{\floor{\log_2 r}}$\;}
\end{algorithm}

\peng{input: z; output: $(l_0, l_1, \ldots, l_k) \in \{0,1\}^k$ such that $z = \sum_{i=0}^k l_i 2^i$}

To describe how bitwise decomposition works, we first focus on how to decompose a single linear equation in \textsc{len}. 
For an arbitrary linear equation $q$ of \textsc{len}: $\tilde{\aa}_q^\top\xxtil=\bbtil(q), q\in[\tilde{m}]$, bitwise decomposition is composed of the following 4 steps. 
\begin{enumerate}
	\item We run Algorithm \ref{algo: bitwise-decomposition} for each nonzero entry of $\tilde{\aa}_q$ and $\bbtil(q)$ so that each nonzero entry has a binary representation. To simplify notations, we denote the sign of $\tilde{\aa}_q(i)$ as $s_q^i$ and the list returned by \textsc{BinaryRepresentation}($\tilde{\aa}_q(i)$) as $L^i_q$, and the sign of $\bbtil(q)$ as $s_q$ and the list returned by \textsc{BinaryRepresentation}($\tilde{\bb}(q)$) as $L_q$. Thus, the $q$th linear equation of \textsc{len} can be rewritten as
	
	\ming{notation good?}
	\begin{equation}
		\label{eq: binary-representation}
		\sum_{i\in[\tilde{n}]}\underbrace{\left(s_q^i \sum_{l\in L^i_q}2^{l}\right)}_{\tilde{\aa}_q(i)}\xxtil(i)= \underbrace{s_q \sum_{l\in L_q}2^{l}}_{\tilde{\bb}(q)}.	
	\end{equation}
	
	\item Letting $N_q$ denote the maximum element of $L_q$ and $L^i_q, i\in[\tilde{n}]$, i.e.,
	\[N_q=\floor{\log_2\max\left\{\norm{\tilde{\aa}_q}_{max}, \norm{\bbtil(q)}_{max}\right\}},\] 
	\ming{floor or ceil?}
	then we can rearrange the left hand side of Eq. \eqref{eq: binary-representation} by gathering those terms located at the same bit (i.e., with the same weight of power of 2), and obtain
	\begin{equation}
		\label{eq: bit-decomp}
		\sum_{l=0}^{N_q} \left(\sum_{\begin{subarray}{c}
				i\in [\tilde{n}]
		\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)\right) 2^l= s_q\sum_{l\in L_q}2^{l},
	\end{equation}
	where $\mathbbm{1}$ is an indicator function such that
	\[\mathbbm{1}_{[l\in L^i_q]}=\left\{\begin{matrix}
		1& \text{if $l\in L^i_q$}, \\ 
		0& \text{otherwise}.
	\end{matrix}\right.\]

	\item We decompose Eq. \eqref{eq: bit-decomp} into \ming{at most? or exactly} $N_q+1$ linear equations such that each one representing a bit, by matching its left hand side and right hand side of Eq. \eqref{eq: bit-decomp} that are located at the same bit. Note that we also need to introduce carry terms for each decomposed linear equation, which serve to pass the carry from one equation to the next. Without carry terms, the new system may have no solution even though the old one has. Moreover, since the carry can be positive, zero, or negative, we represent the carry as a difference of two nonnegative variables $\cc_q(i)-\dd_q(i), \cc_q(i), \dd_q(i)\geq 0$. Starting from the lowest bit, the following are $N_q+1$ linear equations after decomposition.
	\begin{equation}
		\label{eq: 2-len}
		\begin{aligned}
			\sum_{\begin{subarray}{c}
					i\in [\tilde{n}]
			\end{subarray}}\mathbbm{1}_{[0\in L^i_q]} \cdot s_q^i\xxtil(i)-2[\cc_q(0)-\dd_q(0)]&=s_q\mathbbm{1}_{[0\in L_q]}\\
			\sum_{\begin{subarray}{c}
					i\in [\tilde{n}]
			\end{subarray}}\mathbbm{1}_{[1\in L^i_q]} \cdot s_q^i\xxtil(i)+[\cc_q(0)-\dd_q(0)]-2[\cc_q(1)-\dd_q(1)]&=s_q\mathbbm{1}_{[1\in L_q]}\\
			\vdots\\
			\sum_{\begin{subarray}{c}
					i\in [\tilde{n}]
			\end{subarray}}\mathbbm{1}_{[N_q\in L^i_q]} \cdot s_q^i\xxtil(i)+[\cc_q(N_q-1)-\dd_q(N_q-1)]&=s_q\mathbbm{1}_{[N_q\in L_q]}
		\end{aligned}
	\end{equation}
	
	\item We add an additional constraint for each carry variable $\cc_q(i), \dd_q(i)$ to bound the radius of polytope for the reduced \textsc{2-len} instance. Note that without the additional constraints with respect to carry variables, the radius of polytope cannot be bounded.
	It is because carry variables always appear in pairs $\cc_q(i)-\dd_q(i)$ in the new system. Then given a feasible solution of the new system, any arbitrarily large constant can be added to $\cc_q(i)$ and $\dd_q(i)$ simultaneously to generate another feasible solution, rendering the radius of polytope to be unbounded. \ming{need rephrasing}
	More specifically, if there exists a constant $\Delta\geq 0$ such that
	\[\abs{\cc_q(i)-\dd_q(i)}\leq \Delta, \qquad 0\leq i\leq N_q-1,\]
	then it suffices to restrict carry variables by $\Delta$, i.e.,
	\[\cc_q(i), \dd_q(i)\leq \Delta, \qquad 0\leq i\leq N_q-1,\]
	and it can be further reduced to equality constraints by introducing a nonnegative slack variable for each carry variable, i.e.,
	\[\cc_q(i)+\ss_q^c(i)=\Delta, ~~\dd_q(i)+\ss_q^d(i)=\Delta, \qquad 0\leq i\leq N_q-1,\]
	where $\ss_q^c(i), \ss_q^d(i)\geq \bf{0}$.
	We will show the existence of $\Delta$ and bound it later in Eq. \eqref{eq: R_q}.
\end{enumerate}

Repeating the above process for $\tilde{m}$ times, then all linear equations in \textsc{len} can get decomposed. We denote the coefficient matrix of the new system as $\bar{\AA}$, and the right hand side of the new system as $\bar{\bb}$. Then we get a \textsc{2-len} instance $(\bar{\AA}, \bar{\bb}, \bar{R}, 2)$, where $\bar{R}=\max\{1, \max\{ \norm{\bar{\xx}}_1: \bar{\AA} \bar{\xx} = \bar{\bb}, \bar{\xx} \ge \bf{0} \}\}$. 

If a \textsc{2-len} solver returns $\bar{\xx} = (\xxtil^\top, \cc^\top, \dd^\top, \ss^{c\top}, \ss^{d\top})^\top$ for the \textsc{2-len} instance $(\bar{\AA}, \bar{\bb}, \bar{R}, 2)$, 
then we return $\xxtil$ for the \textsc{len} instance $(\AAtil, \bbtil, \Rtil)$. 
\ming{notation good?}
%Note that the 2-LEN instance obtained by bitwise decomposition exhibits more structures than Definition \ref{def: k-le}. Coefficients of the new linear system are integers between $[-2,2]$, where $\pm2$ comes from the coefficients of carry terms, while the right hand sides are just integers between $[-1,1]$. 

%For solution mapping, if $\bar{\xx}=(\tilde{\xx}^\top, \cc^\top, \dd^\top)^\top$ is a solution to the 2-LEN instance, then $\tilde{\xx}$ is a solution to the LEN instance.

\begin{lemma}[\textsc{len} to \textsc{2-len}]
	\label{lm: len-2len}
	Given an \textsc{len} instance $(\AAtil, \bbtil, \tilde{R})$ where $\tilde{\AA}\in \Z^{\tilde{m}\times\tilde{n}}, \tilde{\bb}\in \Z^{\tilde{m}}$,
	we can construct, in $O\left(\nnz(\tilde{\AA})\log X(\tilde{\AA}, \tilde{\bb})\right)$ time, a \textsc{2-len} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2)$ where $\bar{\AA}\in \Z^{\bar{m}\times\bar{n}}, \bar{\bb}\in\Z^{\bar{m}}$ such that 
	\[\bar{n}\leq \tilde{n}+4\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right),~~
	\bar{m}\leq 3\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right),\]
	\[\nnz(\bar{\AA})\leq 17\nnz(\tilde{\AA})\left(1+\log X(\tilde{\AA},\tilde{\bb})\right),~~
	\bar{R}= 8\tilde{m}\tilde{R}X(\tilde{\AA}, \tilde{\bb})\left(1+\log X(\tilde{\AA}, \tilde{\bb})\right),\]
	\[X(\bar{\AA},\bar{\bb})=2X(\tilde{\AA},\tilde{\bb})\tilde{R},\]
	and if the \textsc{len} instance has a solution, then the \textsc{2-len} instance has a solution.
%	if $\bar{\xx}$ is a solution to the \textsc{2-len} instance, then in time $O(\tilde{n})$, we can compute a solution $\tilde{\xx}$ to the \textsc{len} instance.  
\end{lemma}	
\begin{proof}
	Based on the reduction method described above, from any solution $\tilde{\xx}$ to the \textsc{len} instance such that $\AAtil\xxtil=\bbtil$, it is easy to derive a solution $\bar{\xx} = (\xxtil^\top, \cc^\top, \dd^\top, \ss^{c\top}, \ss^{d\top})^\top$ to the \textsc{2-len} instance. Concretely, for any linear equation $q$ in \textsc{len}, $q\in[\tilde{m}]$, with its decomposed equations as shown in Eq. \eqref{eq: 2-len}, we can set the value of $\cc_q, \dd_q$ from the highest bit as 
	\[\cc_q(N_q-1)=\max\left\{0, ~~s_q\mathbbm{1}_{[N_q\in L_q]}-\sum_{\begin{subarray}{c}
			i\in [\tilde{n}]
	\end{subarray}}\mathbbm{1}_{[N_q\in L^i_q]} \cdot s_q^i\xxtil(i)\right\},
		\]
	
	\[\dd_q(N_q-1)=\max\left\{0, ~~\sum_{\begin{subarray}{c}
			i\in [\tilde{n}]
	\end{subarray}}\mathbbm{1}_{[N_q\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[N_q\in L_q]}\right\}.\]
	And then using backward substitution, we can set the value for the rest entries of $\cc_q$ and $\dd_q$ similarly.
	\begin{align*}
		\cc_q(N_q-2)&=\max\left\{0, ~~s_q\mathbbm{1}_{[(N_q-1)\in L_q]}+2[\cc_q(N_q-1)-\dd_q(N_q-1)]-\sum_{\begin{subarray}{c}
				i\in [\tilde{n}]
		\end{subarray}}\mathbbm{1}_{[(N_q-1)\in L^i_q]} \cdot s_q^i\xxtil(i)\right\}\\
		&=\max\left\{0, ~~\sum_{l=\{N_q-1, N_q\}}\left(s_q\mathbbm{1}_{[l\in L_q]}-\sum_{\begin{subarray}{c}
				i\in [\tilde{n}]
		\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)\right)2^{l-(N_q-1)}\right\},
	\end{align*}
	\[\dd_q(N_q-2)=\max\left\{0, ~~\sum_{l=\{N_q-1, N_q\}}\left(\sum_{\begin{subarray}{c}
			i\in [\tilde{n}]
	\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[l\in L_q]}\right)2^{l-(N_q-1)}\right\};\]
%	\[\dd_q(N_q-2)=\max\left\{0, ~~\sum_{\begin{subarray}{c}
%			i\in [\tilde{n}]
%	\end{subarray}}\mathbbm{1}_{[(N_q-1)\in L^i_q]} \cdot s_q^i\xxtil(i)-2[\cc_q(N_q-1)-\dd_q(N_q-1)]-s_q\mathbbm{1}_{[(N_q-1)\in L_q]}\right\},\]
	\[\vdots\] 	
	\begin{align*}
		\cc_q(0)&=\max\left\{0, ~~s_q\mathbbm{1}_{[1\in L_q]}+2[\cc_q(1)-\dd_q(1)]-\sum_{\begin{subarray}{c}
				i\in [\tilde{n}]
		\end{subarray}}\mathbbm{1}_{[1\in L^i_q]} \cdot s_q^i\xxtil(i)\right\}\\
		&=\max\left\{0, ~~\sum_{l=1}^{N_q}\left(s_q\mathbbm{1}_{[l\in L_q]}-\sum_{\begin{subarray}{c}
				i\in [\tilde{n}]
		\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)\right)2^{l-1}\right\},
	\end{align*}
	\[\dd_q(0)=\max\left\{0, ~~\sum_{l=1}^{N_q}\left(\sum_{\begin{subarray}{c}
			i\in [\tilde{n}]
	\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[l\in L_q]}\right)2^{l-1}\right\}.\]
	
	\ming{check}
%	\[\dd_q(0)=\max\left\{0, ~~\sum_{\begin{subarray}{c}
%			i\in [\tilde{n}]
%	\end{subarray}}\mathbbm{1}_{[1\in L^i_q]} \cdot s_q^i\xxtil(i)-2[\cc_q(1)-\dd_q(1)]-s_q\mathbbm{1}_{[1\in L_q]}\right\}.\]	
	Substituting $\cc_q(0), \dd_q(0)$ back to the equation of the lowest bit, we will get Eq. \eqref{eq: bit-decomp}, the rearranged binary representation of equation $q$: $\tilde{\aa}_q^\top\tilde{\xx}=\tilde{\bb}(q)$. Thus, we show that if $\xxtil$ is a solution to equation $q$ in \textsc{len}, then $(\xxtil^\top, \cc_q^\top, \dd_q^\top)^\top$ is a solution to the system of linear equations as Eq. \eqref{eq: 2-len}.
	
	
	Repeating the above process for all $q\in[\tilde{m}]$, we can get $\cc=(\cc_1^\top, \cdots, \cc_{\tilde{m}}^\top)$ and $\dd=(\dd_1^\top, \cdots, \dd_{\tilde{m}}^\top)$. After obtaining $\cc$ and $\dd$, we can then set
	\[\ss^c=\Delta\vecone-\cc,\qquad \ss^d=\Delta\vecone-\dd,\]
	where $\vecone$ is the all-1 vector. Thus, the solution $\bar{\xx} = (\xxtil^\top, \cc^\top, \dd^\top, \ss^{c\top}, \ss^{d\top})^\top$ to the \textsc{2-len} instance is finally constructed.
%	\ming{remove comments if we want the other direction.}	
	% In the other direction, if $\bar{\xx} = (\xxtil^\top, \cc^\top, \dd^\top, \ss^{c\top}, \ss^{d\top})^\top$ solves the \textsc{2-len} instance, then $\xxtil$ solves the \textsc{len} instance.
	\\
	\\\\
	Now, we track the change of problem size after reduction. Based on the reduction method, each linear equation in \textsc{len} can be decomposed into at most $N$ linear equations, where 
	\begin{equation}
		\label{eq: N}
		N=1+\max_{q\in[\tilde{m}]} N_q=1+\floor{\log_2\max\left\{\norm{\tilde{\AA}}_{max}, \norm{\tilde{\bb}}_{max}\right\}}=1+\floor{\log X(\tilde{\AA},\tilde{\bb})}.
	\end{equation}	
	Thus, given an \textsc{len} instance with $\tilde{n}$ variables, $\tilde{m}$ linear equations, and $\nnz(\tilde{\AA})$ nonzero entries, we compute the size of the reduced \textsc{2-len} instance as following.
	\begin{enumerate}
		\item $\bar{n}$ variables. 
		First, all $\tilde{n}$ variables in \textsc{len} are maintained. Then, for each of the $\tilde{m}$ equations in \textsc{len}, it is decomposed into at most $N$ equations, where at most a pair of carry variables are introduced for each newly added equation. Finally, we introduce a slack variable for each carry variable. Thus, we have
		\[\bar{n}\leq\tilde{n}+2\tilde{m}N +2\tilde{m}N\leq \tilde{n}+4\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right).\]
		
		\item $\bar{m}$ linear constraints. First, each equation in \textsc{len} is decomposed into at most $N$ equations in \textsc{2-len}. Next, we add a new constraint for each carry variable. Thus, we have
		\begin{equation}
			\label{eq: bar-m}
			\bar{m}\leq \tilde{m}N+2\tilde{m}N\leq 3\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right).
		\end{equation}
		
		\item $\nnz(\bar{\AA})$ nonzeros.
		To bound it, first, for each nonzero entry in $\tilde{\AA}$, it will be decomposed into at most $N$ bits, thus becomes at most $N$ nonzero entries in $\bar{\AA}$. 
		Then, each equation in \textsc{2-len} involves at most 4 carry variables.
		Furthermore, there are $2\tilde{m}N$ new constraints for carry variables, and each constraint involves a carry variable and a slack variable.
		In total, we have
		\begin{equation}
			\label{eq: 2len-nnz}
			\begin{aligned}
				\nnz(\bar{\AA})&\leq \nnz(\tilde{\AA})N+4\bar{m}+4\tilde{m}N\\
				&\overset{(1)}{\leq} \nnz(\tilde{\AA})\left(1+\log X(\tilde{\AA},\tilde{\bb})\right)+12\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right)+4\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right)\\
				&\overset{(2)}{\leq}  17\nnz(\tilde{\AA})\left(1+\log X(\tilde{\AA},\tilde{\bb})\right), 
			\end{aligned}
		\end{equation}
		where in step (1), we utilize Eq. \eqref{eq: bar-m} for the bound of $\bar{m}$; 
		and in step (2), we use $\tilde{m}\leq \nnz(\tilde{\AA})$.
		
		\item $\bar{R}$ radius of polytope in $\ell_1$ norm.
		The bound of each original variable in \textsc{len} equals to that of itself in \textsc{2-len}. Then, we need to bound carry variables and slack variables.
		For any linear equation $q$ in \textsc{len}, $q\in[\tilde{m}]$, it can be decomposed into at most $1+N_q$ equations, and at most $N_q$ pairs of carry variables are introduced. Again, we bound carry pairs from the highest bit:		
		\begin{align*}
			\abs{\cc_q(N_q-1)-\dd_q(N_q-1)}&= \abs{s_q\mathbbm{1}_{[N_q\in L_q]}-\sum_{\begin{subarray}{c}
						i\in [\tilde{n}]
				\end{subarray}}\mathbbm{1}_{[N_q\in L^i_q]} \cdot s_q^i\xxtil(i)}\\
			&\leq 1+\norm{\tilde{\xx}}_1=(2^1-1)(1+\norm{\tilde{\xx}}_1),
		\end{align*}
		Using backward substitution, we can bound each pair by
		\begin{align*}
			\abs{\cc_q(N_q-2)-\dd_q(N-_q2)}&\leq1+\norm{\tilde{\xx}}_1+2\abs{\cc_q(N_q-1)-\dd_q(N_q-1)}\leq (2^2-1)(1+\norm{\tilde{\xx}}_1),\\
			&\vdots\\
			\abs{\cc_q(0)-\dd_q(0)}&\leq (2^{N_q}-1)(1+\norm{\tilde{\xx}}_1).
		\end{align*}
		\ming{I didn't use the lowest bit, does it matter?}
		As $N=1+\max_{q\in\tilde{m}}N_q$, we can bound the difference of any carry pair uniformly by
		\begin{equation*}
			\begin{aligned}
				\abs{\cc(i)-\dd(i)}&\leq (2^{N-1}-1)(1+\norm{\tilde{\xx}}_1)\\
				&\leq (2^{\log X(\tilde{\AA},\tilde{\bb}) }-1)(1+\norm{\tilde{\xx}}_1) &&\text{By Eq. \eqref{eq: N}}\\
				&\leq X(\tilde{\AA},\tilde{\bb})(1+\norm{\tilde{\xx}}_1)\\
				&\leq 2X(\tilde{\AA},\tilde{\bb})\tilde{R}. &&\text{Because $\norm{\tilde{\xx}}_1\leq \tilde{R}$ and $\tilde{R}\geq 1$}
			\end{aligned}	
		\end{equation*}
		Thus, it suffices to set 
		\begin{equation}
			\label{eq: R_q}
			\Delta=2X(\tilde{\AA},\tilde{\bb})\tilde{R},
		\end{equation}
		where $\Delta$ is the right hand side of the newly added linear constraints with respect to carry variables. Therefore, we can bound individual carry variables and slack variables by
		\[\cc(i), \dd(i), \ss^c(i), \ss^d(i)\leq 2X(\tilde{\AA},\tilde{\bb})R.\]
		As there are at most $2\tilde{m}(N-1)$ carry variables and $2\tilde{m}(N-1)$ slack variables, we have
		\begin{align*}
			\norm{\bar{\xx}}_1&=\norm{\tilde{\xx}}_1+\norm{\cc}_1+\norm{\dd}_1+\norm{\ss^c}_1+\norm{\ss^d}_1\\
			&\leq \tilde{R}+2X(\tilde{\AA},\tilde{\bb})\tilde{R}\cdot 4\tilde{m}(N-1)\\
			&\leq \tilde{R}+8\tilde{m}\tilde{R}X(\tilde{\AA}, \tilde{\bb})\log X(\tilde{\AA}, \tilde{\bb})\\
			&\leq 8\tilde{m}\tilde{R}X(\tilde{\AA}, \tilde{\bb})\left(1+\log X(\tilde{\AA}, \tilde{\bb})\right). &&\text{Because $\tilde{m}, X(\tilde{\AA}, \tilde{\bb})\geq 1$}
		\end{align*}
		Hence, it suffices to set
		\[\bar{R}=8\tilde{m}\tilde{R}X(\tilde{\AA}, \tilde{\bb})\left(1+\log X(\tilde{\AA}, \tilde{\bb})\right).\]
		
		\item $X(\bar{\AA},\bar{\bb})=2X(\tilde{\AA},\tilde{\bb})\tilde{R}$ because by construction,
		\[\norm{\bar{\AA}}_{max}=2, \qquad \norm{\bar{\bb}}_{max}=\Delta=2X(\tilde{\AA},\tilde{\bb})\tilde{R}\geq 2.\]
	\end{enumerate}
	
	To estimate the reduction time, it is noticed that it takes $O(N)$ time to run Algorithm \ref{algo: bitwise-decomposition} for each nonzero entry of $\tilde{\AA}$ and $\tilde{\bb}$. And there are at most $\nnz(\tilde{\AA})+\nnz(\tilde{\bb})=O\left(\nnz(\tilde{\AA})\right)$ entries to be decomposed. In addition, it takes $O\left(\nnz(\bar{\AA})+\nnz(\bar{\bb})\right)=O\left(\nnz(\bar{\AA})\right)$ to construct $\bar{\AA}$ and $\bar{\bb}$. By Eq. \eqref{eq: 2len-nnz}, performing such a reduction takes time in total
	\begin{align*}
		O\left(N\nnz(\tilde{\AA})+\nnz(\bar{\AA})\right)= O\left(\nnz(\tilde{\AA})\log X(\tilde{\AA}, \tilde{\bb})\right).
	\end{align*}
	
%	In terms of the solution mapping time, as it takes constant time to set the value of each entry of $\tilde{\xx}$, and the size of $\tilde{\xx}$ is $\tilde{n}$, such a mapping rule can be performed in time $O(\tilde{n})$.
\end{proof}

%In the reverse direction, we show the solution mapping rule from a solution $\bar{\xx}$ of a 2-LEN instance to a solution $\tilde{\xx}$ of an LEN instance. 
%Given $\bar{\xx}=(\tilde{\xx}^\top, \cc^\top, \dd^\top)^\top$, we can discard those entries of carry variables $\cc,\dd$, and map back trivially for those entries of $\tilde{\xx}$. 



%Assume a linear equation of
%\[5\tilde{\xx}(1)+3\tilde{\xx}(2)-7\tilde{\xx}(3)=-1.\]
%We decompose its coefficients into bits,
%\[(2^0+2^2)\tilde{\xx}(1)+(2^0+2^1)\tilde{\xx}(2)-(2^0+2^1+2^2)\tilde{\xx}(3)=-2^0.\]
%We can rearrange this equation by gathering those terms with the same weight of power of 2, and obtain
%\[\left[\tilde{\xx}(1)+\tilde{\xx}(2)-\tilde{\xx}(3)\right]2^0+\left[\tilde{\xx}(2)-\tilde{\xx}(3)\right]2^1+\left[\tilde{\xx}(1)-\tilde{\xx}(3)\right]2^2=-1\cdot2^0.\]
%The above equation can be decomposed to 3 linear equations, together with carry terms $(\cc(i)-\dd(i))$ to pass the carry from one equation to the next. Note that without carry terms, the new system may have no solution. Moreover, the carry can be positive or negative. That is why we represent the carry by the difference of two nonnegative variables $\cc(i), \dd(i)\geq 0$.
%\begin{align*}
%	\tilde{\xx}(1)+\tilde{\xx}(2)-\tilde{\xx}(3)-2\left[\cc(0)-\dd(0)\right]&=-1\\
%	\tilde{\xx}(2)-\tilde{\xx}(3)+\left[\cc(0)-\dd(0)\right]-2\left[\cc(1)-\dd(1)\right]&=0\\
%	\tilde{\xx}(1)-\tilde{\xx}(3)+\left[\cc(1)-\dd(1)\right]&=0
%\end{align*}
%It is noticed that the 2-LEN obtained by bitwise decomposition exhibits more structures than the definition (Def. \ref{def: k-le}). Coefficients of the new linear system are integers between $[-2,2]$, where $\pm2$ comes from the coefficients of carry terms, while the right hand sides are integers between $[-1,1]$.

\subsubsection{LENA to 2-LENA}
The above lemma shows the reduction between exactly solving an \textsc{len} instance and exactly solving a \textsc{2-len} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.
First of all, we give a definition of the approximate version of \textsc{2-len}.

\begin{definition}[$k$-LEN Approximate Problem ($k$-\textsc{lena})]
	\label{def: klena-new}
	A $k$-\textsc{lena} instance is given by a $k$-\textsc{len} instance $(\AA,\bb,R,k)$ as in Definition \ref{def: k-le} and an error parameter $\eps\in[0,1]$, which we collect in a tuple $(\AA,\bb,R,k,\epsilon)$. We say an algorithm solves the $k$-\textsc{lena} problem, if, given any $k$-\textsc{lena} instance, it returns a vector $\xx\geq \boldsymbol{0}$ such that
	\begin{align*}
		\abs{\AA\xx-\bb}\leq \eps\vecone, 
	\end{align*}
	where $\abs{\cdot}$ is entrywise absolute value and $\vecone$ is the all-1 vector, or it correctly declares that the associated $k$-\textsc{len} instance is infeasible.
\end{definition}

We can use the same reduction method in the exact case to reduce an \textsc{lena} instance to a \textsc{2-lena} instance. Furthermore, if a \textsc{2-lena} solver returns $\bar{\xx} = (\xxtil^\top, \cc^\top, \dd^\top, \ss^{c\top}, \ss^{d\top})^\top$ for the \textsc{2-lena} instance $(\bar{\AA}, \bar{\bb}, \bar{R}, 2, \epsilon^{2le})$, 
then we return $\xxtil$ for the \textsc{lena} instance $(\AAtil, \bbtil, \Rtil, \epsilon^{le})$. 

\begin{lemma}[\textsc{lena} to \textsc{2-lena}]
	Given an \textsc{lena} instance $(\tilde{\AA},\tilde{\bb},\tilde{R}, \epsilon^{le})$, where $\tilde{\AA}\in \Z^{\tilde{m}\times\tilde{n}}, \tilde{\bb}\in \Z^{\tilde{m}}$,
	we can construct, in $O\left(\nnz(\tilde{\AA})\log X(\tilde{\AA}, \tilde{\bb})\right)$ time, a \textsc{2-lena} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2,\epsilon^{2le})$ where $\bar{\AA}\in \Z^{\bar{m}\times\bar{n}}, \bar{\bb}\in\Z^{\bar{m}}$ such that 
	\[\bar{n}\leq \tilde{n}+4\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right),~~
	\bar{m}\leq 3\tilde{m}\left(1+\log X(\tilde{\AA},\tilde{\bb})\right),\]
	\[\nnz(\bar{\AA})\leq 17\nnz(\tilde{\AA})\left(1+\log X(\tilde{\AA},\tilde{\bb})\right),~~
	\bar{R}= 8\tilde{m}\tilde{R}X(\tilde{\AA}, \tilde{\bb})\left(1+\log X(\tilde{\AA}, \tilde{\bb})\right),\]
	\[X(\bar{\AA},\bar{\bb})=2X(\tilde{\AA},\tilde{\bb})\tilde{R},\]
	\[\epsilon^{2le}=\frac{\eps^{le}}{2X(\tilde{\AA},\tilde{\bb})}.\]
	If the \textsc{len} instance $(\tilde{\AA},\tilde{\bb},\tilde{R})$ has a solution, then the \textsc{2-len} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2)$ has a solution.
	Furthermore, if $\bar{\xx}$ is a solution to the \textsc{2-lena} instance, then in time $O(\tilde{n})$, we can compute a solution $\tilde{\xx}$ to the \textsc{lena} instance.  
	%	Given an \textsc{lena} instance $(\tilde{\AA},\tilde{\bb},\tilde{R}, \boldsymbol{\epsilon}^{le}), \tilde{\AA}\in \Z^{\tilde{m}\times\tilde{n}}$, such that 
	%	\[\boldsymbol{\epsilon}^{le}(i)=\epsilon_1^{le}\norm{\tilde{\aa}_i}_1+\epsilon_2^{le}X(\tilde{\AA},\tilde{\bb}),\]
	%	we can compute a \textsc{2-lena} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2,\boldsymbol{\epsilon}^{2le}), \bar{\AA}\in\Z^{\bar{m}\times\bar{n}}$, such that
	%	\[\boldsymbol{\epsilon}^{2le}(i)=\epsilon_1^{2le}\norm{\bar{\aa}_i}_1+\epsilon_2^{2le}\bar{\bb}(i)+\epsilon_3^{2le}\]
	%	in time $O\left(\nnz(\tilde{\AA})\log X(\tilde{\AA}, \tilde{\bb})\right)$, with 
	%	\[\bar{n}\leq \tilde{n}+4\tilde{m}+2\tilde{m}\log X(\tilde{\AA},\tilde{\bb}),~~
	%	\bar{m}\leq 2\tilde{m}+\tilde{m}\log X(\tilde{\AA},\tilde{\bb}),\]
	%	\[\nnz(\bar{\AA})\leq 10\nnz(\tilde{\AA})+5\nnz(\tilde{\AA})\log X(\tilde{\AA},\tilde{\bb}),~~
	%	\bar{R}\leq 16\tilde{m}\tilde{R}X(\tilde{\AA}, \tilde{\bb})(3+\log X(\tilde{\AA}, \tilde{\bb})),\]
	%	and
	%	\begin{align*}
	%		\epsilon^{2le}_1&=\min\left\{\epsilon_1^{le}, \frac{\epsilon^{le}_2}{64}\right\},\\
	%		\epsilon^{2le}_2&=\frac{\epsilon^{le}_2}{64},\\
	%		\epsilon^{2le}_3&=\frac{\epsilon^{le}_2}{64}.
	%	\end{align*}
	%	If $\bar{\xx}$ solves the \textsc{2-lena} instance, then in time $O(\tilde{n})$, we can compute $\tilde{\xx}$ that solves the \textsc{lena} instance.  
\end{lemma}	
\begin{proof}
	Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: len-2len} also apply here, including the reduction time, problem size, and that \textsc{2-len} has a feasible solution when \textsc{len} has one. 
	It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{2-lena} back to an approximate solution to \textsc{lena}.
	
	Based on the solution mapping method described above, given a solution $\bar{\xx}$, we discard those entries of carry variables and slack variables, and map back trivially for those entries of $\xxtil$. As it takes constant time to set the value of each entry of $\xxtil$ by mapping back trivially, and the size of $\xxtil$ is $\tilde{n}$, thus the solution mapping takes $O(\tilde{n})$ time.
	
	\ming{check, not sure if the newly added constraints will affect error analysis}
	Now, we conduct error analysis. By Definition \ref{def: klena-new}, the error of each linear equation in \textsc{2-lena} can be bounded by $\epsilon^{2le}$. By decomposing the $q$th linear equation in \textsc{lena} into equations shown in Eq. \eqref{eq: 2-len}, similarly, we bound the error from the highest bit, and obtain:
	\[\abs{\sum_{\begin{subarray}{c}
			i\in [\tilde{n}]
	\end{subarray}}\mathbbm{1}_{[N_q\in L^i_q]} \cdot s_q^i\xxtil(i)+[\cc_q(N_q-1)-\dd_q(N_q-1)]-s_q\mathbbm{1}_{[N_q\in L_q]}}\leq \epsilon^{2le},\]
	which can be rearranged as
	\begin{small}
	\begin{equation}
		\label{eq: 2len-error-1}
		-\epsilon^{2le}-[\cc_q(N_q-1)-\dd_q(N_q-1)]\leq\sum_{\begin{subarray}{c}
				i\in [\tilde{n}]
		\end{subarray}}\mathbbm{1}_{[N_q\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[N_q\in L_q]}\leq \epsilon^{2le}-[\cc_q(N_q-1)-\dd_q(N_q-1)].
	\end{equation}
	\end{small}
	For the second highest bit, we have
	\begin{small}
	\begin{multline}
		\label{eq: 2len-error-2}
		-\epsilon^{2le}+2[\cc_q(N_q-1)-\dd_q(N_q-1)]-[\cc_q(N_q-2)-\dd_q(N_q-2)]\\
		\leq\sum_{\begin{subarray}{c}
				i\in [\tilde{n}]
		\end{subarray}}\mathbbm{1}_{[(N_q-1)\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[(N_q-1)\in L_q]}\\
	\leq \epsilon^{2le}+2[\cc_q(N_q-1)-\dd_q(N_q-1)]-[\cc_q(N_q-2)-\dd_q(N_q-2)].
	\end{multline}
	\end{small}
	We can eliminate the pair of carry $[\cc_q(N_q-1)-\dd_q(N_q-1)]$ by computing $2\times\text{Eq. \eqref{eq: 2len-error-1}} + \text{Eq. \eqref{eq: 2len-error-2}}$, and obtain
	\begin{small}
		\begin{multline}
			\label{eq: 2len-error-3}
			-(2^0+2^1)\epsilon^{2le}-[\cc_q(N_q-2)-\dd_q(N_q-2)]\\
			\leq\sum_{l=\{N_q-1, N_q\}}\left(\sum_{\begin{subarray}{c}
					i\in [\tilde{n}]
			\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[l\in L_q]}\right)2^{l-(N_q-1)}\\
			\leq (2^0+2^1)\epsilon^{2le}-[\cc_q(N_q-2)-\dd_q(N_q-2)].
		\end{multline}
	\end{small}
	By repeating the process until the equation of the lowest bit, we can eliminate all pairs of carry variables and obtain
	\begin{small}
		\begin{multline}
			\label{eq: 2len-error-4}
			-(2^0+\cdots+2^{N_q})\epsilon^{2le}
			\leq\underbrace{\sum_{l=0}^{N_q}\left(\sum_{\begin{subarray}{c}
					i\in [\tilde{n}]
			\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[l\in L_q]}\right)2^{l}}_{=\tilde{\aa}_q^\top\tilde{\xx}-\tilde{\bb}(q) ~~ \text{by Eq.  \eqref{eq: bit-decomp}}}
			\leq (2^0+\cdots+2^{N_q})\epsilon^{2le}.
		\end{multline}
	\end{small}
%	Compared to Eq. \eqref{eq: bit-decomp}, it is noticed that 
%	\[\tilde{\aa}_q^\top\tilde{\xx}-\tilde{\bb}(q)=\sum_{l=0}^{N_q}\left(\sum_{\begin{subarray}{c}
%			i\in [\tilde{n}]
%	\end{subarray}}\mathbbm{1}_{[l\in L^i_q]} \cdot s_q^i\xxtil(i)-s_q\mathbbm{1}_{[l\in L_q]}\right)2^{l},\]
	Hence, we can bound the $q$th linear equation in \textsc{len} by
	\[\abs{\tilde{\aa}_q^\top\tilde{\xx}-\tilde{\bb}(q)}\leq (2^0+\cdots+2^{N_q})\epsilon^{2le}\leq2^{N_q+1}\epsilon^{2le},\]
	which implies that the error of the $q$th equation of \textsc{lena} is accumulated as a weighted sum of at most $N_q$ equations in \textsc{2-lena}, where the weight is in the form of power of 2. 
	
	To bound all the linear equations in \textsc{lena} uniformly, we have
	\begin{align*}
		\tau^{le}=&~\max_{q\in[\tilde{m}]}\abs{\tilde{\aa}_q^\top\tilde{\xx}-\tilde{\bb}(q)}\\
		\leq &~ \max_{q\in[\tilde{m}]} 2^{N_q+1}\epsilon^{2le}\\
		\leq &~ 2^{N}\epsilon^{2le} && \text{Because $N=1+\max_{q\in\tilde{m}}N_q$}\\
		\leq &~ 2^{1+\log X(\tilde{\AA},\tilde{\bb})}\epsilon^{2le} &&\text{Because $N=1+\floor{\log X(\tilde{\AA},\tilde{\bb})}$}\\
		\leq &~ 2X(\tilde{\AA},\tilde{\bb})\epsilon^{2le}.
	\end{align*}	 
	As we set in the reduction that $\epsilon^{2le}=\frac{\eps^{le}}{2X(\tilde{\AA},\tilde{\bb})}$, then we have
	\begin{align*}
		\tau^{le}\leq 2X(\tilde{\AA},\tilde{\bb})\frac{\eps^{le}}{2X(\tilde{\AA},\tilde{\bb})}
		=\epsilon^{le},
	\end{align*}
	which indicates that $\tilde{\xx}$ is a solution to the \textsc{lena} instance.
	
%	Let $\bar{\aa}_{i(q)}^\top\bar{\xx}=\bar{\bb}(i(q)), i\leq N, q\in[\tilde{m}]$ denote the equation that represents the $i$th bit in the decomposition of the $q$th equation in \textsc{lena}. If $\bar{\xx}$ is a solution to the \textsc{2-lena} instance, then by Definition \ref{def: klena-new}, we have	
%	\begin{align*}
%		\abs{\bar{\aa}_{i(q)}^\top\bar{\xx}-\bar{\bb}(i(q))}\leq \epsilon^{2le}, \qquad  i\leq N, ~q\in[\tilde{m}].
%	\end{align*}
%	\ming{check}
%	
%	The error of the $q$th equation of \textsc{lena} is then accumulated as a weighted sum of at most $N$ equations in \textsc{2-lena}, where the weight is in the form of power of 2. Then we have 
%	\begin{equation}
%		\label{eq: le-2le}
%		\begin{aligned}
%			\tau^{le}=&~\max_{q\in[\tilde{m}]}\abs{\tilde{\aa}_q^\top\tilde{\xx}-\tilde{\bb}(q)}\\
%			\leq&~ \max_{q\in[\tilde{m}]}\left\{2^0 \abs{\bar{\aa}_{1(q)}^\top\bar{\xx}-\bar{\bb}(1(q))}+2^1\abs{\bar{\aa}_{2(q)}^\top\bar{\xx}-\bar{\bb}(2(q))}+\cdots + 2^N\abs{\bar{\aa}_{N(q)}^\top\bar{\xx}-\bar{\bb}(N(q))}\right\}\\
%			\leq&~ \epsilon^{2le}(2^0+\cdots+2^N)\\
%			\leq&~ 2^{N+1}\epsilon^{2le}\\
%			\leq &~ 2^{2+\log X(\tilde{\AA},\tilde{\bb})}\epsilon^{2le} \\
%			=&~ 4X(\tilde{\AA},\tilde{\bb})\epsilon^{2le}.
%		\end{aligned}
%	\end{equation}
	
	
	%		\begin{align*}
	%			\abs{\bar{\aa}_{i(q)}^\top\bar{\xx}-\bar{\bb}(i(q))}\leq \boldsymbol{\epsilon}^{2le}(i(q))= \epsilon_1^{2le}\norm{\bar{\aa}_{i(q)}}_1+\epsilon_2^{2le}\bar{\bb}(i(q))+\epsilon_3^{2le}.
	%		\end{align*}
	%		\ming{check}
	%		The error of the $q$th equation of \textsc{lena} is accumulated as a weighted sum of at most $N$ equations of \textsc{2-lena}, and we have 
	%		\begin{equation}
	%			\label{eq: le-2le}
	%			\begin{aligned}
	%				\abs{\tilde{\aa}_q^\top\tilde{\xx}-\tilde{\bb}(q)}\leq&~ 2^0 \abs{\bar{\aa}_{1(q)}^\top\bar{\xx}-\bar{\bb}(1(q))}+2^1\abs{\bar{\aa}_{2(q)}^\top\bar{\xx}-\bar{\bb}(2(q))}+\cdots + 2^N\abs{\bar{\aa}_{N(q)}^\top\bar{\xx}-\bar{\bb}(N(q))}\\
	%				\leq&~ \epsilon_1^{2le}\left(2^0\norm{\bar{\aa}_{1(q)}}_1+\cdots+2^N \norm{\bar{\aa}_{N(q)}}_1\right)+\epsilon_2^{2le}\left(2^0\bar{\bb}(1(q))+\cdots+2^N \bar{\bb}(N(q))\right)\\
	%				&+\epsilon_3^{2le}(2^0+\cdots+2^N).
	%			\end{aligned}
	%		\end{equation}
	%		Notice that 
	%		\begin{align*}
	%			\norm{\tilde{\aa}_q}_1&\overset{(1)}{=}2^0\left(\norm{\bar{\aa}_{1(q)}}_1-4\right)+2^1\left(\norm{\bar{\aa}_{2(q)}}_1-6\right)+\cdots+2^N \left(\norm{\bar{\aa}_{N(q)}}_1-2\right)\\
	%			&\geq2^0\norm{\bar{\aa}_{1(q)}}_1+\cdots+2^N \norm{\bar{\aa}_{N(q)}}_1-6(2^0+\cdots+2^N),
	%		\end{align*}
	%		where in step (1), the constant 2, 4, 6 that are subtracted in parentheses is due to the coefficients of carry variables.
	%		
	%		Hence, we can upper bound
	%		\[2^0\norm{\bar{\aa}_{1(q)}}_1+\cdots+2^N \norm{\bar{\aa}_{N(q)}}_1\leq \norm{\tilde{\aa}_q}_1+6(2^0+\cdots+2^N),\] 
	%		and also 
	%		\[\bar{\bb}(i(q))\leq 1, i\in[\bar{m}].\] 
	%		Plugging these upper bounds back to Eq. \eqref{eq: le-2le}, we obtain
	%		\begin{align*}
	%			\boldsymbol{\tau}^{le}(q)=\abs{\tilde{\aa}_q^\top\tilde{\xx}-\tilde{\bb}(q)}\leq&~ \epsilon_1^{2le}\norm{\tilde{\aa}_q}_1+(6\epsilon^{2le}_1+\epsilon_2^{2le}+\epsilon_3^{2le})(2^0+\cdots+2^N)\\
	%			=&~ \epsilon_1^{2le}\norm{\tilde{\aa}_q}_1+2^{N+1}(6\epsilon^{2le}_1+\epsilon_2^{2le}+\epsilon_3^{2le})\\
	%			=&~ \epsilon_1^{2le}\norm{\tilde{\aa}_q}_1+2^{3+\log X(\tilde{\AA},\tilde{\bb}) }(6\epsilon^{2le}_1+\epsilon_2^{2le}+\epsilon_3^{2le})\\
	%			\leq&~ \epsilon_1^{2le}\norm{\tilde{\aa}_q}_1+8(6\epsilon^{2le}_1+\epsilon_2^{2le}+\epsilon_3^{2le})X(\tilde{\AA},\tilde{\bb}).
	%		\end{align*}
	%	
	%		As we set in the reduction that $\epsilon^{2le}_1=\min\left\{\epsilon_1^{le}, \frac{\epsilon^{le}_2}{64}\right\},
	%		\epsilon^{2le}_2=\frac{\epsilon^{le}_2}{64},
	%		\epsilon^{2le}_3=\frac{\epsilon^{le}_2}{64}$, then we have
	%		\begin{align*}
	%			\boldsymbol{\tau}^{le}(q)&\leq\epsilon^{le}_1\norm{\tilde{\aa}_q}_1+8(\frac{6\epsilon^{le}_2}{64}+\frac{\epsilon^{le}_2}{64}+\frac{\epsilon^{le}_2}{64})X(\tilde{\AA}, \tilde{\bb})\\
	%			&=\epsilon^{le}_1\norm{\tilde{\aa}_q}_1+\epsilon^{le}_2X(\tilde{\AA}, \tilde{\bb})\\
	%			&=\boldsymbol{\epsilon}^{le}(q).
	%		\end{align*}
	%	Therefore, if $\bar{\xx}$ solves the \textsc{2-lena} instance with the error $\epsilon^{2le}_1, epsilon^{2le}_2, epsilon^{2le}_3$ as set in the reduction, we can map it back to $\tilde{\xx}$ that solves the \textsc{lena} instance with error $\boldsymbol{\epsilon}^{le}$.
\end{proof}

\subsection{$2$-LEN(A) to $1$-LEN(A)}
\label{sect: 2lena-1lena}
\subsubsection{$2$-LEN to $1$-LEN}
%To reduce a \textsc{2-lena} instance to a \textsc{1-lena} instance, we need to deal with two cases:
%\paragraph{Case 1.} Every occurrence of the variable $\bar{\xx}(j)$ with coefficients $\bar{\AA}(i,j)=\pm2$, we can replace this term by $\pm(\bar{\xx}(j)+\bar{\xx}'(j))$, and add the equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$. 
%\paragraph{Case 2.} If $\bar{\bb}(i)=2$, we can change $\bar{\aa}_i^\top\bar{\xx}=2$ to $\bar{\aa}_i^\top\bar{\xx}-\zz(i)=1, \zz(i)=1$. 
We show the reduction from a \textsc{2-len} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2)$ to a \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$. The \textsc{2-len} instance has the form of $\bar{\AA}\bar{\xx}=\bar{\bb}$, where entries of $\bar{\AA}$ are integers between $[-2,2]$. 
To reduce it to a \textsc{1-len} instance, at every occurrence of the variable $\bar{\xx}(j)$ with coefficient $\bar{\AA}(i,j)=\pm2$, we replace this term $\pm2\bar{\xx}(j)$ by two terms $\pm(\bar{\xx}(j)+\bar{\xx}'(j))$, and add an additional equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$. 

If an \textsc{1-len} solver returns $\hat{\xx}=(\bar{\xx}^\top, \bar{\xx}'^\top)^\top$ for the \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$, then we return $\bar{\xx}$ for the \textsc{2-len} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2)$.
%Given a solution $\hat{\xx}$ returned by the \textsc{1-lena} solver, we can map back those variables that get split by taking the average of their corresponding two terms, and trivially map back those variables without getting split. As the size of $\bar{\xx}$ is $\bar{n}$, such a mapping rule can be performed in $O(\bar{n})$ time.	

\begin{lemma}[\textsc{2-len} to \textsc{1-len}]
	\label{lm: 2len-1len}
	Given a \textsc{2-len} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2)$ where $\bar{\AA}\in\Z^{\bar{m}\times\bar{n}}, \bar{\bb}\in \Z^{\bar{m}}$, 
	we can construct, in $O(\nnz(\bar{\AA}))$ time, a \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$ where $\hat{\AA}\in \Z^{\hat{m}\times\hat{n}}, \hat{\bb}\in \Z^{\hat{m}}$ such that
	\[\hat{n}\leq 2\bar{n},~~\hat{m}\leq \bar{m}+\bar{n},~~ \nnz(\hat{\AA})\leq 4\nnz(\bar{\AA}),~~ \hat{R}=2\bar{R},\]
	\[X(\hat{\AA},\hat{\bb})=X(\bar{\AA},\bar{\bb}),\]
	and if the \textsc{2-len} instance has a solution, then the \textsc{1-len} instance has a solution.
%	if $\hat{\xx}$ is a solution to the \textsc{1-len} instance, then in time $O(\bar{n})$, we can compute a solution $\bar{\xx}$ to the \textsc{2-len} instance.
\end{lemma}	
\begin{proof}
	Based on the reduction described above, from any solution $\bar{\xx}$ to the \textsc{2-len} instance such that $\bar{\AA}\bar{\xx}=\bar{\bb}$, it is easy to derive a solution $\hat{\xx}=(\bar{\xx}^\top, \bar{\xx}'^\top)^\top$ to the \textsc{1-len} instance. Concretely, for each $\bar{\xx}(j)$ having a $\pm2$ coefficient in $\bar{\AA}$, we set its corresponding entry in $\bar{\xx}'$ to be equal to $\bar{\xx}(j)$.\ming{need rephrasing} As such, we have $\pm(\bar{\xx}(j)+\bar{\xx}'(j))=\pm2\bar{\xx}(j)$, which implies that $\hat{\xx}$ is a solution to \textsc{1-len} if $\bar{\xx}$ is a solution to \textsc{2-len}.
	
	Now, we track the change of problem size after reduction. Based on the reduction method, given a \textsc{2-len} instance with $\bar{n}$ variables, $\bar{m}$ linear equations, and $\nnz(\bar{\AA})$ nonzero entries, we can compute the size of the reduce \textsc{1-len} instance as following.
	\begin{enumerate}
		\item $\hat{n}$ variables, where
		\[\hat{n}\leq 2\bar{n}.\]
		It is because each variable $\bar{\xx}(j)$ in \textsc{2-len} is replaced by at most 2 variables $\bar{\xx}(j)+\bar{\xx}'(j)$ in \textsc{1-len}.
		
		\item $\hat{m}$ linear constraints. In addition to the original $\bar{m}$ linear equations, each variable $\bar{\xx}(j)$ with $\pm2$ coefficient in \textsc{2-len} will introduce a new equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$ in \textsc{1-len}.  Thus,
		\[\hat{m}\leq \bar{m}+\bar{n}.\]
		
		
		\item $\nnz(\hat{\AA})$ nonzeros. To bound it,
		first, each nonzero entry in $\bar{\AA}$ becomes at most two nonzero entries in $\hat{\AA}$ because of the replacement of $\pm2\bar{\xx}(j) $ by $\pm(\bar{\xx}(j)+\bar{\xx}'(j))$.
		Next, at most $2\bar{n}$ new nonzero entries are generated because of the newly added equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$. Thus,
		\[\nnz(\hat{\AA})\leq 2(\nnz(\bar{\AA})+\bar{n})\leq4\nnz(\bar{\AA}),\]
		where we use $\bar{n}\leq \nnz(\bar{\AA})$. \ming{do we need to prove it?}
		
		\item $\hat{R}$ radius of polytope in $\ell_1$ norm. We have
		\[\norm{\hat{\xx}}_1=\norm{\bar{\xx}}_1+\norm{\bar{\xx}'}_1\leq 2\norm{\bar{\xx}}_1\leq 2\bar{R}.\]
		Hence, it suffices to set
		\[\hat{R}= 2\bar{R}.\] 
		
		\item $X(\hat{\AA},\hat{\bb})=X(\bar{\AA},\bar{\bb})$ because by construction,
		\[\norm{\hat{\AA}}_{max}\leq \norm{\bar{\AA}}_{max},\qquad \norm{\hat{\bb}}_{max}=\norm{\bar{\bb}}_{max}.\]
%		It is because the bound of each variable in \textsc{2-len} equals to the bound of itself, while the number of variables increases at least twice in \textsc{1-len}.
		
		%		\begin{enumerate}
		%			\item $\hat{n}$ variables, where
		%			\[\hat{n}\leq 2\bar{n}+\bar{m}.\]
		%			\begin{proof}
		%				First, each variable $\bar{\xx}(j)$ in \textsc{2-lena} is represented by at most 2 variables $\bar{\xx}(j)+\bar{\xx}'(j)$ in \textsc{1-lena}. Then, each equation in \textsc{2-lena} introduces at most one new variable $\zz(i)$ in \textsc{1-lena}. 
		%			\end{proof}
		%			\item $\hat{m}$ linear constraints, where
		%			\[\hat{m}\leq 2\bar{m}+\bar{n}.\]
		%			\begin{proof}
		%				First, each equation $i$ in \textsc{2-lena} is represented by at most 2 equations in \textsc{1-lena} if $\bar{\bb}(i)=2$. Then, each variable $\bar{\xx}(j)$ in \textsc{2-lena} introduces at most one new equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$ in \textsc{1-lena}. 
		%			\end{proof}
		%			\item $\nnz(\hat{\AA})$ nonzeros, where
		%			\[\nnz(\hat{\AA})\leq 2(\nnz(\bar{\AA})+\bar{m}+\bar{n})\leq6\nnz(\bar{\AA}).\]
		%			\begin{proof}
		%				First, each nonzero entry in $\bar{\AA}$ becomes at most two nonzero entries in $\hat{\AA}$ because of $\pm(\bar{\xx}(j)+\bar{\xx}'(j))$.
		%				Then, at most $\bar{m}$ new nonzero entries are generated because of the appearance of $\zz(i)$.
		%				Next, at most $2\bar{n}$ new nonzero entries are generated because of the newly added equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$.
		%				Finally, at most $\bar{m}$ new nonzero entries are generated because of the newly added equation $\zz(i)=1$.
		%			\end{proof}
		%			\item $\hat{R}$ diameter of polytope in $\ell_1$ norm, where
		%			\[\hat{R}\leq \bar{R}+\bar{m}.\] 
		%			\ming{check}
		%			\begin{proof}
		%				First, the bound of each variable $\bar{\xx}(j)$ in \textsc{2-lena} equals to the bound of itself or $\bar{\xx}(j)+\bar{\xx}'(j)$ in \textsc{1-lena}.
		%				Then, there are at most $\bar{m}$ entries corresponding to $\zz(i)$ in \textsc{1-lena}, and each of which is bounded by 1. 
		%				%plus certain error terms, as shown in Eq. \eqref{eq: 2le-1le-z}.
		%			\end{proof}
		%			Note that $\nnz(\bar{\AA})\geq \bar{m}, \bar{n}$.
	\end{enumerate}
	
	To estimate the reduction time, it takes constant time to deal with each $\bar{\AA}(i,j)$ being $\pm2$, and there are at most $\nnz(\bar{\AA})$ occurrences of $\pm2$ to be dealt with. Hence, it takes $O(\nnz(\bar{\AA}))$ time to eliminate all the occurrence of $\pm2$. Moreover, copy the rest coefficients also takes $O(\nnz(\bar{\AA}))$ time. Thus, the reduction of this step takes $O(\nnz(\bar{\AA}))$ time. 
	
%	In terms of the solution mapping time, as the size of $\bar{\xx}$ is $\bar{n}$, such a mapping rule can be performed in $O(\bar{n})$ time.	
\end{proof}
	
	\subsubsection{$2$-LENA to $1$-LENA}
	The above lemma shows the reduction between exactly solving a \textsc{2-len} instance and exactly solving a \textsc{1-len} instance. 
	Next, we generalize the case with exact solutions to the case that allows approximate solutions.

	
	We can use the same reduction method in the exact case to reduce a \textsc{2-lena} instance to a \textsc{1-lena} instance. We can also use the same solution mapping method, but we make a slight adjustment in the approximate case for the simplicity of the following error analysis. More specifically, if a \textsc{1-lena} solver returns $\hat{\xx}=(\xx^\top, \xx'^\top)^\top$ for the \textsc{1-lena} instance $(\hat{\AA}, \hat{\bb}, \hat{R}, 1, \epsilon^{1le})$, instead of returning $\xx$ directly as the solution to the \textsc{2-lena} instance $(\bar{\AA}, \bar{\bb}, \bar{R}, 2, \epsilon^{2le})$, we map back those variables that get split by taking the average of their corresponding two terms in $\hat{\xx}$, and trivially map back those variables without getting split. \ming{need to rephrase}


\begin{lemma}[\textsc{2-lena} to \textsc{1-lena}]
	\label{lm: 2lena-1lena}
	Given a \textsc{2-lena} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2,\epsilon^{2le})$ where $\bar{\AA}\in\Z^{\bar{m}\times\bar{n}}, \bar{\bb}\in \Z^{\bar{m}}$, 
	we can construct, in $O(\nnz(\bar{\AA}))$ time, a \textsc{1-lena} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1,\epsilon^{1le})$ where $\hat{\AA}\in \Z^{\hat{m}\times\hat{n}}, \hat{\bb}\in \Z^{\hat{m}}$ such that
	\[\hat{n}\leq 2\bar{n},~~\hat{m}\leq \bar{m}+\bar{n},~~ \nnz(\hat{\AA})\leq 4\nnz(\bar{\AA}),~~ \hat{R}=2\bar{R},\]
	\[X(\hat{\AA},\hat{\bb})=X(\bar{\AA},\bar{\bb}),\]
	\[\epsilon^{1le}=\frac{\eps^{2le}}{\bar{n}+1}.\]
	If the \textsc{2-len} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2)$ has a solution, then the \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$ has a solution.
	Furthermore, if $\hat{\xx}$ is a solution to the \textsc{1-lena} instance, then in time $O(\bar{n})$, we can compute a solution $\bar{\xx}$ to the \textsc{2-lena} instance.
	%	Given a \textsc{2-lena} instance $(\bar{\AA},\bar{\bb},\bar{R}, 2,\boldsymbol{\epsilon}^{2le}), \bar{\AA}\in\Z^{\bar{m}\times\bar{n}}$, such that 
	%	\[\boldsymbol{\epsilon}^{2le}(i)=\epsilon_1^{2le}\norm{\bar{\aa}_i}_1+\epsilon_2^{2le}\bar{\bb}(i)+\epsilon_3^{2le},\]
	%	we can compute a \textsc{1-lena} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1,\boldsymbol{\epsilon}^{1le}), \hat{\AA}\in\Z^{\hat{m}\times\hat{n}}$, such that
	%	\[\boldsymbol{\epsilon}^{1le}(i)=\epsilon_1^{1le}\norm{\hat{\aa}_i}_1+\epsilon_2^{1le}\hat{\bb}(i)+\epsilon_3^{1le},\]
	%	in time $O(\nnz(\bar{\AA}))$, with 
	%	\[\hat{n}\leq 2\bar{n},~~\hat{m}\leq \bar{m}+\bar{n},~~ \nnz(\hat{\AA})\leq 4\nnz(\bar{\AA}),~~ \hat{R}=2\bar{R},\]
	%	and 
	%	\begin{align*}
	%		\epsilon^{1le}_1&=\min\left\{\epsilon^{2le}_1, \frac{\epsilon^{2le}_3}{4\bar{n}}\right\},\\
	%		\epsilon^{1le}_2&=\epsilon^{2le}_2,\\
	%		\epsilon^{1le}_3&=\frac{\epsilon^{2le}_3}{4\bar{n}}.
	%	\end{align*}
	%	If $\hat{\xx}$ solves the \textsc{1-lena} instance, then in time $O(\bar{n})$, we can compute $\bar{\xx}$ that solves the \textsc{2-lena} instance.
\end{lemma}	

\begin{proof}	
	%		To conduct the error analysis, we first deal with these two cases separately, and then we combine these two cases.
	%		
	%		\paragraph{Case 1.} We first deal with the occurrence of the variable $\bar{\xx}(j)$ with coefficients $\bar{\AA}(i,j)=\pm2$. 
	Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: 2len-1len} also apply here, including the reduction time, problem size, and that \textsc{1len} has a feasible solution when \textsc{2len} has one. 
	It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{1-lena} back to an approximate solution to \textsc{2-lena}.
	
	Based on the solution mapping method described above, it takes constant time to set the value of each entry of $\bar{\xx}$ by computing an averaging or mapping back trivially, and the size of $\bar{\xx}$ is $\bar{n}$, thus the solution mapping takes $O(\bar{n})$ time.
	
	Now, we conduct the error analysis. By Definition \ref{def: klena-new}, the error of each linear equation in \textsc{1-lena} can be bounded by $\epsilon^{1le}$. For a single occurrence of $\bar{\AA}(i,j)=\pm2$, we first bound the error of the equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$, and obtain
	\[|\bar{\xx}(j)-\bar{\xx}'(j)|\leq \epsilon^{1le},\]
	hence, we have
	\begin{equation*}
		\label{eq: 2LEN}
		-\epsilon^{1le}\leq \bar{\xx}(j)-\bar{\xx}'(j)\leq \epsilon^{1le},
	\end{equation*}
	and thus
	\begin{equation}
		\label{eq: 2LEN1}
		-\epsilon^{1le}+2\bar{\xx}(j)\leq \bar{\xx}(j)+\bar{\xx}'(j)\leq \epsilon^{1le}+2\bar{\xx}(j).
	\end{equation}		
	We first consider the case that, in the equation $\bar{\aa}_i^\top\bar{\xx}=\bar{\bb}(i)$, there is only one entry $j$ such that $\bar{\aa}_i(j)=\pm2$. By separating this term, we can write
	\[\bar{\aa}_i^\top\bar{\xx}=\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)\pm2\bar{\xx}(j), \qquad \hat{\aa}_i^\top\hat{\xx}=\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)\pm(\bar{\xx}(j)+\bar{\xx}'(j)).\] 
	Adding $\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)$ to Eq, \eqref{eq: 2LEN1}, we have
	\begin{small}
		\begin{equation*}
			\label{eq: 2LEN2}
			-\epsilon^{1le}\underbrace{\pm2\bar{\xx}(j)+\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)}_{\bar{\aa}_i^\top\bar{\xx}}\leq \underbrace{\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)\pm(\bar{\xx}(j)+\bar{\xx}'(j))}_{\hat{\aa}_i^\top\hat{\xx}} \leq \epsilon^{1le}\underbrace{\pm2\bar{\xx}(j)+\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)}_{\bar{\aa}_i^\top\bar{\xx}}.
		\end{equation*}
	\end{small}	
	And since $\hat{\bb}(i)=\bar{\bb}(i)$, we can subtract it from all parts and get
	\begin{equation*}
		\label{eq: 2LEN3}
		-\epsilon^{1le}+\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)\leq \hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i) \leq \epsilon^{1le}+\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i).
	\end{equation*}
	which can be further transformed to
	\begin{equation}
		\label{eq: 2LEN4}
		-\epsilon^{1le}+\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)\leq \bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)\leq \hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)+ \epsilon^{1le}.
	\end{equation}
	If there are $k_i$ occurrence of $\bar{\AA}(i,j)=\pm2$, then we can generalize Eq. \eqref{eq: 2LEN4} to
	\begin{equation}
		\label{eq: 2LEN4.5}
		-k_i\epsilon^{1le}+\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)\leq \bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)\leq \hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)+ k_i\epsilon^{1le},
	\end{equation}
	hence, we can bound
	\begin{equation}
		\label{eq: 2LEN5}
		\begin{aligned}
			\abs{\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)}&\leq k_i\epsilon^{1le}+\abs{\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)}\\
			&\leq (k_i+1)\epsilon^{1le},
		\end{aligned}
	\end{equation}	
	where the last inequality is because $\abs{\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)}\leq \epsilon^{1le}$ by applying the error of the \textsc{1-lena} instance.
	
	To bound all the linear equations in \textsc{2-lena} uniformly, we have
	\begin{equation*}
		\label{eq: 2LEN8}
		\begin{aligned}
			\tau^{2le}&=\max_{i\in[\bar{m}]}\abs{\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)}\\
			&\leq  \max_{i\in[\bar{m}]}(k_i+1)\epsilon^{1le} && \text{Because of Eq. \eqref{eq: 2LEN5}}\\
			&\leq (\bar{n}+1)\epsilon^{1le} && \text{Because $k_i\leq \bar{n}$}
		\end{aligned}			
	\end{equation*}
	As we set in the reduction that $\epsilon^{1le}=\frac{\eps^{2le}}{\bar{n}+1}$, then we have
	\begin{align*}
		\tau^{2le}\leq (\bar{n}+1)\frac{\eps^{2le}}{\bar{n}+1}=\eps^{2le},
	\end{align*}
	which indicates that $\bar{\xx}$ is a solution to the \textsc{2-lena} instance.
	
	%		Now, we conduct the error analysis. For a single occurrence of $\bar{\AA}(i,j)=\pm2$, we first apply the error of the \textsc{1-lena} solver to the equation $\bar{\xx}(j)-\bar{\xx}'(j)=0$, and obtain
	%		\[|\bar{\xx}(j)-\bar{\xx}'(j)|\leq 2\epsilon_1^{1le}+\epsilon^{1le}_3,\]
	%		hence,
	%		\begin{equation*}
	%			\label{eq: 2LEN}
	%			-2\epsilon_1^{1le}-\epsilon^{1le}_3\leq \bar{\xx}(j)-\bar{\xx}'(j)\leq 2\epsilon_1^{1le}+\epsilon^{1le}_3.
	%		\end{equation*}
	%		Then, by adding some extra terms to each part simultaneously, we can get
	%		\begin{equation*}
	%			\label{eq: 2LEN1}
	%			-2\epsilon_1^{1le}-\epsilon^{1le}_3+2\bar{\xx}(j)\leq \bar{\xx}(j)+\bar{\xx}'(j)\leq 2\epsilon_1^{1le}+\epsilon^{1le}_3+2\bar{\xx}(j),
	%		\end{equation*}	
	%		\begin{footnotesize}
	%		\begin{equation*}
	%			\label{eq: 2LEN2}
	%			-2\epsilon_1^{1le}-\epsilon^{1le}_3\pm2\bar{\xx}(j)+\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)\leq \sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)\pm(\bar{\xx}(j)+\bar{\xx}'(j)) \leq 2\epsilon_1^{1le}+\epsilon^{1le}_3\pm2\bar{\xx}(j)+\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k).
	%		\end{equation*}
	%		\end{footnotesize}
	%
	%		Let $\bar{\aa}_i^\top$ denote the $i$th row of $\bar{\AA}$, and $\hat{\aa}_i^\top$ denote the $i$th row of $\hat{\AA}$, we have $\hat{\aa}_i^\top\hat{\xx}=\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)\pm(\bar{\xx}(j)+\bar{\xx}'(j))$ and $\bar{\aa}_i^\top\bar{\xx}=\sum_{k\neq j}\bar{\AA}(i,k)\bar{\xx}(k)\pm2\bar{\xx}(j)$. Then the above inequality can be simplified as
	%		\begin{equation*}
	%			\label{eq: 2LEN2.5}
	%			-2\epsilon_1^{1le}-\epsilon^{1le}_3+\bar{\aa}_i^\top\bar{\xx}\leq \hat{\aa}_i^\top\hat{\xx} \leq 2\epsilon_1^{1le}+\epsilon^{1le}_3+\bar{\aa}_i^\top\bar{\xx}.
	%		\end{equation*}
	%		And since $\hat{\bb}(i)=\bar{\bb}(i)$, we can subtract it from all parts and get
	%		\begin{equation*}
	%			\label{eq: 2LEN3}
	%			-2\epsilon_1^{1le}-\epsilon^{1le}_3+\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)\leq \hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i) \leq 2\epsilon_1^{1le}+\epsilon^{1le}_3+\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i).
	%		\end{equation*}
	%		which can be further transformed to
	%		\begin{equation}
	%			\label{eq: 2LEN4}
	%			-2\epsilon_1^{1le}-\epsilon^{1le}_3+\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)\leq \bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)\leq \hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)+ 2\epsilon_1^{1le}+\epsilon^{1le}_3.
	%		\end{equation}
	%		If there are $k_i$ occurrence of $\bar{\AA}(i,j)=\pm2$, then we can generalize Eq. \eqref{eq: 2LEN4} to
	%		\begin{equation}
	%			\label{eq: 2LEN4.5}
	%			-2k_i\epsilon_1^{1le}-k_i\epsilon^{1le}_3+\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)\leq \bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)\leq \hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)+ 2k_i\epsilon_1^{1le}+k_i\epsilon^{1le}_3.
	%		\end{equation}
	%		which indicates that we can bound $\abs{\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)}$ by bounding $\abs{\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)}$.
	%		
	%		To bound $\abs{\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)}$, we then apply the error of \textsc{1-lena} solver to the corresponding equation in \textsc{1-lena} of the $i$th equation in \textsc{2-lena}, and obtain
	%		\begin{equation}
	%			\label{eq: 2LEN5}
	%			|\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)|\leq\boldsymbol{\epsilon}^{1le}(i)= \epsilon_1^{1le}\norm{\hat{\aa}_i}_1+\epsilon_2^{1le}\hat{\bb}(i)+\epsilon_3^{1le}.
	%		\end{equation}
	%		Plugging Eq. \eqref{eq: 2LEN5} to \eqref{eq: 2LEN4.5}, we obtain 
	%		\begin{equation}
	%			\label{eq: 2LEN8}
	%			|\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)|\leq  \epsilon_1^{1le}\left(2k_i+\norm{\bar{\aa}_i}_1\right)+\epsilon_2^{1le}\bar{\bb}(i)+(1+k_i)\epsilon_3^{1le}.
	%		\end{equation}
	%		where we use $\sum_{j\in[\hat{n}]}|\hat{\AA}(i,j)|=\sum_{j\in[\bar{n}]}|\bar{\AA}(i,j)|$ and $\hat{\bb}(i)=\bar{\bb}(i)$.
	%
	%		Because $k_i\leq \bar{n}$, we can set $\boldsymbol{\epsilon}^{2le}(i)$ as the error of any equation $i$ with $k_i$ coefficients of $\pm2$ by
	%		\begin{equation*}
	%			\begin{aligned}
	%				\boldsymbol{\tau}^{2le}(i)=|\bar{\aa}_i^\top\bar{\xx}-\bar{\bb}(i)| &\leq \epsilon_1^{1le}\left(2\bar{n}+\norm{\bar{\aa}_i}_1\right)+\epsilon_2^{1le}\bar{\bb}(i)+(\bar{n}+1)\epsilon_3^{1le}\\
	%				&\leq \epsilon_1^{1le}\norm{\bar{\aa}_i}_1+\epsilon_2^{1le}\bar{\bb}(i)+2\bar{n}(\epsilon^{1le}_1+\epsilon_3^{1le}) && \text{Because $\bar{n}\geq 1$} 
	%			\end{aligned}
	%		\end{equation*}
	%	As we set in the reduction that $\epsilon^{1le}_1=\min\left\{\epsilon^{2le}_1, \frac{\epsilon^{2le}_3}{4\bar{n}}\right\},
	%	\epsilon^{1le}_2=\epsilon^{2le}_2,
	%	\epsilon^{1le}_3=\frac{\epsilon^{2le}_3}{4\bar{n}}$, then we have
	%	\begin{align*}
	%		\boldsymbol{\tau}^{2le}(i)&\leq \epsilon^{2le}_1\norm{\bar{\aa}_i}_1+\epsilon^{2le}_2\bar{\bb}(i)+2\bar{n}\left(\frac{\epsilon^{2le}_3}{4\bar{n}}+\frac{\epsilon^{2le}_3}{4\bar{n}}\right)\\
	%		&=\epsilon^{2le}\norm{\bar{\aa}_i}_1+\epsilon^{2le}_2\bar{\bb}(i)+\epsilon^{2le}_3\\
	%		&=\boldsymbol{\epsilon}^{2le}(i).
	%	\end{align*}
	%	Therefore, if $\hat{\xx}$ solves the \textsc{1-lena} instance with the error $\epsilon^{1le}_1, \epsilon^{1le}_2, \epsilon^{1le}_3$ as set in the reduction, we can map it back to $\bar{\xx}$ that solves the \textsc{2-lena} instance with error $\boldsymbol{\epsilon}^{2le}$.
\end{proof}

\subsection{$1$-LEN(A) to FHF(A)}
\label{sect: 1lena-fhfa}
\subsubsection{$1$-LEN to FHF}
The following is the approach to reduce a \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$ to an \textsc{fhf} instance $(G^h, F^h, \uu^h, \calH^h, s, t)$. 
The \textsc{1-len} has the form of $\hat{\AA}\hat{\xx}=\hat{\bb}$, where $\hat{\AA}\in \Z^{\hat{m}\times\hat{n}}, \hat{\bb}\in\Z^{\hat{m}}$. For an arbitrary equation $i$ in the \textsc{1-len} instance, $\hat{\aa}_i^\top\hat{\xx}=\hat{\bb}(i), i\in[\hat{m}]$, let $J_i^{+}=\{j|\hat{\aa}_i(j)=1\}$ and $J_i^{-}=\{j|\hat{\aa}_i(j)=-1\}$ denote the set of indices of variables with coefficients being 1 and -1 in equation $i$, respectively. Then, each equation can be rewritten as a difference of the sum of variables with coefficient 1 and -1:
\begin{equation}
	\label{eq: l-u-LEN}
	\sum_{j\in J^i_+}\hat{\xx}(j) - \sum_{j\in J^i_{-}}\hat{\xx}(j) =\hat{\bb}(i), ~~ i\in[\hat{m}].
\end{equation}
We claim that $\hat{\AA}\hat{\xx}=\hat{\bb}$ can be represented by a graph that is composed of a number of homologous edges and fixed flow edges, as shown in Figure \ref{fig: homo}. 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.7\textwidth]{image/homo_new}
	\caption{The reduction from \textsc{1-len} to \textsc{fhf}.} 
	\label{fig: homo}
\end{figure}
\ming{figure caption}

%	We construct a homologous flow network that maintains the sparsity of 1-LEN and has a feasible flow if and only if Eq. \eqref{eq: l-u-LEN} has a solution.	
More specifically, the fixed homologous flow network consists of a source $s$, a sink $t$, and $\hat{m}$ sections such that each section $i$ represents the $i$th linear equation in \textsc{1-len}, as shown in Eq. \eqref{eq: l-u-LEN}.

Inside each section $i$, there are $2$ vertices $\{J_i^{-}, J_i^{+}\}$ and a number of edges:
\begin{itemize}		
	\item For incoming edges of $\{J_i^{-}, J_i^{+}\}$,
	\begin{itemize}
		\item if $\hat{\aa}_i(j)=1$, then $s$ is connected to $J_i^+$ by edge $\hat{x}_i^j$ with capacity $\hat{R}$;
		\item if $\hat{\aa}_i(j)=-1$, then $s$ is connected to $J_i^-$ by edge $\hat{x}_i^j$ with capacity $\hat{R}$;
		\item if $\hat{\aa}_i(j)=0$, no edge is needed.
	\end{itemize}
	Note that the problem sparsity is preserved in the graph construction. \ming{maybe more comments about the sparsity.}
	The amount of flow routed in these incoming edges equals to the value of the corresponding variables. To ensure the consistency of the value of variables over $\hat{m}$ equations, those incoming edges that correspond to the same variable are forced to route the same amount of flow, i.e., $(\hat{x}_1^j, \cdots, \hat{x}_{\hat{m}}^j), j\in[\hat{n}]$ constitute a homologous edge set that corresponds to the variable $\hat{\xx}(j)$. Note that the size of such a homologous edge set is at most $\hat{m}$.		
	\item For outgoing edges of $\{J_i^{-}, J_i^{+}\}$,
	\begin{itemize}
		\item $J_i^+$ is connected to $t$ by a fixed flow edge $\hat{b}_i$ that routes $\hat{\bb}(i)$ units of flow;
		\item $J_i^{+}$ and $J_i^-$ are connected to $t$ by a pair of homologous edges $e_i^{+}, e_i^{-}$ with capacity $\hat{R}$.
	\end{itemize}				
\end{itemize}

If an \textsc{fhf} solver returns $\ff^h$ for the \textsc{fhf} instance $(G^h, F^h, \uu^h, \calH^h, s, t)$, then we return $\hat{\xx}$ for the \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$, by setting 
\[\hat{\xx}(j)=\ff^h(\hat{x}^j_i), ~\text{for an arbitrary $i\in[\hat{m}]$ and for all $j\in[\hat{n}]$.}\]

\begin{lemma}[\textsc{1-len} to \textsc{fhf}]
	\label{lm: 1len-fhf}
	Given a \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$ where $\hat{\AA}\in\Z^{\hat{m}\times\hat{n}}, \hat{\bb}\in \Z^{\hat{m}}$, we 
	we can construct, in time $O(\nnz(\hat{\AA}))$, an \textsc{fhf} instance $(G^h, F^h, \uu^h, \mathcal{H}^h=(H_1, \cdots, H_h), s, t)$ such that
	\[|V^h|=2\hat{m}+2,\qquad |E^h|\leq4\nnz(\hat{\AA}),\qquad |F^h|=\hat{m},\]
	\[h=\hat{n}+\hat{m},\qquad \norm{\uu^h}_{max}=\max\left\{\hat{R}, X(\hat{\AA}, \hat{\bb})\right\},  \]
	and if the \textsc{1-len} instance has a solution, then the \textsc{fhf} instance has a solution.
%	and if $\ff^h$ is a solution to the FHF instance, then in time $O(\hat{n})$, we can compute a solution $\hat{\xx}$ to the 1-LEN instance.
\end{lemma}	
\begin{proof}
	According to the reduction described above, from any solution $\hat{\xx}$ to the \textsc{1-len} instance such that $\hat{\AA}\hat{\xx}=\hat{\bb}$, it is easy to derive a solution $\ff^h$ to the \textsc{fhf} instance. Concretely, we define a feasible flow $\ff^h$ as follows: 
	\begin{itemize}
		\item For incoming edges of $\{J_i^{-}, J_i^{+}\}$, we set
		\[\ff^h(\hat{x}^j_1)=\cdots=\ff^h(\hat{x}^j_{\hat{m}})=\hat{\xx}(j)\leq \hat{R}, \qquad \forall j\in[\hat{n}],\]
		which satisfies the homologous constraint for the homologous edge sets $(\hat{x}_1^j, \cdots, \hat{x}_{\hat{m}}^j), j\in[\hat{n}]$, as well as the capacity constraint. 
		\item For outgoing edges of $\{J_i^{-}, J_i^{+}\}$, we set
		\[\ff^h(\hat{b}_i)=\hat{\bb}(i),\qquad \forall i\in\hat{m},\]
		which satisfies the fixed flow constraint for edges $\hat{b}_1,\cdots,\hat{b}_{\hat{m}}$;
		and set
		\[\ff^h(e^+_i)=\ff^h(e^-_i)=\sum_{j\in J^i_{-}}\hat{\xx}(j)=\sum_{j\in J^i_{+}}\hat{\xx}(j)-\hat{\bb}(j),\]
		which satisfies the homologous constraint for edge $e_i^{+}, e_i^{-}$, and the conservation of flows for vertices $J_i^{+}, J_i^{-}$.
	\end{itemize}
	Therefore, we conclude that $\ff^h$ is a feasible flow to the \textsc{fhf} instance.
	%	In the other direction, given a feasible flow, it is easy to construct a solution to Eq. \eqref{eq: l-u-LEN}. Therefore, 1-LEN is satisfied if and only if there exists a feasible flow.
	 \\\\
	 Now, we track the change of problem size after reduction. Based on the reduction method, given a \textsc{1-lena} instance with $\hat{n}$ variables, $\hat{m}$ linear equations, and $\nnz(\hat{\AA})$ nonzero entries, it is straightforward to get the size of the reduced \textsc{fhfa} instance as follows.
	\begin{enumerate}
		\item $|V^h|$ vertices, where
		\[|V^h|=2\hat{m}+2.\]
		\item $|E^h|$ edges, where
		\[|E^h|=\nnz(\hat{\AA})+3\hat{m}\leq 4\nnz(\hat{\AA}),\]
		since $\hat{m}\leq \nnz(\hat{\AA})$.
		\item $|F^h|$ fixed flow edges, where
		\[|F^h|=\hat{m}.\]
		\item $h$ homologous edge sets, where
		\[h=\hat{m}+\hat{n}.\]
		\item The maximum edge capacity is bounded by 
		\[\norm{\uu^h}_{max}=\max\left\{\hat{R}, \norm{\hat{\bb}}_{max}\right\}\leq \max\left\{\hat{R}, X(\hat{\AA}, \hat{\bb})\right\}.\]
	\end{enumerate}
	
	%		\item \textbf{Reduction time}\\
	To estimate the reduction time, as there are $|V^h|=O(\hat{m})$ vertices and $|E^h|=O(\nnz(\hat{\AA}))$ edges in $G^h$, thus, performing such a reduction takes $O(\nnz(\hat{\AA}))$ time to construct $G^h$.
\end{proof}

\subsubsection{$1$-LENA to FHFA}
The above lemma shows the reduction between exactly solving a \textsc{1-len} instance and exactly solving a \textsc{fhf} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.
First of all, we give a definition of the approximate version of \textsc{fhf}.

 \begin{definition}[FHF Approximate Problem (\textsc{fhfa})]
 	\label{def: fhfa-new}
 	An \textsc{fhfa} instance is given by an \textsc{fhf} instance $\left(G, F, \uu, \mathcal{H}, s, t\right)$ as in Definition \ref{def: fhf}, and error parameters $\epsilon_l,\epsilon_u\in[0,1]$, $\epsilon_{d},\epsilon_h \geq 0$, \ming{all in $[0,1]$?}which we collect in a tuple $\left(G, F, \mathcal{H}, \uu, s,t, \epsilon_l, \epsilon_u,\epsilon_d,\epsilon_h(k)\right)$.
 	We say an algorithm solves the \textsc{fhfa} problem, if, given any \textsc{fhfa} instance, it returns a flow $\ff\geq\bf{0}$ that satisfies
 	\begin{align}
 		&(1-\epsilon_l)\uu(e)\leq \ff(e)\leq(1+\epsilon_u)\uu(e), ~ \forall e \in F \label{eqn:fhfa_error_congestion_1} \\
 		&0\leq \ff(e)\leq(1+\epsilon_u)\uu(e), ~ \forall e \in E\backslash F \label{eqn:fhfa_error_congestion_2} \\
 		& \abs{\sum_{\begin{subarray}{c}
 					u:
 					(u,v)\in E
 			\end{subarray}}\ff(u,v)-\sum_{\begin{subarray}{c}
 					w:
 					(v,w)\in E
 			\end{subarray}}\ff(v,w)}\leq \epsilon_d, ~ \forall v\in V\backslash\{s,t\}  \label{eqn:fhfa_error_demand}\\
 		& \abs{\ff(v,w)-\ff(v',w')}\leq (k-1)\epsilon_h, ~ \forall (v,w),(v',w')\in H_i,~ \abs{H_i}=k \label{eqn:fhfa_error_homology}
 	\end{align}
	or it correctly declares that the associated \textsc{fhf} instance is infeasible. We refer to the error in \eqref{eqn:fhfa_error_congestion_1} and \eqref{eqn:fhfa_error_congestion_2} as error in congestion, error in \eqref{eqn:fhfa_error_demand} as error in demand, and error in \eqref{eqn:fhfa_error_homology} as error in homology.
 \end{definition}	
\begin{remark*}
	\ming{check} Note that error in demand in \textsc{fhfa} is assumed to be additive. Error in demand for $\{s, t\}$ are not defined since it is a single commodity problem and no requirements are imposed on the flow value.
\end{remark*}	

We can use the same reduction method and solution mapping method in the exact case to reduce a \textsc{1-lena} instance to an \textsc{fhfa} instance. Note that, though we still obtain $\hat{\xx}$ by setting 
\[\hat{\xx}(j)=\ff^h(\hat{x}^i_j), \qquad \text{for an arbitrary $i\in[\hat{m}]$ and for all $j\in[\hat{n}]$},\]
the value of $\hat{\xx}(j)$ depends on which edge $\hat{x}^i_j$ is chosen in the approximate case, since we allow error in homology.
%Furthermore, if an \textsc{fhfa} solver returns $\ff^h$ for the
%\textsc{fhfa} instance $(G^h, F^h, \uu^h, \mathcal{H}^h, s,t, \epsilon^h_l, \epsilon^h_u, \epsilon^h_d, \epsilon^h_h(k))$, then we return $\hat{\xx}$ for the \textsc{1-lena} instance $(\hat{\AA}, \hat{\bb}, 1, \bar{R}, \epsilon^{1le})$, by setting:
%\[\hat{\xx}(j)=\ff^h(\hat{x}^i_j), \qquad \text{for an arbitrary $i\in[\hat{m}]$ and for all $j\in[\hat{n}]$},\]
%where $\hat{m}$ and $\hat{n}$ are the number of linear equations and variables in the \textsc{1-lena} instance, respectively. Note that, different from the exact case, the value of $\hat{\xx}(j)$ depends on which edge $\hat{x}^i_j$ is chosen.

%	Given a solution $\hat{\xx}$ to Eq. \eqref{eq: l-u-LEN}, we can define a feasible flow as follows: $\hat{\xx}(j)=\ff(\hat{x}^i_j)$, for all $i\in[\hat{m}]$ s.t. $\hat{\AA}(i,j)\neq 0$. The edges are homologous so that the value of $\hat{\xx}(j)$ stays the same in all the equations. 
%	Also, according to the flow conservation constraint and the homology of $(J^i_+, t)$ and $(J^i_{-}, t)$, we have
%	\[\ff(J^i_{-}, t)=\ff(J^i_+, t)=\sum_{j\in J^i_+}\hat{\xx}(j) - \hat{\bb}(i)=\sum_{j\in J^i_{-}}\hat{\xx}(j), ~~ i\in[\hat{m}]\]
%	



\begin{lemma}[\textsc{1-lena} to \textsc{fhfa}]
	Given a \textsc{1-lena} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1,\epsilon^{1le},)$ where $\hat{\AA}\in\Z^{\hat{m}\times\hat{n}}, \hat{\bb}\in\Z^{\hat{m}}$, we can construct, in $O(\nnz(\hat{\AA}))$ time, an \textsc{fhfa} instance $(G^h, F^h, \mathcal{H}^h=(H_1, \cdots, H_h), \uu^h, s,t, \epsilon^h_l, \epsilon^h_u, \epsilon^h_d, \epsilon^h_h)$ such that
	\[|V^h|=2\hat{m}+2,\qquad |E^h|\leq4\nnz(\hat{\AA}),\qquad |F^h|=\hat{m},\]
	\[h=\hat{n}+\hat{m},\qquad  \norm{\uu^h}_{max}=\max\left\{\hat{R}, X(\hat{\AA}, \hat{\bb})\right\}, \]
	\[\epsilon^h_l=\frac{\epsilon^{1le}}{3X(\hat{\AA}, \hat{\bb})}, \qquad
	\epsilon^h_u=\frac{\epsilon^{1le}}{3X(\hat{\AA}, \hat{\bb})},\qquad
	\epsilon^h_d=\frac{\epsilon^{1le}}{6},\qquad
	\epsilon^h_h=\frac{\epsilon^{1le}}{3\hat{n}\hat{m} X(\hat{\AA}, \hat{\bb}) }.\]
%	\begin{align*}
%		\epsilon^h_l&=\frac{\epsilon^{1le}}{3X(\hat{\AA}, \hat{\bb})}, \\
%		\epsilon^h_u&=\frac{\epsilon^{1le}}{3X(\hat{\AA}, \hat{\bb})},\\
%		\epsilon^h_d&=\frac{\epsilon^{1le}}{6},\\
%		\epsilon^h_h&=\frac{\epsilon^{1le}}{3\hat{n}\hat{m} X(\hat{\AA}, \hat{\bb}) }.
%	\end{align*}
	If the \textsc{1-len} instance $(\hat{\AA},\hat{\bb},\hat{R}, 1)$ has a solution, then the \textsc{fhf} instance $(G^h, F^h,  \mathcal{H}^h, \uu^h, s,t)$ has a solution. 
	Furthermore, if $\ff^h$ is a solution to the \textsc{fhfa} instance, then in time $O(\hat{n})$, we can compute a solution $\hat{\xx}$ to the \textsc{1-lena} instance.
	
	%	Given a \textsc{1-lena} instance $(\hat{\AA},\hat{\bb},1,\boldsymbol{\epsilon}^{1le}), \hat{\AA}\in\Z^{\hat{m}\times\hat{n}}$, it can be reduced to a \textsc{fhfa} instance $(G^h, \ll^h, \uu^h, h=h_m+h_p, H=H_m\cup H_p=\left\{\bigcup_{i\in[h_m]}  g^m_i\right\}\cup \left\{\bigcup_{i\in[h_p]}  g^p_i\right\}, R, \epsilon^h_l, \epsilon^h_u, \epsilon^h_d, \epsilon^h_h(k))$ in $O(\nnz(\hat{\AA}))$ time, such that $G^h$ has $|V^h|=O(\hat{m})$ vertices, $|E^h|=O(\nnz(\hat{\AA}))$ edges, which includes
	%	\begin{itemize}
	%		\item $h_m=\hat{n}$ multi-homologous edge sets;
	%		\item $h_p=\hat{m}$ pairwise homologous edge sets;
	%		\item $|H_m|=\nnz(\hat{\AA})$ multi-homologous edges;
	%		\item $\max_{i\in[h_m]}g^m_i=O(\hat{m})$ is the maximum size of multi-homologous edge sets.
	%	\end{itemize}
	%	Suppose there is a \textsc{fhfa} solver with 
	%	\begin{itemize}
	%		\item $((1-\epsilon_l^h)\ll^h,(1+\epsilon_u^h)\uu^h)$ error in congestion;
	%		\item $\epsilon^h_{d}$ error in demand;
	%		\item $\epsilon^h_h(k)$ error in homology.
	%	\end{itemize}
	%	Then it can be translated into a \textsc{1-lena} solver with error
	%	\[\boldsymbol{\epsilon}^{1le}(i)=\epsilon_1^{1le}\norm{\hat{\aa}_i}_1+\epsilon_2^{1le}\hat{\bb}(i)+\epsilon_3^{1le},\]
	%	where $\epsilon^{1le}_1=(\hat{m}-1)\epsilon^h_h,  \epsilon^{1le}_2=\max\{\epsilon_l^h, \epsilon_u^h\},  \epsilon^{1le}_3=2\epsilon_d^h+\epsilon^h_h$. 
\end{lemma}	
\begin{proof}
	Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: 1len-fhf} also apply here, including the reduction time, problem size, and that \textsc{fhf} has a feasible solution when \textsc{1-len} has one. 
	It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{fhfa} back to an approximate solution to \textsc{1-lena}.
	
	Based on the solution mapping method described above, it takes constant time to set the value of each entry of $\hat{\xx}$ as $\ff^h$ on certain edges. As $\hat{\xx}$ has $\hat{n}$ entries, such a solution mapping takes $O(\hat{n})$ time.		
	
	Now, we conduct error analysis. Let $\hat{\xx}_i(j)=\ff^h(\hat{x}^j_i)$ denote the amount of flow routed through in the $i$th section of $G^h$. We firstly investigate the error in the $i$th linear equation in the \textsc{1-lena} instance $\hat{\aa}_i^\top\hat{\xx}=\hat{\bb}(i)$.
	For each edge $\hat{x}_i^j$ in the $i$th section of $G^h$, by error in homology defined in Eq. \eqref{eqn:fhfa_error_homology}, we have
	\[\abs{\hat{\xx}(j)-\hat{\xx}_i(j)}\leq (\hat{m}-1)\epsilon^h_h,\qquad \forall j\in[\hat{n}]\]
	because the homologous edge set corresponding to the variable $\hat{\xx}(j)$ has size at most $\hat{m}$. Thus, we can bound $|\hat{\aa}_i^\top\hat{\xx}-\hat{\aa}_i^\top\hat{\xx}_i|$ by
	\begin{equation}
		\label{eq: LEN1}
		\begin{aligned}
			|\hat{\aa}_i^\top\hat{\xx}-\hat{\aa}_i^\top\hat{\xx}_i|=|\hat{\aa}_i^\top(\hat{\xx}-\hat{\xx}_i)|\leq (\hat{m}-1)\epsilon^h_h|\hat{\aa}_i^\top\vecone|=(\hat{m}-1)\epsilon^h_h\norm{\hat{\aa}_i}_1.
		\end{aligned}
	\end{equation}	
	Moreover, we use $\ff^h(s, J_i^{\pm})$ to denote the total incoming flow of vertex $J_i^{\pm}$. Then, we have 
	\begin{itemize}
		\item $\ff^h(\hat{b}_i)\in\left[(1-\epsilon_l^h)\hat{\bb}(i),(1+\epsilon_u^h)\hat{\bb}(i)\right]$ because of error in congestion of fixed flow edges; 
		\item $\abs{\ff^h(s,J_i^{+})-(\ff^h(e_i^{+})+\ff^h(\hat{b}_i))}\leq \epsilon_{d}^{h}$ because of error in demand of vertex $J_i^+$;
		\item $\abs{\ff^h(s,J_i^{-})-\ff^h(e_i^-)}\leq \epsilon_{d}^{h}$ because of error in demand of vertex $J_i^-$;
		\item $|\ff^h(e_i^+)-\ff^h(e_i^-)|\leq (2-1)\epsilon^h_h=\epsilon^h_h$ because of error in homology between edge $e_i^+, e_i^-$.
	\end{itemize}
	Putting the above inequalities together,  and with the fact that
	\[\hat{\aa}_i^\top\hat{\xx}_i = \ff^h(s,J_i^{+})-\ff^h(s,J_i^{-}),\]
	%	\[|J^i_+|+|J^i_-|=\sum_{j\in[\hat{n}]}|\hat{\AA}(i,j)|,\]
	we have
	\[-2\epsilon_{d}^{h}-\epsilon^h_h-\epsilon_l^h\cdot\hat{\bb}(i)\leq\hat{\aa}_i^\top\hat{\xx}_i-\hat{\bb}(i)\leq 2\epsilon_{d}^{h}+\epsilon^h_h+\epsilon_u^h\cdot\hat{\bb}(i).\]
	Combining with Eq. \eqref{eq: LEN1}, we have
	\begin{align*}
		|\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)|&=|\hat{\aa}_i^\top\hat{\xx}-\hat{\aa}_i^\top\hat{\xx}_i+\hat{\aa}_i^\top\hat{\xx}_i-\hat{\bb}(i)|\\
		&\leq |\hat{\aa}_i^\top\hat{\xx}-\hat{\aa}_i^\top\hat{\xx}_i|+|\hat{\aa}_i^\top\hat{\xx}_i-\hat{\bb}(i)|\\
		&\leq  (\hat{m}-1)\epsilon^h_h\norm{\hat{\aa}_i}_1+\max\{\epsilon_l^h, \epsilon_u^h\}\hat{\bb}(i)+2\epsilon_d^h+\epsilon^h_h.
	\end{align*}
	To bound all the linear equations in \textsc{1-lena} uniformly, we have
	\begin{align*}
		\tau^{1le}&=\max_{i\in[\hat{m}]} |\hat{\aa}_i^\top\hat{\xx}-\hat{\bb}(i)|\\
		&\leq \max_{i\in[\hat{m}]}\left\{(\hat{m}-1)\epsilon^h_h\norm{\hat{\aa}_i}_1+\max\{\epsilon_l^h, \epsilon_u^h\}\hat{\bb}(i)+2\epsilon_d^h+\epsilon^h_h\right\}\\
		&\leq (\hat{m}-1)\epsilon^h_h \cdot \hat{n}X(\hat{\AA})+\max\{\epsilon_l^h, \epsilon_u^h\} X(\hat{\bb})+2\epsilon_d^h+\epsilon^h_h\\
		&\leq (\hat{m}-1)\epsilon^h_h \cdot \hat{n}X(\hat{\AA}, \hat{\bb})+\max\{\epsilon_l^h, \epsilon_u^h\} X(\hat{\AA}, \hat{\bb})+2\epsilon_d^h+\epsilon^h_h\\
		&\leq \epsilon^h_h\cdot\hat{n}\hat{m} X(\hat{\AA}, \hat{\bb})+\max\{\epsilon_l^h, \epsilon_u^h\} X(\hat{\AA}, \hat{\bb})+2\epsilon_d^h. && \text{Because $\hat{n}, X(\hat{\AA}, \hat{\bb})\geq 1$}
	\end{align*}	
	
	As we set in the reduction that $\epsilon^h_l=\frac{\epsilon^{1le}}{3X(\hat{\AA}, \hat{\bb})}, 
	\epsilon^h_u=\frac{\epsilon^{1le}}{3X(\hat{\AA}, \hat{\bb})},
	\epsilon^h_d=\frac{\epsilon^{1le}}{6},
	\epsilon^h_h=\frac{\epsilon^{1le}}{3\hat{n}\hat{m} X(\hat{\AA}, \hat{\bb}) }$, then we have
	\begin{align*}
		\tau^{1le}&\leq \frac{\epsilon^{1le}}{3\hat{n}\hat{m} X(\hat{\AA}, \hat{\bb}) }\cdot\hat{n}\hat{m} X(\hat{\AA}, \hat{\bb})+\frac{\epsilon^{1le}}{3X(\hat{\AA}, \hat{\bb})} \cdot X(\hat{\AA}, \hat{\bb})+2\cdot \frac{\epsilon^{1le}}{6}\\
		&=\frac{\epsilon^{1le}}{3}+\frac{\epsilon^{1le}}{3}+\frac{\epsilon^{1le}}{3}
		=\epsilon^{1le},
	\end{align*}
	which indicates that $\hat{\xx}$ is a solution to the \textsc{1-lena} instance.
\end{proof}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> proofs_flows.tex <==
%!TEX root = main.tex

\subsection{FHF(A) to FPHF(A)}
\label{sect: fhfa-fphfa}
\subsubsection{FHF to FPHF}
We show the reduction from an \textsc{fhf} instance $(G^h, H^h, \mathcal{H}^h, \uu^h,  s,t)$ to an \textsc{fphf} instance $(G^p, F^p, \mathcal{H}^p, \uu^p, s,t)$. 
Assume that $(v_1, w_1),\cdots, (v_k,w_k) \in E^h$ belong to a homologous edge set of size $k$ in $G^h$. As shown in Figure \ref{fig: h-ph}, we replace $(v_i,w_i), i\in\{2, \cdots, k-1\}$ by two edges $(v_i, z_i)$ and $(z_i, w_i)$ such that $z_i$ is a new vertex incident only to these two edges, and edge capacities of the two new edges are the same as that of the original edge $(v_i,w_i)$. Then, we can construct $k-1$ pairs of homologous edges: $(v_1,w_1)$ and $(v_2,z_2)$; $(z_2, w_2)$ and $(v_3,z_3)$; $\cdots$; $(z_i, w_i)$ and $(v_{i+1},z_{i+1})$; $\cdots$; $(z_{k-1}, w_{k-1})$ and $(v_k,w_k)$.
In addition, no reduction is performed on non-homologous edges in $G^h$, and we trivially copy these edges to $G^p$.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{image/h-ph}
	\caption{The reduction from \textsc{fhf} to \textsc{fphf}.} 
	\label{fig: h-ph}
\end{figure}

If an \textsc{fphf} solver returns $\ff^p$ for the \textsc{pfhf} instance $(G^p, F^p,  \mathcal{H}^p, \uu^p,s,t)$, then we return $\ff^h$ for the \textsc{fhf} instance $(G^h, H^h, \mathcal{H}^h,\uu^h,  s,t)$, by setting $\ff^h(e)=\ff^p(e_1)$ if $e$ is homologous and gets split into two edges $e_1, e_2$ such that $e_1$ precedes $e_2$. Moreover, we map back trivially for the rest edges. \ming{need rephrasing}

\begin{lemma}[\textsc{fhf} to \textsc{fphf}]
	\label{lm: fhf-fphf}
	Given an \textsc{fhf} instance $(G^h, F^h, \mathcal{H}^h=(H_1, \cdots, H_h), \uu^h, s, t)$,
	we can construct, in time $O(|E^h|)$, an \textsc{fphf} instance $(G^p, F^p,  \mathcal{H}^p=(H_1, \cdots, H_p), \uu^p,s, t)$ such that
	\[|V^{p}|\leq|V^h|+|E^h|, \qquad |E^{p}|\leq2|E^h|, \qquad |F^p|=|F^h|, \qquad p \leq |E^h|, \qquad \norm{\uu^p}_{max}=\norm{\uu^h}_{max},\]
	and if the \textsc{fhf} instance has a solution, then the \textsc{fphf} instance has a solution.
	%	and if $\ff^h$ is a solution to the FHF instance, then in time $O(\hat{n})$, we can compute a solution $\hat{\xx}$ to the 1-LEN instance.
\end{lemma}	
\begin{proof}
	According to the reduction described above, from any solution $\ff^h$ to the \textsc{fhf} instance, it is easy to derive a solution $\ff^p$ to the \textsc{fphf} instance. Concretely, for any homologous edge $e\in E^h$ that is split into two edges $e_1, e_2\in E^p$, we set
	\[\ff^p(e_1)=\ff^p(e_2)=\ff^h(e).\]
	Since the vertex between $e_1$ and $e_2$ is only incident to these two edges, then the conservation of flows is satisfied on the inserted vertices. Moreover, since the edge capacity of $e_1$ and $e_2$ are the same as that of $e$, and they route the same amount of flows, thus the capacity constraint is also satisfied on the split edges. In addition, conservation of flows and capacity constraints are trivially satisfies for the rest vertices and edges. Therefore, $\ff^p$ is a feasible flow to the \textsc{fphf} instance.
	\\\\
	Now, we track the change of problem size after reduction. Based on the reduction method, given an \textsc{fhf} instance with $|V^h|$ vertices, $|E^h|$ edges (including $|H^h|$ fixed flow edges, and $h$ homologous edge sets $\mathcal{H}^h=\{H_1, \cdots, H_h\}$), we can compute the size of the reduced \textsc{fphfa} instance as follows.
	\begin{enumerate}
		\item $|V^{p}|$ vertices. Since all vertices in $V^h$ are maintained, and for each homologous edge set $H_i\in \mathcal{H}^h$, $|H_i|-2$ new vertices are inserted, thus we have
		\begin{align*}
			|V^{p}|&= |V^h|+\sum_{i\in[h]}(|H_i|-2)\\
%			&=|V^h|+|E^h|-|H^h|-2h  &&\text{Because $|E^h|=|H^h|+\sum_{i\in[h]}|H_i|$}\\
			&\leq |V^h|+|E^h|. &&\text{Because $\sum_{i\in[h]}|H_i|\leq |E^h|$}
		\end{align*}
		
		\item $|E^{p}|$ edges. Since all edges in $E^h$ are maintained and a new edge is generated by inserting a new vertex, thus we have
		\[|E^{p}|= |E^h|+\sum_{i\in[h]}(|H_i|-2)\leq 2|E^h|.\]
		
		\item $|F^p|$ fixed flow edges, where
		\[|F^p|=|F^h|.\]
		It is because all fixed flow edges in $F^h$ are maintained, and no new fixed flow edges are generated by reduction of this step.
		
		\item $p$ pairs of homologous edges. Since each homologous edge set $H_i\in\mathcal{H}^h$ can be transformed into $|H_i|-1$ pairs, then we have
		\[p=\sum_{i\in[h]}(|H_i|-1)\leq |E^h|.\]		
		
		\item The maximum edge capacity is bounded by
		\[\norm{\uu^p}_{max}=\norm{\uu^h}_{max},\]
		because the reduction of this step only separate edges by inserting new vertices without modifying edge capacities.		
	\end{enumerate}
 	To estimate the reduction time, inserting a new vertex takes a constant time and there are $O(|E^h|)$ new vertices to be inserted. Also, it takes constant time to copy each of the rest $O(|E^h|)$ non-homologous edges. Hence, the reduction of this step takes $O(|E^h|)$ time. 
\end{proof}	

\subsubsection{FHFA to FPHFA}
The above lemma shows the reduction between exactly solving an \textsc{fhf} instance and exactly solving an \textsc{fphf} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.
First of all, we give a definition of the approximate version of \textsc{fphf}.

\begin{definition}[FPHF Approximate Problem (\textsc{fphfa})]
	\label{def: fphfa-new}
	An \textsc{fphfa} instance is given by an \textsc{fphf} instance $\left(G, F,  \mathcal{H}=\{H_1, \cdots, H_p\}, \uu,s, t\right)$ as in Definition \ref{def: fphf}, and error parameters $\epsilon_l,\epsilon_u\in[0,1]$, $\epsilon_{d},\epsilon_h \geq 0$, which we collect in a tuple $\left(G, F, \mathcal{H}, \uu, s,t, \epsilon_l, \epsilon_u,\epsilon_d,\epsilon_h\right)$.
	We say an algorithm solves the \textsc{fphfa} problem, if, given any \textsc{fphfa} instance, it returns a flow $\ff\geq\bf{0}$ that satisfies
	\begin{align}
		&(1-\epsilon_l)\uu(e)\leq \ff(e)\leq(1+\epsilon_u)\uu(e), ~ \forall e \in F \label{eqn:fphfa_error_congestion_1} \\
		&0\leq \ff(e)\leq(1+\epsilon_u)\uu(e), ~ \forall e \in E\backslash F \label{eqn:fphfa_error_congestion_2} \\
		& \abs{\sum_{\begin{subarray}{c}
					u:
					(u,v)\in E
			\end{subarray}}\ff(u,v)-\sum_{\begin{subarray}{c}
					w:
					(v,w)\in E
			\end{subarray}}\ff(v,w)}\leq \epsilon_d, ~ \forall v\in V\backslash\{s,t\}  \label{eqn:fphfa_error_demand}\\
		& \abs{\ff(v,w)-\ff(y,z)}\leq \epsilon_h, ~ \forall H_i \ni (v,w), (y,z), i\in [p] \label{eqn:fphfa_error_homology}
	\end{align}
	or it correctly declares that the associated \textsc{fphf} instance is infeasible. We refer to the error in \eqref{eqn:fphfa_error_congestion_1} and \eqref{eqn:fphfa_error_congestion_2} as error in congestion, error in \eqref{eqn:fphfa_error_demand} as error in demand, and error in \eqref{eqn:fphfa_error_homology} as error in pair homology.
\end{definition}	

We can use the same reduction and solution mapping method in the exact case to the approximate case.
%reduce an \textsc{fhfa} instance to an \textsc{fphfa} instance. Furthermore, we use the same solution mapping method to map $\ff^p$ returned by an \textsc{fphfa} solver back to a solution of the \textsc{fhfa} instance.


\begin{lemma}[\textsc{fhfa} to \textsc{fphfa}]
	\label{lm: fhfa-fphfa}
	Given an \textsc{fhfa} instance $(G^h, F^h, \mathcal{H}^h=(H_1,\cdots, H_h),\uu^h, s,t, \epsilon^h_l, \epsilon^h_u, \epsilon^h_d, \epsilon^h_h)$, we can construct, in $O(|E^h|)$ time, an \textsc{fphfa} instance $(G^{p}, F^{p},\mathcal{H}^p=(H_1, \cdots, H_p), \uu^{p}, s,t, \epsilon^{p}_l, \epsilon^{p}_u, \epsilon^{p}_d, \epsilon^{p}_h)$ such that
	\[|V^{p}|\leq|V^h|+|E^h|, \qquad |E^{p}|\leq2|E^h|, \qquad |F^p|=|F^h|,\qquad p \leq |E^h|, \qquad \norm{\uu^p}_{max}=\norm{\uu^h}_{max},\]
	and
	\[\epsilon^p_l=\epsilon^h_l,\qquad
	\epsilon^p_u=\epsilon^h_u,\qquad
	\epsilon^p_d=\frac{\epsilon^h_d}{|E^h|},\qquad
	\epsilon^p_h=\epsilon^h_h.\]
%	\begin{align*}
%		\epsilon^p_l&=\epsilon^h_l,\\
%		\epsilon^p_u&=\epsilon^h_u,\\
%		\epsilon^p_d&=\frac{\epsilon^h_d}{|E^h|},\\
%		\epsilon^p_h&=\epsilon^h_h.
%	\end{align*}	
	If the \textsc{fhf} instance $(G^h, H^h, \mathcal{H}^h,\uu^h, s,t)$ has a solution, then the \textsc{fpfh} instance $(G^{p}, F^{p},\mathcal{H}^p, \uu^{p}, s,t)$ has a solution.
	Furthermore, if $\ff^p$ is a solution to the \textsc{fphfa} instance, then in time $O(\abs{E^h})$, we can compute a solution $\ff^h$ to the \textsc{fhfa} instance.
	
%	Given a \textsc{fhfa} instance $(G^h, \ll^h, \uu^h, h=h_m+h_p, H=H_m\cup H_p=\left\{\bigcup_{i\in[h_m]}  g^m_i\right\}\cup \left\{\bigcup_{i\in[h_p]}  g^p_i\right\}, R, \epsilon^h_l, \epsilon^h_u, \epsilon^h_d, \epsilon^h_h(k))$, with $|V^h|$ vertices and $|E^h|$ edges,
%%	including $h=\sum_{k>2}\abs{H_k}$ multi-homologous edges that are divided into $q_{k}$ sets, and $q_2$ sets of pairwise homologous edges),	
%	it can be reduced to a \textsc{fphfa} instance $(G^{p}, \ll^{p},\uu^{p}, p, P=\bigcup_{i\in[p]}  g_i, R, \epsilon^{p}_l, \epsilon^{p}_u, \epsilon^{p}_d, \epsilon^{p})$ in $O(\abs{H_m})$ time, such that $G^{p}$ has $|V^{p}|=O(|V^h|+\abs{H_m})$ vertices, $|E^{p}|=O(|E^h|+\abs{H_m})$ edges, and $p=O(\abs{H_m}+h_p)$ pairs of homologous edges.
%	Suppose there is a \textsc{fphfa} solver with
%	\begin{itemize}
%		\item $((1-\epsilon_l^{p})\ll^p,(1+\epsilon_u^{p})\uu^p)$ error in congestion;
%		\item $\epsilon^{p}_{d}$ error in demand;
%		\item $\epsilon^{p}$ error in pairwise homology.
%	\end{itemize}
%	Then it can be translated into a homologous flow solver with
%	\begin{itemize}
%		\item $((1-\epsilon_l^h)\ll^h,(1+\epsilon_u^h)\uu^h)$ error in congestion, where
%		\[\epsilon_l^{h}=\epsilon_l^{p},\qquad \epsilon_u^{h}=\epsilon_u^{p};\]
%		\item $\epsilon^h_{d}$ error in demand, where
%		\[\epsilon^{h}_d=2\epsilon^{p}_d;\]
%		\item $\epsilon^h_h(k)$ error in homology, where
%		\[\epsilon^h_h(k)=(k-1)\epsilon^{p}_h. \]
%	\end{itemize}
\end{lemma}	
\begin{proof}
		Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: fhf-fphf} also apply here, including the reduction time, problem size, and that \textsc{fphf} has a feasible solution when \textsc{fhf} has one. 
		It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{fphfa} back to an approximate solution to \textsc{fhfa}.
		
		Based on the solution mapping method described above, it takes constant time to set the value of each homologous or non-homologous entry of $\ff^h$, and $\ff^h$ has $|E^h|$ entries, such a solution mapping takes $O(|E^h|)$ time.		

%		Given a solution $\ff^p$ returned by the \textsc{fphfa} solver, we map the solution back to $G^h$ by setting $\ff^h(e)=\ff^p(e_1)$ if $e$ is homologous and gets split. We trivially map back the rest edges. As there are $|E^h|$ entries to set value, mapping $\ff^p$ back to $\ff^h$ takes $O(|E^h|)$ time.
		
		Now, we conduct error analysis. We claim that the mapping will generate three types of error: (1) error in congestion; (2) error in demand; (3) error in homology.
%		According to Def. \ref{def: fhf}, fixed flow edges and homologous edges are disjoint, thus $\ll(e)=0, \forall e\in H_i\in\mathcal{H}^h$.
		\begin{enumerate}
			\item Error in congestion.\\
			We first track the error of the upper bound of capacity. For any homologous edge $e$, the maximum flow to be routed in $e$ is
			\[(1+\tau^h_u)\uu^h(e)=\ff^p(e_1)\leq (1+\epsilon^p_u)\uu^p(e_1)=(1+\epsilon^p_u)\uu^h(e),\]
			thus,
			\[\tau^h_u\leq \epsilon^p_u.\]
			As we set $\epsilon^p_u=\epsilon^h_u$ in the reduction, then we have
			\[\tau^h_u\leq \epsilon^h_u.\]			
			This $\tau^h_u$ also applies to fixed flow edges since no reduction is made on them. 
			
			Next, we track the error of the lower bound of capacity.
			Since only fixed flow edges have lower bound of capacity, and no reduction is made on fixed flow edges, then we obtain trivially that $\tau^h_l\leq \epsilon^p_l$. By setting $\epsilon^p_l=\epsilon^h_l$ in the reduction, we have
			\[\tau^h_l\leq \epsilon^h_l.\]
			
			\item Error in demand.\\
			For simplicity, we denote $H^h=\bigcup_{i\in[h]}H_i$ as the set of all homologous edges. By Eq. \eqref{eqn:fhfa_error_demand} in Definition \ref{def: fhfa-new}, the error in demand that we can achieve for vertices other than $s, t$ in $G^h$ is computed as 
			\ming{check}
			\begin{scriptsize}
			\begin{equation}
				\label{eq: fhfa-fphfa-d}
				\begin{aligned}
					\tau^{h}_d&=\max_{w\in V^h\backslash\{s,t\}}\abs{\sum_{(v,w)\in E^h}\ff^h(v,w)-\sum_{(w,u)\in E^h}\ff^h(w,u)}\\
					&\overset{(1)}{=} \max_{w\in V^h\backslash\{s,t\}}\abs{\left(\sum_{(v,w)\in H^h}\ff^h(v,w)+\sum_{(v,w)\in E^h\backslash H^h}\ff^h(v,w)\right)-\left(\sum_{(w,u)\in H^h}\ff^h(w,u)+\sum_{(w,u)\in E^h\backslash H^h}\ff^h(w,u)\right)}\\
					&\overset{(2)}{=} \max_{w\in V^h\backslash\{s,t\}}\abs{\left(\sum_{e=(v,w)\in H^h}\ff^p(e_1)+\sum_{(v,w)\in E^h\backslash H^h}\ff^p(v,w)\right)-\left(\sum_{e=(w,u)\in H^h}\ff^p(e_1)+\sum_{(w,u)\in E^h\backslash H^h}\ff^p(w,u)\right)}\\
					&\overset{(3)}{\leq} \epsilon_{d}^p+\max_{w\in V^h\backslash\{s,t\}}\abs{\left(\sum_{e=(v,w)\in H^h}\ff^p(e_1)+\sum_{(v,w)\in E^h\backslash H^h}\ff^p(v,w)\right)-\left(\sum_{e=(v,w)\in H^h}\ff^p(e_2)+\sum_{(v,w)\in E^h\backslash H^h}\ff^p(v,w)\right)}\\
					&=\epsilon_{d}^p+ \max_{w\in V^h\backslash\{s,t\}}\abs{\sum_{e=(v,w)\in H^h}\ff^p(e_1)-\sum_{e=(v,w)\in H^h}\ff^p(e_2)}\\
					&=\epsilon_{d}^p+ \max_{w\in V^h\backslash\{s,t\}}\abs{\sum_{e=(v,w)\in  H^h}(\ff^p(e_1)-\ff^p(e_2))}\\
					&\leq \epsilon_{d}^p+\max_{w\in V^h\backslash \{s,t\}}\sum_{e=(v,w)\in  H^h}\abs{\ff^{p}(e_1)-\ff^{p}(e_2)}\\
					& \overset{(4)}{\leq}\epsilon_{d}^p+|H^h|\epsilon_{d}^p\\
					&\overset{(5)}{\leq} |E^h|\epsilon_{d}^p. 
				\end{aligned} 
			\end{equation}
			\end{scriptsize}
			
			For step (1), we separate homologous edges from other edges that are incident to vertex $w$.
			For step (2), we apply the rule of mapping $\ff^p$ back to $\ff^h$.
			For step (3), we apply Eq. \eqref{eqn:fphfa_error_demand} in Definition \ref{def: fphfa-new} with respect to vertex $w$, so that we can replace the sum of outgoing flows of $w$ by the sum of its incoming flows with an error in demand of $G^p$ being introduced, i.e.,
			\begin{scriptsize}
				\[\abs{\left(\sum_{e=(w,u)\in H^h}\ff^p(e_1)+\sum_{(w,u)\in E^h\backslash H^h}\ff^p(w,u)\right)-\left(\sum_{e=(v,w)\in H^h}\ff^p(e_2)+\sum_{(v,w)\in E^h\backslash H^h}\ff^p(v,w)\right)}\leq \epsilon^p_{d}.\]
			\end{scriptsize}
		
			For step (4), we apply Eq. \eqref{eqn:fphfa_error_demand} again with respect to the new inserted vertex. Since the new inserted vertex is only incident to $e_1$ and $e_2$, we have
			\[\abs{\ff^p(e_1)-\ff^p(e_2)}\leq \epsilon_d^p.\]
			For step (5), we utilize $|E^h|-|H^h|\geq 1$, i.e., there are more than one non-homologous edges in $G^h$.			
			As we set in the reduction that $\epsilon^p_d=\frac{\epsilon^h_d}{|E^h|}$, then we have
			\[\tau^h_d\leq |E^h|\frac{\epsilon^h_d}{|E^h|}=\epsilon^h_d.\]
			
			\item Error in homology.\\
			By Eq. \eqref{eqn:fhfa_error_homology} in Definition \ref{def: fhfa-new}, the error in homology for a homologous edge set of size $k$ that we can achieve is computed as  
			\begin{equation}
				\label{eq: h-h}
				\begin{aligned}
					(k-1)\tau^h_h&=\max_{\begin{subarray}{c}
							e, e'\in H_i\in \mathcal{H}^h\\
							|H_i|=k
						\end{subarray}
						} \abs{\ff^h(e)-\ff^h(e')}\\
					&=\max_{\begin{subarray}{c}
							e, e'\in H_i\in \mathcal{H}^h\\
							|H_i|=k
					\end{subarray}} \abs{\ff^p(e_1)-\ff^p(e'_1)}\\
					&\leq (k-1)\epsilon^p_h.
				\end{aligned}
			\end{equation} 
			where the last inequality comes from a reverse process of telescoping such that the error in pair homology is accumulated for at most $k-1$ times, because $k-1$ pair homologous edge sets are reduced from $H_i$. 
			
			As we set in the reduction that $\epsilon^p_h=\epsilon^h_h$, then we have
			\[\tau^h_h\leq \epsilon^h_h.\]
		\end{enumerate}
		To summarize, if $\ff^p$ is a solution to the \textsc{fphfa} instance with the error $\epsilon^p_l,\epsilon^p_u,\epsilon^p_d, \epsilon^p_h$ as set in the reduction, we can map it back to a solution $\ff^h$ to the \textsc{fhfa} instance with its error target achieved.
		
%		By construction, each homologous edge in $G^h$ is separated into at most two edges by inserting a vertex, then 
%		error in congestion of $G^h$ remains the same as that of $G^p$, and error in demand of $G^h$ can be accumulated by at most 2 times than that of $G^p$.
%		Moreover, since the set of homologous edges of size $k$ in $G^h$ can be mapped into $k-1$ pairs of homologous edges in $G^p$, the additive error in homology can be accumulated by $(k-1)$ times. Therefore, the difference among these $k$ homologous edges is upper bounded by $\epsilon^h_h(k)=(k-1)\epsilon^p_h$.
		%Finally, since there are at most $n$ homologous edges that are forced to route the same amount of flow, we have $k\leq n$.
\end{proof}


\subsection{FPHF(A) to SFF(A)}
\label{sect: fphfa-sffa}
\subsubsection{FPHF to SFF}
We show the reduction from an \textsc{fphf} instance $(G^p, F^p, \mathcal{H}^p, \uu^p, s,t)$ to an \textsc{sff} instance $(G^s,F^s, S_1, S_2, \\\uu^s, s_1,t_1,s_2,t_2)$. 
Assume that $\{e,\hat{e}\}\in  \mathcal{H}^p$ is an arbitrary homologous edge set in $G^p$. As shown in Figure \ref{fig: phomo-slu2cf}, we map $\{e,\hat{e}\}$ in $G^p$ to a gadget consisting edges $\{e_1,e_2,e_3,e_4,e_5 ( \text{or}~\hat{e}_3), \hat{e}_1, \hat{e}_2,\hat{e}_4,\hat{e}_5\}$ in $G^s$. The key idea to remove the homologous requirement is by introducing a second commodity between a source-sink pair $(s_2,t_2)$. Concretely, we impose the fixed flow constraint on $(e_4, \hat{e}_4)$, the selective constraint of commodity 1 on $(e_1, e_2, \hat{e}_1,\hat{e}_2)$, and the selective constraint of commodity 2 on $(e_3, e_5 ( \text{or}~\hat{e}_3),\hat{e}_5)$. Then, there is a flow of commodity 2 that routes through the directed path $e_3\rightarrow e_4\rightarrow e_5 ( \text{or}~\hat{e}_3) \rightarrow \hat{e}_4\rightarrow \hat{e}_5$, and a flow of commodity 1 through paths $e_1 \rightarrow e_4\rightarrow e_2$ and $\hat{e}_1 \rightarrow \hat{e}_4 \rightarrow \hat{e}_2 $. The fixed flow constraint on $(e_4, \hat{e}_4)$ forces the flow of commodity 1 through the two paths to be equal, which simulate the homologous requirement for edge $e$ and $\hat{e}$.
 %thanks to the conservation of flows. 
In addition, as no reduction is performed on non-homologous edges in $G^p$, we trivially copy these edges to $G^s$, and restrict these edges to be selective for commodity 1.
\begin{figure}[t]
	\centering
	\includegraphics[width=\textwidth]{image/phomo-slu2CF}
	\caption{The reduction from \textsc{fphf} to \textsc{sff}. } 
	\label{fig: phomo-slu2cf}
\end{figure}
%\ming{explain that homologous edge and fixed flow edge are disjoint.}

If an \textsc{sff} solver returns $\ff^s$ for the \textsc{sff} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2)$, then we return $\ff^p$ for the \textsc{pfhf} instance $(G^p, F^p, \mathcal{H}^p, \uu^p, s,t)$ by the following method:
for each pair of homologous edges $e$ and $\hat{e}$, we set $\ff^p(e)=\ff^s_1(e_1), \ff^p(\hat{e})=\ff^s_1(\hat{e}_1)$; for each non-homologous edge $e'$, we set $\ff^p(e')=\ff^s_1(e')$. Note that $\ff^s$ is a two-commodity flow while $\ff^p$ is a single-commodity flow.

\begin{lemma}[\textsc{fphf} to \textsc{sff}]
	\label{lm: fphf-sff}
	Given an \textsc{fphf} instance $(G^p, F^p, \mathcal{H}^p=(H_1, \cdots, H_p),\uu^p,  s, t)$,
	we can construct, in time $O(|E^p|)$, an \textsc{sff} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2)$ such that
	\[|V^s|=|V^{p}|+4p+2,\qquad |E^s|=|E^{p}|+7p,\qquad |F^s|=|F^p|+2p, \]
	\[ |S_1|=|E^{p}|+2p,\qquad |S_2|=3p, \qquad \norm{\uu^s}_{max}=\norm{\uu^p}_{max},\]
	and if the \textsc{fphf} instance has a solution, then the \textsc{sff} instance has a solution.
	%	and if $\ff^h$ is a solution to the FHF instance, then in time $O(\hat{n})$, we can compute a solution $\hat{\xx}$ to the 1-LEN instance.
\end{lemma}	
\begin{proof}
	According to the reduction described above, from any solution $\ff^p$ to the \textsc{fphf} instance, it is easy to derive a solution $\ff^s$ to the \textsc{sff} instance. Concretely, we define a feasible flow $\ff^s$ as follows:
	\begin{itemize}
		\item For any pair of homologous edge $\{e,\hat{e}\}\in  \mathcal{H}^p$, in its corresponding gadget in $G^s$, we set
		\[\ff^s_1(e_1)=\ff^s_1(e_4)=\ff^s_1(e_2)=\ff^p(e)=\ff^p(\hat{e})=\ff^s_1(\hat{e}_1)=\ff^s_1(\hat{e}_4)=\ff^s_1(\hat{e}_2) \leq u,\]
		where $u=\uu^p(e)=\uu^p(\hat{e})$, and set
		\[\ff^s_2(e_1)=\ff^s_2(e_2)=\ff^s_2(\hat{e}_1)=\ff^s_2(\hat{e}_2)=0.\]
		It is obvious that $\ff^s$ satisfies the selective constraint and the capacity constraint on edges $e_1, e_2, \hat{e}_1,\hat{e}_2$, and satisfies conservation of flows for commodity 1 on vertices $vw, vw', yz, yz'$.
		
		Moreover, we set
		\[\ff^s_2(e_3)=\ff^s_2(e_4)=\ff^s_2(e_5)=\ff^s_2(\hat{e}_4)=\ff^s_2(\hat{e}_5)=u-\ff^p(e)\leq u,\]
		and
		\[\ff^s_1(e_3)=\ff^s_1(e_4)=\ff^s_1(e_5)=\ff^s_1(\hat{e}_4)=\ff^s_1(\hat{e}_5)=0.\]
		Then it is obvious that $\ff^s$ satisfies the selective constraint and the capacity constraint on edges $e_3, e_5, \hat{e}_5$, and satisfies the flow conservation constraint of commodity 2 on vertices $vw, vw', yz, yz'$.
		
		It remains to verify if $\ff^s$ satisfies the fixed flow constraint on edges $e_4, \hat{e}_4$. According to the above constructions, we have
		\[\ff^s(e_4)=\ff^s_1(e_4)+\ff^s_2(e_4)=\ff^p(e)+(u-\ff^p(e))=u,\]
		\[\ff^s(\hat{e}_4)=\ff^s_1(\hat{e}_4)+\ff^s_2(\hat{e}_4)=\ff^p(\hat{e})+(u-\ff^p(\hat{e}))=u.\]
		
		\item For any non-homologous edge $e'\in E^p$, we also have $e'\in E^s$ since no reduction is made on this edge, and we copy it trivially to $G^s$. We set
		\[\ff^s_1(e')=\ff^p(e') ,\qquad \ff^s_2(e')=0.\]
		Since $\ff^p$ is a feasible flow in $G^p$, it is easy to check that $\ff^s$ also satisfies the selective constraint for commodity 1 and the capacity constraint on non-homologous edges, as well as conservation of flows on vertices incident to non-homologous edges. 
	\end{itemize}
	To conclude, $\ff^s$ is a feasible flow to the \textsc{sff} instance.
	\\
	\\
	Now, we track the change of problem size after reduction. Based on the reduction method, given an \textsc{fphf} instance with $|V^p|$ vertices, $|E^p|$ edges (including $|F^p|$ fixed flow edges, and $p$ pairwise homologous edge sets $\mathcal{H}^p=\{H_1,\cdots, H_p\}$), we can compute the size of the reduced \textsc{sff} instance as follows.
	\begin{enumerate}
		\item $|V^s|$ vertices. To bound it, first, all vertices in $V^p$ are maintained. 
		Then, for each pair of homologous edges $(v,w)$ and $(y,z)$, 4 auxiliary vertices $vw, vw',yz,yz'$ are added. 
		And finally, a source-sink pair of commodity 2 $(s_2, t_2)$ is added. Therefore, we have
		\[|V^s|=|V^{p}|+4p+2.\]		
		
		\item $|E^s|$ edges. Since non-homologous edges are maintained, 
		and each pair of homologous edges is replaced by a gadget with 9 edges, thus we have
		\[|E^s|=(|E^p|-2p)+9p=|E^p|+7p.\]
		
		\item $|F^s|$ fixed flow edges. First, all fixed flow edges in $F^p$ are maintained since by Def. \ref{def: fphf}, fixed flow edges and homologous edges are disjoint, thus no reduction is made.
		Then, for each pair of homologous edges as shown in Figure \ref{fig: phomo-slu2cf}, the reduction generate 2 fixed flow edges (i.e., $e_4, \hat{e}_4$). Hence, we have
		\[|F^s|=|F^p|+2p.\]
				
		\item $|S_i|$ edges that select the $i$-th commodity. First, all non-homologous edges in $E^p$ are selective for the commodity 1.
		Then, for each pair of homologous edges as shown in Figure \ref{fig: phomo-slu2cf}, the reduction generates 4 edges selecting commodity 1 (i.e., $e_1, e_2, \hat{e}_1,\hat{e}_2$) and 3 edges selecting commodity 2 (i.e., $e_3, e_5/\hat{e}_3, \hat{e}_5$). Thus, we have
		\[|S_1|=(|E^{p}|-2p)+4p=|E^p|+2p,\qquad |S_2|=3p.\]
		%			\[|S_1|=(|E^{p}|-2p)+4p=|E^{p}|+2p,\qquad |S_2|=3p, \qquad |S_{1,2}|=2p.\]
		
		\item The maximum edge capacity is bounded by
		\[\norm{\uu^s}_{max}=\norm{\uu^p}_{max}.\]
		First, capacity of non-homologous edges is unchanged in $G^s$ since no reduction is made.
		Then, for each pair of homologous edges $\{e, \hat{e}\}$ with capacity $\uu^p(e) (=\uu^p(\hat{e}))$, the capacity of the corresponding 9 edges are either selective edges with capacity $\uu^p(e)$ or fixed flow edges with fixed flow $\uu^p(e)$.
		
	\end{enumerate}
	To estimate the reduction time, first, it takes constant time to reduce each pair of homologous edges since only a constant number of vertices and edges are added. Also, it takes constant time to copy each of the rest non-homologous edges, then the reduction of this step takes $O(|E^p|)$ time in total.
\end{proof}	

\subsubsection{FPHFA to SFFA}
The above lemma shows the reduction between exactly solving an \textsc{fphf} instance and exactly solving an \textsc{sff} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.
First of all, we give a definition of the approximate version of \textsc{sff}.


\begin{definition}[SFF Approximate Problem (\textsc{sffa})]
	\label{def: sffa-new}
	An \textsc{sffa} instance is given by an \textsc{sff} instance $(G,F, S_1, S_2, \uu, s_1,t_1,s_2,t_2)$ as in Definition \ref{def: sff}, and error parameters $\epsilon_l,\epsilon_u\in[0,1]$, $\epsilon_{d1},\epsilon_{d2}, \epsilon_{t1},\epsilon_{t2} \geq 0$, which we collect in a tuple $\left(G,F, S_1, S_2, \uu, s_1,t_1,s_2,t_2, \epsilon_l, \epsilon_u,\epsilon_{d1},\epsilon_{d2}, \epsilon_{t1},\epsilon_{t2}\right)$.
	We say an algorithm solves the \textsc{sffa} problem, if, given any \textsc{sffa} instance, it returns a pair of flows $\ff_1, \ff_2\geq\bf{0}$ (denote $\ff=\ff_1+\ff_2$) that satisfies
	\begin{align}
		&(1-\epsilon_l)\uu(e)\leq \ff_1(e)+\ff_2(e)\leq(1+\epsilon_u)\uu(e), ~~ \forall e \in F \label{eqn:sffa_error_congestion_1} \\
		&0\leq \ff_1(e)+\ff_2(e)\leq(1+\epsilon_u)\uu(e), ~~ \forall e \in E\backslash F \label{eqn:sffa_error_congestion_2} \\
		& \abs{\sum_{\begin{subarray}{c}
					u:
					(u,v)\in E
			\end{subarray}}\ff_i(u,v)-\sum_{\begin{subarray}{c}
					w:
					(v,w)\in E
			\end{subarray}}\ff_i(v,w)}\leq \epsilon_{di}, ~~ \forall v\in V\backslash \{s_i,t_i\},~ i\in\{1,2\} \label{eqn:sffa_error_demand}\\
		& \sum_{\begin{subarray}{c}
				u:
				(s_{\bar{i}}, w)\in E
		\end{subarray}}\ff_i(s_{\bar{i}}, w)=0, \sum_{\begin{subarray}{c}
				u:
				(u,t_{\bar{i}})\in E
		\end{subarray}}\ff_i(u,t_{\bar{i}})\leq \epsilon_{di}, ~~ \bar{i}=\{1,2\}\backslash i \label{eqn:sffa_error_demand_s_t}\\
		& \ff_{\bar{i}}(e) \leq \epsilon_{ti}(e), ~~ \forall e\in S_{i},~ \bar{i}=\{1,2\}\backslash i \label{eqn:sffa_error_type}
	\end{align}
	or it correctly declares that the associated \textsc{sff} instance is infeasible. We refer to the error in \eqref{eqn:sffa_error_congestion_1} and \eqref{eqn:sffa_error_congestion_2} as error in congestion, error in \eqref{eqn:sffa_error_demand} and \eqref{eqn:sffa_error_demand_s_t} as error in demand, and error in \eqref{eqn:sffa_error_type} as error in type.
\end{definition}	

We can use the same reduction and solution mapping method in the exact case to the approximate case.


\begin{lemma}[\textsc{fphfa} to \textsc{sffa}]
	\label{lm: fphfa-sffa}
	Given an \textsc{fphfa} instance $(G^{p}, F^{p},\mathcal{H}^p=(H_1, \cdots, H_p), \uu^{p},  s,t, \epsilon^{p}_l, \epsilon^{p}_u, \epsilon^{p}_d, \epsilon^{p}_h)$, we can construct, in $O(|E^p|)$ time, an \textsc{sffa} instance $\left(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2, \epsilon^s_l, \epsilon^s_u,\epsilon^s_{d1},\epsilon^s_{d2}, \epsilon^s_{t1},\epsilon^s_{t2}\right)$ such that
	\[|V^s|=|V^{p}|+4p+2,\qquad |E^s|=|E^{p}|+7p,\qquad |F^s|=|F^p|+2p, \]
	\[ |S_1|=|E^{p}|+2p,\qquad |S_2|=3p,\qquad \norm{\uu^s}_{max}=\norm{\uu^p}_{max},\]
	and
	\[\epsilon_l^s=\min\left\{\frac{\epsilon^p_l}{2},~~ \frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}\right\},\qquad
	\epsilon_u^s=\min\left\{\epsilon_u^p, ~~\frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}\right\},\]
	\[\epsilon_{d1}^s= \min\left\{\frac{\epsilon^p_d}{6|E^p|},~~ \frac{\epsilon^p_h}{10}\right\},\qquad
	\epsilon_{d2}^s= \frac{\epsilon^p_h}{10},\]
	\[\epsilon_{t1}^s= \min\left\{\frac{\epsilon^p_l}{2}, \frac{\epsilon^p_h}{10}\right\},\qquad
	\epsilon_{t2}^s= \min\left\{\frac{\epsilon^p_d}{6|E^p|}, ~~\frac{\epsilon^p_h}{10}\right\}.\]
%	\begin{align*}
%		\epsilon_l^s&=\min\left\{\frac{\epsilon^p_l}{2}, \frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}\right\},\\
%		\epsilon_u^s&=\min\left\{\epsilon_u^p, \frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}\right\},\\
%		\epsilon_{d1}^s&= \min\left\{\frac{\epsilon^p_d}{6|E^p|}, \frac{\epsilon^p_h}{10}\right\},\\
%		\epsilon_{d2}^s&= \frac{\epsilon^p_h}{10},\\
%		\epsilon_{t1}^s&= \min\left\{\frac{\epsilon^p_l}{2}, \frac{\epsilon^p_h}{10}\right\},\\
%		\epsilon_{t2}^s&= \min\left\{\frac{\epsilon^p_d}{6|E^p|}, \frac{\epsilon^p_h}{10}\right\}.
%	\end{align*}	
	If the \textsc{fphf} instance $(G^{p}, F^{p},\mathcal{H}^p,\uu^{p}, s,t)$ has a solution, then the \textsc{sff} instance $\left(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2\right)$ has a solution.
	Furthermore, if $\ff^s$ is a solution to the \textsc{sffa} instance, then in time $O(\abs{E^p})$, we can compute a solution $\ff^p$ to the \textsc{fphfa} instance.

%	Given a \textsc{fphfa} instance $(G^{p}, \ll^{p},\uu^{p}, p, P=\bigcup_{i\in[p]}  g_i , R, \epsilon^{p}_l, \epsilon^{p}_u, \epsilon^{p}_d, \epsilon^{p}_h)$, it can be reduced to a \textsc{sffa} instance $(G^s,\ll^s,\uu^s, S=S_1\cup S_2, \epsilon_l^s,\epsilon_u^s, \epsilon_{d1}^s, \epsilon_{d2}^s, \epsilon_{t1}^s,\epsilon_{t2}^s)$ in $O(p)$ time, such that $G^s$ has
%	\begin{itemize}
%		\item $|V^s|=O(|V^{p}|+p)$ vertices;
%		\item $|E^s|=O(|E^{p}|+p)$ edges, among which 
%		\begin{itemize}
%			\item $|S_1|=O(|E^{p}|+p)$ edges selecting commodity 1;
%			\item $|S_2|=O(p)$ edges selecting commodity 2.
%		%	\item $|S_{1,2}|=O(p)$ non-selective edges.
%		\end{itemize}
%	\end{itemize}
%	If there is a \textsc{sffa} solver with 
%	\begin{itemize}
%		\item $((1-\epsilon_l^s)\ll^s, (1+\epsilon_u^s)\uu^s)$ error in congestion;
%		\item $\epsilon_{di}^s, i\in\{1,2\}$ error in demand of commodity $i$;
%		\item $\epsilon_{ti}^s, i\in\{1,2\}$ error in type for edges selecting commodity $i$.
%	\end{itemize}
%	Then it can be translated into a \textsc{fphfa} solver with
%	\begin{itemize}
%		\item $((1-\epsilon_l^{p})\ll^p,(1+\epsilon_u^{p})\uu^p)$ error in congestion, where
%		\[\epsilon_l^{p}=\epsilon_l^s, \qquad \epsilon_u^{p}=\epsilon_u^s;\]
%		\item $\epsilon^{p}_{d}$ error in demand, where
%		\[\epsilon^{p}_d=O\left(|E^p|(\epsilon_{d1}^s+\epsilon_{t2}^s)\right);\]
%		\item $\epsilon^{p}$ error in pairwise homology, where
%		\[\epsilon^p_h=O\left(R(\epsilon_l^s+\epsilon_u^s)+\epsilon_{d1}^s+\epsilon_{d2}^s+\epsilon_{t1}^s+\epsilon_{t2}^s\right).\]
%	\end{itemize}
\end{lemma}	
\begin{proof}
	Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: fphf-sff} also apply here, including the reduction time, problem size, and that \textsc{sff} has a feasible solution when \textsc{fphf} has one. 
	It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{sffa} back to an approximate solution to \textsc{fphfa}.
	
	Based on the solution mapping method described above, it takes constant time to set the value of each homologous or non-homologous entry of $\ff^p$, and $\ff^p$ has $|E^p|$ entries, such a solution mapping takes $O(|E^p|)$ time.		
	
%		Given a solution $\ff^s$ returned by the \textsc{sffa} solver, we map the solution back to $\ff^p$ by the following mechanism: for pairwise homologous edges $e$ and $\hat{e}$, we map back by setting $\ff^p(e)=\ff^s_1(e_1), \ff^p(\hat{e})=\ff^s_1(\hat{e}_1)$; for each non-homologous edge $e'$, we map back by setting $\ff^p(e')=\ff^s_1(e')$. Note that $\ff^s$ is a two-commodity flow while $\ff^p$ is a single-commodity flow.
%		As there are $|E^p|$ entries to set value, mapping $\ff^s$ back to $\ff^p$ takes $O(|E^p|)$ time.
		
	Now, we conduct error analysis. We claim that the mapping will generate three types of error: (1) error in congestion; (2) error in demand; (3) error in pair homology. 
	%According to Def. \ref{def: fphf}, fixed flow edges and homologous edges are disjoint, thus $\ll(e)=0, \forall e\in H_i\in\mathcal{H}^p$.
	% Definition \ref{def: fphfa}, capacity bound for homologous edges in $G^p$ can only be in the form of $(0,R)$, where $R$ is the polytope diameter of \textsc{lpa}.
	\begin{enumerate}
		\item Error in congestion.\\
		We first track the error of the upper bound of capacity. For any pair of homologous edges $e$ and $\hat{e}$ with capacity $\uu^p(e)=\uu^p(\hat{e})$, the maximum flow to be routed in $e$ and $\hat{e}$ is
		\[(1+\tau^p_u)\uu^p(e)=\ff^s_1(e_1)\leq \ff^s(e_1)\leq (1+\epsilon^s_u)\uu^s(e_1)=(1+\epsilon^s_u)\uu^p(e),\]
		and 
		\[(1+\tau^p_u)\uu^p(\hat{e})=\ff^s_1(\hat{e}_1)\leq \ff^s(\hat{e}_1)\leq (1+\epsilon^s_u)\uu^s(\hat{e}_1)=(1+\epsilon^s_u)\uu^p(\hat{e}),\]
		thus,
		\begin{equation}
			\label{eq: fph-sff-u}
			\tau^p_u\leq \epsilon^s_u.
		\end{equation}
		
		For any non-homologous edge $e'$, then $e'$ is a fixed flow edge with fixed flow $\uu^p(e')$, the maximum flow to be routed in $e'$ is
		\[(1+\tau_u^{p})\uu^p(e')=\ff^s_1(e')\leq \ff^s(e')\leq (1+\epsilon^s_u)\uu^s(e')=(1+\epsilon^s_u)\uu^p(e'),\]
		thus again,
		\[\tau^{p}_u\leq \epsilon^s_u.\]
	
		Next, we track the error of the lower bound of capacity. And we only need to take fixed flow edges (thus non-homologous edges) into consideration. For any fixed flow edge $e'\in F^p$, as it is copied to an edge selecting commodity 1 in $G^s$, then the minimum flow to be routed in $e'$ can be lower bounded by
		\begin{align*}
			(1-\tau^p_l)\uu^p(e')&=\ff^s_1(e')\\
			&\geq \ff^s(e')-\epsilon^s_{t1} && \text{Because of error in type in $G^s$}\\
			&\geq (1-\epsilon^s_l)\uu^s(e')-\epsilon^s_{t1} && \text{Because of error in congestion in $G^s$}\\
			&=(1-\epsilon^s_l)\uu^p(e')-\epsilon^s_{t1} && \text{Because $\uu^p(e')=\uu^s(e')$}\\
			&=\left(1-\epsilon^s_l-\frac{\epsilon^s_{t1}}{\uu^p(e')}\right)\uu^p(e')\\
			&\geq \left(1-\epsilon^s_l-\epsilon^s_{t1}\right)\uu^p(e') && \text{$\uu^p(e')\geq 1$ because of integer capacities}
		\end{align*}			
		Thus, we have
		\begin{equation}
			\label{eq: fph-sff-l}
			\tau^{p}_l\leq \epsilon^s_l+\epsilon^s_{t1}.
		\end{equation}

		
		\item Error in demand.\\	
		%According to Definition \ref{def: fphfa}, 
		For simplicity, we denote $H^p=\bigcup_{i\in[p]}H_i$ as the set of all homologous edges. By Eq. \eqref{eqn:fphfa_error_demand} in Definition \ref{def: fphfa-new}, the error in demand that we can achieve for vertices other than $s, t$ in $G^p$ is computed as 
		\begin{scriptsize}
		\begin{equation}
			\label{eq: ph-slu}
			\begin{aligned}
				\tau^{p}_d&=\max_{w\in V^p\backslash\{s,t\}}\abs{\sum_{(v,w)\in E^p}\ff^p(v,w)-\sum_{(w,u)\in E^p}\ff^p(w,u)}\\
				&\overset{(1)}{=} \max_{w\in V^p\backslash\{s,t\}}\abs{\left(\sum_{(v,w)\in H^p}\ff^p(v,w)+\sum_{(v,w)\in E^p\backslash H^p}\ff^p(v,w) \right)-\left(\sum_{(w,u)\in H^p}\ff^p(w,u)+\sum_{(w,u)\in E^p\backslash H^p}\ff^p(w,u)\right)}\\
				&\overset{(2)}{=} \max_{w\in V^p\backslash\{s,t\}}\abs{\left(\sum_{e=(v,w)\in H^p}\ff^s_1(e_1)+\sum_{(v,w)\in E^p\backslash H^p}\ff^s_1(v,w)\right)-\left(\sum_{e=(w,u)\in H^p}\ff^s_1(e_1)+\sum_{(w,u)\in E^p\backslash H^p}\ff^s_1(w,u)\right)}\\
				&\overset{(3)}{\leq} \epsilon_{d1}^s+\max_{w\in V^p\backslash\{s,t\}}\abs{\left(\sum_{e=(v,w)\in H^p}\ff^s_1(e_1)+\sum_{(v,w)\in E^p\backslash H^p}\ff^s_1(v,w)\right)-\left(\sum_{e=(v,w)\in H^p}\ff^s_1(e_2)+\sum_{(v,w)\in E^p\backslash H^p}\ff^s_1(v,w)\right)}\\
				&=\epsilon_{d1}^s+ \max_{w\in V^p\backslash\{s,t\}}\abs{\sum_{e=(v,w)\in H^p}\ff^{s}_1(e_1)-\sum_{e=(v,w)\in H^p}\ff^{s}_1(e_2)}\\
				&=\epsilon_{d1}^s+ \max_{w\in V^p\backslash\{s,t\}}\abs{\sum_{e=(v,w)\in H^p}(\ff^{s}_1(e_1)-\ff^{s}_1(e_2))}\\
				&\leq \epsilon_{d1}^s+\max_{w\in V^p\backslash \{s,t\}}\sum_{e=(v,w)\in H^p}\abs{\ff^{s}_1(e_1)-\ff^{s}_1(e_2)}.
			\end{aligned}
		\end{equation}
		\end{scriptsize}
		
		For step (1), we separate homologous edges from non-homologous edges that are incident to vertex $w$.
		For step (2), we apply the rule of mapping $\ff^s$ back to $\ff^p$.
		For step (3), we apply Eq. \eqref{eqn:sffa_error_demand} in Definition \ref{def: sffa-new} with respect to vertex $w$, so that we replace the sum of outgoing flows of $w$ by the sum of its incoming flows with an error in demand for commodity 1 in $G^s$ being introduced, i.e.,
		\begin{scriptsize}
			\[\abs{\left(\sum_{e=(w,u)\in H^p}\ff^s_1(e_1)+\sum_{(w,u)\in E^p\backslash H^p}\ff^s_1(w,u)\right)-\left(\sum_{e=(v,w)\in H^p}\ff^s_1(e_2)+\sum_{(v,w)\in E^p\backslash H^p}\ff^s_1(v,w)\right)}\leq \epsilon^s_{d1}.\]
		\end{scriptsize}
		
		Now, we try to bound $\abs{\ff^{s}_1(e_1)-\ff^{s}_1(e_2)}$. We apply Eq. \eqref{eqn:sffa_error_demand} again with respect to vertex $vw$. Since $vw$ is only incident to $e_1, e_3, e_4$, we have
		\begin{equation}
		   \label{eq: ph-slu-vw}
		   \abs{\ff^s_1(e_1)+\ff^s_1(e_3)-\ff^s_1(e_4)}\leq \epsilon_{d1}^{s}.
		\end{equation}
		Similarly, by error in demand of vertex $vw'$, we have
		\begin{equation}
		   \label{eq: ph-slu-vw'}
		   \abs{\ff^s_1(e_2)+\ff^s_1(e_5)-\ff^s_1(e_4)}\leq \epsilon_{d1}^{s}.
		\end{equation}
	
		Combining Eq. \eqref{eq: ph-slu-vw} and Eq. \eqref{eq: ph-slu-vw'}, we have
		\begin{align*}
			\abs{(\ff^s_1(e_1)+\ff^s_1(e_3))-(\ff^s_1(e_2)+\ff^s_1(e_5))}\leq 2\epsilon_{d1}^{s}.
		\end{align*}
		Moreover, we can also lower bound its left hand side by
		\begin{align*}
		   \abs{(\ff^s_1(e_1)+\ff^s_1(e_3))-(\ff^s_1(e_2)+\ff^s_1(e_5))}&=\abs{(\ff^s_1(e_1)-\ff^s_1(e_2))+(\ff^s_1(e_3)-\ff^s_1(e_5))}\\
		   &\geq\abs{\ff^s_1(e_1)-\ff^s_1(e_2)}-\abs{\ff^s_1(e_3)-\ff^s_1(e_5)}.
		\end{align*}
     By rearranging, $\abs{\ff^s_1(e_1)-\ff^s_1(e_2)}$ can be upper bounded by
     \begin{equation}
         \label{eq: ph-slu-2}
         \begin{aligned}
             &\abs{\ff^s_1(e_1)-\ff^s_1(e_2)}\\
             \leq & \abs{\ff^s_1(e_3)-\ff^s_1(e_5)}+\abs{(\ff^s_1(e_1)+\ff^s_1(e_3))-(\ff^s_1(e_2)+\ff^s_1(e_5))}\\
             \leq& \abs{\ff^s_1(e_3)-\ff^s_1(e_5)}+2\epsilon_{d1}^s \\
            	\leq& \max\{\ff^s_1(e_3), \ff^s_1(e_5)\}+2\epsilon_{d1}^s && \text{Because $\ff^s_1(e_3), \ff^s_1(e_5)\geq 0$}\\
            	\leq& \epsilon_{t2}^s+2\epsilon_{d1}^s, 
         \end{aligned}
     \end{equation}
     where the last inequality comes from error in type for $e_3$ and $e_5$, since they are both selective edges for commodity 2.
     
     Finally, applying the upper bound of $\abs{\ff^s_1(e_1)-\ff^s_1(e_2)}$ Eq. \eqref{eq: ph-slu-2} back to Eq. \eqref{eq: ph-slu}, we obtain
     \begin{equation}
        	\label{eq: fph-sff-d}
        	\begin{aligned}
        		\tau_d^p&\leq \epsilon_{d1}^s+|H^p| \abs{\ff_1^s(e_1)-\ff_1^s(e_2)}\\
        		&\leq \epsilon_{d1}^s+|H^p|(\epsilon_{t2}^s+2\epsilon_{d1}^s)\\
        		&=(2|H^p|+1)\epsilon_{d1}^s+|H^p|\epsilon_{t2}^s\\
        		&\leq 3|H^p|(\epsilon_{d1}^s+\epsilon_{t2}^s) && \text{Because $|H^p|\geq 1$}\\
        		&\leq 3|E^p|(\epsilon_{d1}^s+\epsilon_{t2}^s).
        	\end{aligned}
     \end{equation}

		
		\item Error in pair homology.\\
		%According to Definition \ref{def: fphfa}, 
		By Eq. \eqref{eqn:fphfa_error_homology} in Definition \ref{def: fphfa-new}, the error in pair homology that we can achieve is computed as
		\begin{equation}
			\label{eq: ph-ph}
			\begin{aligned}
				\tau^p_h&=\max_{\mathcal{H}^p\ni H_i=\{(v,w),(y,z)\}} \abs{\ff^p(v,w)-\ff^p(y,z)}\\
				&=\max_{\mathcal{H}^p\ni H_i=\{e=(v,w),\hat{e}=(y,z)\}} \abs{\ff^s_1(e_1)-\ff^s_1(\hat{e}_1)},
			\end{aligned}
		\end{equation} 
		where the last equality comes from the rule of mapping $\ff^s$ back to $\ff^p$ for homologous edges.		
			
		Now, we try to bound $\abs{\ff^s_1(e_1)-\ff^s_1(\hat{e}_1)}$ for an arbitrary pair of homologous edges $e,\hat{e}$ with capacity $\uu^p(e) (=\uu^p(\hat{e}))$.
		
		As $e_4$ and $\hat{e}_4$ are fixed flow edges, we apply error in congestion as defined in Eq. \eqref{eqn:sffa_error_congestion_1} in Definition \ref{def: sffa-new}, so that their flow difference can be bounded by 
		\[\abs{\ff^s(e_4)-\ff^s(\hat{e}_4)}\leq (\epsilon_l^s+\epsilon_u^s)\uu^p(e).\]
		And by error in demand of vertices $vw$ and $yz$ in $G^s$, we have
		\[\abs{\ff^s(e_1)+\ff^s(e_3)-\ff^s(e_4)}\leq \epsilon_{d1}^{s}+ \epsilon_{d2}^{s},\]
		\[\abs{\ff^s(\hat{e}_1)+\ff^s(\hat{e}_3)-\ff^s(\hat{e}_4)}\leq \epsilon_{d1}^{s}+ \epsilon_{d2}^{s}.\]
		Combining the above three inequalities, we have
		\begin{align*}
			\abs{(\ff^s(e_1)+\ff^s(e_3))-(\ff^s(\hat{e}_1)+\ff^s(\hat{e}_3))}\leq (\epsilon_l^s+\epsilon_u^s)\uu^p(e)+2\epsilon_{d1}^{s}+ 2\epsilon_{d2}^{s}.
		\end{align*}
		Again, we can also lower bound its left hand side by 
		\begin{align*}
			&\abs{(\ff^s(e_1)+\ff^s(e_3))-(\ff^s(\hat{e}_1)+\ff^s(\hat{e}_3))}\\
			=&\abs{(\ff^s_1(e_1)+\ff^s_2(e_1)+\ff^s_1(e_3)+\ff^s_2(e_3))-(\ff^s_1(\hat{e}_1)+\ff^s_2(\hat{e}_1)+\ff^s_1(\hat{e}_3)+\ff^s_2(\hat{e}_3))}\\
			=&\abs{(\ff^s_1(e_1)-\ff^s_1(\hat{e}_1))+(\ff^s_2(e_1)-\ff^s_2(\hat{e}_1))+(\ff^s_1(e_3)-\ff^s_1(\hat{e}_3))+(\ff^s_2(e_3)-\ff^s_2(\hat{e}_3))}\\
			\geq& \abs{\ff^s_1(e_1)-\ff^s_1(\hat{e}_1)}-\abs{(\ff^s_2(e_1)-\ff^s_2(\hat{e}_1))+(\ff^s_1(e_3)-\ff^s_1(\hat{e}_3))+(\ff^s_2(e_3)-\ff^s_2(\hat{e}_3))}.
		\end{align*}
		By rearranging, we can upper bound $\abs{\ff^s_1(e_1)-\ff^s_1(\hat{e}_1)}$ by
		\begin{small}
		\begin{align*}
			&\abs{\ff^s_1(e_1)-\ff^s_1(\hat{e}_1)}\\
			\leq&\abs{(\ff^s(e_1)+\ff^s(e_3))-(\ff^s(\hat{e}_1)+\ff^s(\hat{e}_3))} +\abs{(\ff^s_2(e_1)-\ff^s_2(\hat{e}_1))+(\ff^s_1(e_3)-\ff^s_1(\hat{e}_3))+(\ff^s_2(e_3)-\ff^s_2(\hat{e}_3))}\\
			\leq& (\epsilon_l^s+\epsilon_u^s)\uu^p(e)+2\epsilon_{d1}^{s}+ 2\epsilon_{d2}^{s}+\abs{\ff^s_2(e_1)-\ff^s_2(\hat{e}_1)}+\abs{\ff^s_1(e_3)-\ff^s_1(\hat{e}_3)}+\abs{\ff^s_2(e_3)-\ff^s_2(\hat{e}_3)},
		\end{align*}
		\end{small}
		where we have 
		\begin{itemize}
			\item $\abs{\ff^s_2(e_1)-\ff^s_2(\hat{e}_1)}\leq \max\{\ff^s_2(e_1),\ff^s_2(\hat{e}_1)\}\leq \epsilon_{t1}^{s}$ because of error in type in $G^s$ and $e_1,\hat{e}_1$ are selective edges for commodity 1;
			\item $\abs{\ff^s_1(e_3)-\ff^s_1(\hat{e}_3)}\leq \max\{\ff^s_1(e_3), \ff^s_1(\hat{e}_3)\}\leq \epsilon_{t2}^{s}$ because of error in type in $G^s$ and $e_3,\hat{e}_3$ are selective edges for commodity 2;
			\item $\abs{\ff^s_2(e_3)-\ff^s_2(\hat{e}_3)} \leq \epsilon_{t1}^s+2\epsilon_{d2}^s$, which can be obtained directly by symmetry from the bound of $\abs{\ff^s_1(e_1)-\ff^s_1(e_2)}$ in Eq. \eqref{eq: ph-slu-2}.
		\end{itemize}
		
		Putting all together, we have
		\begin{align*}
			\abs{\ff^s_1(e_1)-\ff^s_1(\hat{e}_1)}&\leq \uu^p(e)(\epsilon_l^s+\epsilon_u^s)+2\epsilon_{d1}^{s}+ 2\epsilon_{d2}^{s}+\epsilon_{t}^{s1}+\epsilon_{t2}^{s}+\epsilon_{t1}^s+2\epsilon_{d2}^s\\
			&\leq \norm{\uu^p}_{max}(\epsilon_l^s+\epsilon_u^s)+2\epsilon_{d1}^s+4\epsilon_{d2}^{s}+2\epsilon_{t1}^s+\epsilon_{t2}^s.
		\end{align*}
		%where $u^p_{max}=\max_{e\in E^p\backslash F^p} \uu^p(e)$.
		Thus, by Eq. \eqref{eq: ph-ph}, we have
		\begin{equation}
			\label{eq: fph-sff-p}
			\tau^p_h\leq \norm{\uu^p}_{max}(\epsilon_l^s+\epsilon_u^s)+2\epsilon_{d1}^s+4\epsilon_{d2}^{s}+2\epsilon_{t1}^s+\epsilon_{t2}^s.
		\end{equation}
	\end{enumerate}

	Now, we prove that $\ff^p$ is a solution to the \textsc{fphfa} instance by showing that the errors achieved by $\ff^p$ is less than the error target set in the \textsc{fphfa} instance. Combining Eq. \eqref{eq: fph-sff-u}, \eqref{eq: fph-sff-l}, \eqref{eq: fph-sff-d}, \eqref{eq: fph-sff-p}, we have
	\begin{align*}
		\tau^{p}_u&\leq \epsilon^s_u,\\
		\tau^{p}_l&\leq \epsilon^s_l+\epsilon^s_{t1},\\
		\tau^p_d&\leq 3|E^p|(\epsilon_{d1}^s+\epsilon_{t2}^s),\\
		\tau^p_h&\leq \norm{\uu^p}_{max}(\epsilon_l^s+\epsilon_u^s)+2\epsilon_{d1}^s+4\epsilon_{d2}^{s}+2\epsilon_{t1}^s+\epsilon_{t2}^s.
	\end{align*}
	As we set in the reduction that $\epsilon_l^s=\min\left\{\frac{\epsilon^p_l}{2}, \frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}\right\},
	\epsilon_u^s=\min\left\{\epsilon_u^p, \frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}\right\},
	\epsilon_{d1}^s= \min\left\{\frac{\epsilon^p_d}{6|E^p|}, \frac{\epsilon^p_h}{10}\right\},\\
	\epsilon_{d2}^s= \frac{\epsilon^p_h}{10},
	\epsilon_{t1}^s= \min\left\{\frac{\epsilon^p_l}{2},\frac{\epsilon^p_h}{10}\right\},
	\epsilon_{t2}^s= \min\left\{\frac{\epsilon^p_d}{6|E^p|}, \frac{\epsilon^p_h}{10}\right\}$,
	thus we have 
	\[\tau^p_u\leq \epsilon^p_u,\]
	\[\tau^p_l\leq \frac{\epsilon^p_l}{2}+\frac{\epsilon^p_l}{2}=\epsilon^p_l,\]
	\[\tau^p_d\leq 3|E^p|\left(\frac{\epsilon^p_d}{6|E^p|}+\frac{\epsilon^p_d}{6|E^p|}\right)=\epsilon^p_d,\]
	\[\tau^p_h\leq \norm{\uu^p}_{max}\left(\frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}+\frac{\epsilon^p_h}{20\norm{\uu^p}_{max}}\right)+\frac{2\epsilon^p_h}{10}+\frac{4\epsilon^p_h}{10}+\frac{2\epsilon^p_h}{10}+\frac{\epsilon^p_h}{10}=\epsilon^p_h.\]
	
	Thus, we can conclude that if $\ff^s$ is a solution to the \textsc{sffa} instance with the error $\epsilon^s_l,\epsilon^s_u, \epsilon^s_{d1}, \epsilon^s_{d2}, \epsilon^s_{t1}, \epsilon^s_{t2}$ as set in the reduction, we can map it back to a solution $\ff^p$ to the \textsc{fphfa} instance with its error target achieved.
\end{proof}


\subsection{SFF(A) to 2CFF(A)}
\label{sect: sffa-2cffa}
\subsubsection{SFF to 2CFF}
We show the reduction from an \textsc{sff} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2)$ to a \textsc{2cff} instance $(G^f, F^f, \uu^f, s_1,t_1, s_2,t_2)$. 
Assume that $e\in S_i$ is an arbitrary selective edge for commodity $i$ in $G^p$. As shown in Figure \ref{fig: slu2cf-lu2cf}, we map $e$ in $G^s$ to a gadget consisting of edges $\{e_1,e_2,e_3,e_4,e_5\}$ in $G^f$. Note that selective edges can be both fixed flow edges and non-fixed flow edges. We integrate these two cases in Figure \ref{fig: slu2cf-lu2cf}, where $l=u$ if it is a fixed flow edge and $l=0$ if it is a non-fixed flow edge.\ming{need rephrasing}
Moreover, no reduction is performed on non-selective edges in $G^s$, and we trivially copy these edges to $G^f$. 

The key idea to remove the selective requirement is utilizing edge directions and the source-sink pair $(s_i, t_i)$ to simulate a selective edge $e$ for commodity $i$. 
More specifically, in the gadget, the flow of commodity $i$ routes through three directed paths: (1) $e_1\rightarrow e_4$, (2) $e_5\rightarrow e_2\rightarrow e_4$, (3) $e_5\rightarrow e_3$. The selective requirement is realized because $e_4$ is the only outgoing edge of $xy$ and only flow of commodity $i$ is allowed in $e_4$, hence in $e_1$. Similarly, $e_5$ is the only incoming edge of $xy'$ and only flow of commodity $i$ is allowed in $e_5$, hence in $e_3$.
In addition, to ensure that $e_1$ and $e_3$ route the same amount of flow, flows in $e_4$ and $e_5$ must be equal by the conservation of flows. 
Therefore, we impose the fixed flow constraint on $e_4$ and $e_5$ by setting the fixed flow to be $u$. We remove $e_2$ if $e$ is a fixed flow edge, or set capacity of $e_2$ to be $u$ otherwise. \ming{need rephrasing}
%the difference of the upper and lower capacity bound of $e$. This can simulate the capacity bound of $e$ in the gadget.
%Note that the lower capacity bound of a selective edge $e$ is either 0 (if $e\notin F^s$) or equal to the upper capacity bound (if $e\in F^s$).


\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\textwidth]{image/slu2CF-lu2CF}
	\caption{The reduction from \textsc{sff} to \textsc{2cff}. $l=u$ if $e$ is a fixed flow edge, and $l=0$ if $e$ is a non fixed flow edge.} 
	\label{fig: slu2cf-lu2cf}
\end{figure}

If a \textsc{2cff} solver returns $\ff^f$ for the \textsc{2cff} instance $(G^f, F^f, \uu^f, s_1,t_1, s_2,t_2)$, then we return $\ff^s$ for the \textsc{sff} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2)$ by the following method:
for any selective edge $e\in S_i$, we set $\ff^s_i(e)=\ff^f_i(e_1), \ff^s_{\bar{i}}(e)=\ff^f_{\bar{i}}(e_1)=0, \bar{i}\in\{1,2\}\backslash i$; and for any non-selective edge $e\in E^s\backslash (S_1\bigcup S_2)$, we map back trivially by setting $\ff^s_i(e)=\ff^f_i(e), i\in\{1,2\}$. 


%To reduce an \textsc{sffa} instance to a \textsc{2cffa} instance, we map each edge $e\in S_i$ that selects commodity $i$ in $G^s$ to edges $\{e_1,e_2,e_3,e_4,e_5\}$ in $G^f$, as shown in Figure \ref{fig: slu2cf-lu2cf}. Note that $F^s \bigcap S \neq \emptyset$, thus selective edges can be both non-fixed flow edges (i.e., $\ll(e)=0$) and fixed flow edges (i.e., $\ll(e)=\uu(e)$). Moreover, as no reduction is performed on non-selective edges in $E^s\backslash S$, we trivially copy these edges to $G^f$.

\begin{lemma}[\textsc{sff} to \textsc{2cff}]
	\label{lm: sff-2cff}
	Given an \textsc{sff} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2)$,
	we can construct, in time $O(|E^s|)$, a \textsc{2cff} instance $(G^f, F^f, \uu^f, s_1,t_1, s_2,t_2)$ such that
	\[|V^f|=|V^s|+2(|S_1|+|S_2|),\qquad |E^f|=|E^s|+4(|S_1|+|S_2|), \qquad |F^f|\leq4(|F^s|+|S_1|+|S_2|), \]
	\[\norm{\uu^f}_{max}= \norm{\uu^s}_{max},\]
	and if the \textsc{sff} instance has a solution, then the \textsc{2cff} instance has a solution.
	%	and if $\ff^h$ is a solution to the FHF instance, then in time $O(\hat{n})$, we can compute a solution $\hat{\xx}$ to the 1-LEN instance.
\end{lemma}	
\begin{proof}
	According to the reduction described above, from any solution $\ff^s$ to the \textsc{sff} instance, it is easy to derive a solution $\ff^f$ to the \textsc{2cff} instance. Concretely, we define a feasible flow $\ff^f$ as follows:
	\begin{itemize}
		\item For any selective edge $e\in S_i$, in its corresponding gadget in $G^f$, we set
		\[l\leq \ff^f_i(e_1)=\ff^f_i(e_3)=\ff^s_i(e)\leq u,\]
		\[\ff^f_i(e_4)=\ff^f_i(e_5)=u,\]
		\[0\leq \ff^f_i(e_2)=u-\ff^s_i(e) \leq u-l,\]
		where $l=0$ if $e$ is an non-fixed flow edge, or $l=u=\uu^s(e)$ if $e$ is a fixed flow edge. And we set
		\[\ff^f_{\bar{i}}(e_1)=\ff^f_{\bar{i}}(e_2)=\ff^f_{\bar{i}}(e_3)=\ff^f_{\bar{i}}(e_4)=\ff^f_{\bar{i}}(e_5)=0, \qquad \bar{i}=\{1,2\}\backslash i.\]
		It is obvious that $\ff^f$ satisfies the capacity constraint on edges $(e_1, \ldots, e_5)$, and the flow conservation constraint on vertices $xy, xy'$.
		
		\item For any non-selective edge $e'\in E^s\backslash (S_1\bigcup S_2)$, we also have $e'\in E^f$ since no reduction is made on this edge, and we copy it trivially to $G^f$. We set
		\[\ff^f_i(e')=\ff^s_i(e'), \qquad i\in\{1,2\}.\]
		Since $\ff^s$ is a feasible flow in $G^s$, it is easy to check that $\ff^f$ also satisfies the capacity constraint on non-selective edges, as well as the flow conservation constraint on vertices incident to non-selective edges. Moreover, if $e'$ is a fixed flow edge, the fixed flow edge constraint is also satisfied.
	\end{itemize}
	To conclude, $\ff^f$ is a feasible flow to the \textsc{2cff} instance.
	\\
	\\
	Now, we track the change of problem size after reduction. Based on the reduction method, given an \textsc{sff} instance with $|V^s|$ vertices, $|E^s|$ edges (including $|F^s|$ fixed flow edges, and $|S_i|$ edges selecting commodity $i$), we can compute the size of the reduced \textsc{2cff} instance as follows.
	\begin{enumerate}
		\item $|V^f|$ vertices. As all vertices in $V^s$ are maintained, and for each selective edge $(x,y)\in (S_1\cup S_2)$, 2 auxiliary vertices $xy, xy'$ are added, we have
		\[|V^f|=|V^s|+2(|S_1|+|S_2|).\]
		
		\item $|E^f|$ edges. Since all non-selective edges in $E^s\backslash (S_1\cup S_2)$ are maintained, and each selective edge $e\in (S_1\cup S_2)$ is replaced by a gadget with 5 edges $(e_1, \cdots, e_5)$, we have
		\[|E^f|=(|E^s|-|S_1|-|S_2|)+5(|S_1|+|S_2|)=|E^s|+4(|S_1|+|S_2|).\]
		
		\item $|F^f|$ fixed flow edges. First, all non-selective fixed flow edges $e\in F^s\backslash (S_1\cup S_2)$ are maintained since no reduction is made.
		Then, for all selective fixed flow edges $e\in F^s\bigcap (S_1\cup S_2)$, the reduction generates 4 fixed flow edges (i.e., $e_1, e_3, e_4, e_5$).
		Finally, for all non-fixed flow selective edges $e\in (S_1\cup S_2)\backslash F^s$, the reduction generates 2 fixed flow edges (i.e., $e_4, e_5$). Hence, we have
		\[|F^f|=|F^s\backslash (S_1\cup S_2)|+4|F^s\cap (S_1\cup S_2)|+2|(S_1\cup S_2)\backslash F^s|\leq 4|F^s\cup S_1\cup S_2| \leq 4(|F^s|+|S_1|+|S_2|).\]
		
		\item The maximum edge capacity is bounded by 
		\[\norm{\uu^f}_{max}=\norm{\uu^s}_{max}.\]
		First, capacity of all non-selective edges in $E^s\backslash (S_1\cup S_2)$ is unchanged in $G^f$ since no reduction is made. Then, for all selective edges $e\in (S_1\cup S_2)$ with capacity (or fixed flow) $\uu^s(e)$, capacity of the 5 edges $(e_1,\ldots, e_5)$ in the gadget are with capacity at most $\uu^s(e)$.
	\end{enumerate}
	To estimate the reduction time, it is observed that it takes constant time to reduce each selective edge in $S_1\cup S_2$ since only a constant number of vertices and edges are added. And it takes constant time to copy each of the other non-selective edges in $E^s\backslash (S_1\cup S_2)$. Thus, the reduction of this step takes $O(|E^s|)$ time.
\end{proof}


\subsubsection{SFFA to 2CFFA}
The above lemma shows the reduction between exactly solving an \textsc{sff} instance and exactly solving a \textsc{2cff} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.
First of all, we give a definition of the approximate version of \textsc{2cff}.
	
% \textbf{Remark:} Note that error in demand in \textsc{2cffa} is assumed to be additive. There is no error in demand for $\{s_1,s_2\}$ since no requirements are imposed on the flow value of each commodity.
% \ming{Is it reasonable to set error in demand of $\{s_1,s_2\}$ is zero in the definition?}


\begin{definition}[2CFF Approximate Problem (\textsc{2cffa})]
	\label{def: 2cffa-new}
	A \textsc{2cffa} instance is given by a \textsc{2cff} instance $(G, F, \uu, s_1,t_1, s_2,t_2)$ as in Definition \ref{def: 2cff}, and error parameters $\epsilon_l,\epsilon_u\in[0,1]$, $\epsilon_{d1},\epsilon_{d2} \geq 0$, which we collect in a tuple $\left(G,F, \uu, s_1,t_1,s_2,t_2, \epsilon_l, \epsilon_u,\epsilon_{d1},\epsilon_{d2}\right)$.
	We say an algorithm solves the \textsc{2cffa} problem, if, given any \textsc{2cffa} instance, it returns a pair of flows $\ff_1, \ff_2\geq\bf{0}$ (denote $\ff=\ff_1+\ff_2$) that satisfies
	\begin{align}
		&(1-\epsilon_l)\uu(e)\leq \ff_1(e)+\ff_2(e)\leq(1+\epsilon_u)\uu(e), ~~ \forall e \in F \label{eqn:2cffa_error_congestion_1} \\
		&0\leq \ff_1(e)+\ff_2(e)\leq(1+\epsilon_u)\uu(e), ~~ \forall e \in E\backslash F \label{eqn:2cffa_error_congestion_2} \\
		& \abs{\sum_{\begin{subarray}{c}
					u:
					(u,v)\in E
			\end{subarray}}\ff_i(u,v)-\sum_{\begin{subarray}{c}
					w:
					(v,w)\in E
			\end{subarray}}\ff_i(v,w)}\leq \epsilon_{di}, ~~ \forall v\in V\backslash \{s_i,t_i\},~ i\in\{1,2\} \label{eqn:2cffa_error_demand}\\
		& \sum_{\begin{subarray}{c}
				w:
				(s_{\bar{i}}, w)\in E
		\end{subarray}}\ff_i(s_{\bar{i}}, w)=0, \sum_{\begin{subarray}{c}
				u:
				(u,t_{\bar{i}})\in E
		\end{subarray}}\ff_i(u,t_{\bar{i}})\leq \epsilon_{di}, ~~ \bar{i}=\{1,2\}\backslash i \label{eqn:2cffa_error_demand_s_t}
	\end{align}
	or it correctly declares that the associated \textsc{2cff} instance is infeasible. We refer to the error in \eqref{eqn:2cffa_error_congestion_1} and \eqref{eqn:2cffa_error_congestion_2} as error in congestion, error in \eqref{eqn:2cffa_error_demand} and \eqref{eqn:2cffa_error_demand_s_t} as error in demand.
\end{definition}	

We can use the same reduction method and solution mapping method in the exact case to the approximate case.
%Furthermore, if a \textsc{2cffa} solver returns $\ff^f$ for the \textsc{2cffa} instance $\left(G^f,F^f, \uu^f, s_1,t_1,s_2,t_2, \epsilon^f_l, \epsilon^f_u,\epsilon^f_{d1},\epsilon^f_{d2}\right)$, then we return $\ff^s$ for the \textsc{sffa} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2, \epsilon^s_l, \epsilon^s_u,\epsilon^s_{d1},\epsilon^s_{d2},\epsilon^s_{t1},\epsilon^s_{t2})$ by the following method:
%for any selective edge $e\in S_i$, we set $\ff^s_i(e)=\ff^f_i(e_1), \ff^s_{\bar{i}}(e)=\ff^f_{\bar{i}}(e_1), \bar{i}\in\{1,2\}\backslash i$; and for any non-selective edge $e\in E^s\backslash (S_1\bigcup S_2)$, we map back trivially by setting $\ff^s_i(e)=\ff^f_i(e), i\in\{1,2\}$. 
Note that, different from the exact case where $\ff^s_{\bar{i}}(e)=\ff^f_{\bar{i}}(e_1)=0$ if $e\in S_i$, it can be nonzero in the approximate case, which gives rise to error in type in $G^s$.


\begin{lemma}[\textsc{sffa} to \textsc{2cffa}]
	\label{lm: sffa-2cffa}
	Given an \textsc{sffa} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2, \epsilon^s_l, \epsilon^s_u,\epsilon^s_{d1},\epsilon^s_{d2},\epsilon^s_{t1},\epsilon^s_{t2})$, we can construct, in $O(|E^s|)$ time, an \textsc{2cffa} instance $\left(G^f,F^f, \uu^f, s_1,t_1,s_2,t_2, \epsilon^f_l, \epsilon^f_u,\epsilon^f_{d1},\epsilon^f_{d2}\right)$ such that
	\[|V^f|=|V^s|+2(|S_1|+|S_2|),\qquad |E^f|=|E^s|+4(|S_1|+|S_2|), \qquad |F^f|\leq4(|F^s|+|S_1|+|S_2|), \]
	\[\norm{\uu^f}_{max}= \norm{\uu^s}_{max},\]
	and
	\begin{align*}
		&\epsilon_l^f=\min\left\{\frac{\epsilon^s_l}{2}, \frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}\right\},
		&\epsilon_u^f=\min\left\{\epsilon_u^s, \frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}\right\},\\
		&\epsilon^f_{d1}= \min\left\{\frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)},\frac{\epsilon^s_l}{4}, \frac{\epsilon^s_{t2}}{2}\right\},
		&\epsilon^f_{d2}= \min\left\{\frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)}, \frac{\epsilon^s_l}{4}, \frac{\epsilon^s_{t2}}{2}\right\}.
	\end{align*}
%	where $u^s_{max}=\max_{e\in S}\uu^s(e)$. 
	If the \textsc{sff} instance $(G^s,F^s, S_1, S_2, \uu^s, s_1,t_1,s_2,t_2)$ has a solution, then the \textsc{2cffa} instance \\$\left(G^f,F^f, \uu^f, s_1,t_1,s_2,t_2\right)$ has a solution.
	Furthermore, if $\ff^f$ is a solution to the \textsc{2cffa} instance, then in time $O(|E^s|)$, we can compute a solution $\ff^s$ to the \textsc{sffa} instance.

%	Given a \textsc{sffa} instance $(G^s,F^s,\uu^s, S=S_1\cup S_2, \epsilon_l^s,\epsilon_u^s, \epsilon_{d1}^s, \epsilon_{d2}^s, \epsilon_{t1}^s,\epsilon_{t2}^s)$, it can be reduced to a \textsc{2cffa} instance $(G^f,F^f,\uu^f,\epsilon_l^f,\epsilon_u^f,\epsilon_{d1}^f,\epsilon_{d2}^f)$ in $O(|S_1|+|S_2|)$ time, such that $G^f$ has $|V^f|=O(|V^s|+|S_1|+|S_2|)$ vertices and $|V^f|=O(|E^s|+|S_1|+|S_2|)$ edges.
%	Suppose there is a \textsc{2cffa} solver with 
%	\begin{itemize}
%		\item $((1-\epsilon_l)\ll^f, (1+\epsilon_u)\uu^f)$ error in congestion;
%		\item $\epsilon_{di}^f, i\in\{1,2\}$ error in demand for commodity $i$.
%	\end{itemize}
%	Then it can be translated into a \textsc{sffa} solver with
%	\begin{itemize}
%		\item $((1-\epsilon_l^s)\ll^s, (1+\epsilon_u^s)\uu^s)$ error in congestion, where		
%		\[\epsilon_l^s=\epsilon_l^f+\frac{\epsilon_{d1}^f+\epsilon_{d2}^f}{u_{min}^f},\qquad \epsilon_u^s=\epsilon_u^f;\]
%		\item $\epsilon_{d1}^s$ error in demand of commodity 1, where
%		\[\epsilon_{d1}^s=O\left(|E^s|(\epsilon_{d1}^f+\epsilon_{d2}^f+u_{max}^f(\epsilon_l^f+\epsilon_u^f))\right);\]
%		
%		\item $\epsilon_{d2}^s$ error in demand of commodity 2, where
%		\[\epsilon_{d2}^s=O\left(|E^s|(\epsilon_{d1}^f+\epsilon_{d2}^f+u_{max}^f(\epsilon_l^f+\epsilon_u^f))\right);\]
%		
%		\item $\epsilon_{ti}^s, i\in\{1,2\}$ error in type for edges selecting commodity $i$, where
%		\[\epsilon_{ti}^s=O\left(\epsilon_{d\bar{i}}^f\right).\]
%	\end{itemize}
\end{lemma}	

\begin{proof}
	
%		\item \textbf{Reduction time}\\
%		It takes constant time to reduce each selective edge in $S$ since only a constant number of vertices and edges are added. And it takes constant time to copy each of the other edges in $E^s\backslash S$. Thus, the reduction of this step takes $O(|E^s|)$ time.
	Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: sff-2cff} also apply here, including the reduction time, problem size, and that \textsc{2cff} has a feasible solution when \textsc{sff} has one. 
	It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{2cffa} back to an approximate solution to \textsc{sffa}.
	
	Based on the solution mapping method described above, it takes constant time to set the value of each selective or non-selective entry of $\ff^s$, and $\ff^s$ has $|E^s|$ entries, such a solution mapping takes $O(|E^s|)$ time.	

%		Given a solution $\ff^f$ returned by the \textsc{2cffa} solver, we map the solution back to $G^s$ with the following rule: for any selective edge $e\in S$, we set $\ff^s_i(e)=\ff^f_i(e_1), i\in\{1,2\}$; and for any non-selective edge $e\in E^s\backslash S$, we map back trivially by setting $\ff^s_i(e)=\ff^f_i(e), i\in\{1,2\}$. As there are $|E^s|$ entries to set value, it takes $O(|E^s|)$ time to map $\ff^f$ back to $\ff^r$.
	Now, we conduct error analysis. The mapping will generate three types of error: (1) error in congestion; (2) error in demand; (3) error in type.
		\begin{enumerate}
			\item Error in congestion.\\
			Since we map solution back trivially for non-selective edges in $E^s\backslash (S_1\cup S_2)$, error in congestion of $G^f$ (i.e., $\epsilon^f_l, \epsilon^f_u$) still holds for $G^s$. Therefore, we focus on how error in congestion changes when mapping solution back to selective edges in $S_1 \cup S_2$.
			
			We first track the error of the upper bound of capacity. For any selective edge $e$, the maximum flow to be routed in $e$ is
			\[(1+\tau^s_u)\uu^s(e)=\sum_{i=\{1,2\}}\ff^s_i(e)=\sum_{i=\{1,2\}}\ff^f_i(e_1)\leq (1+\epsilon_u^f)\uu^f(e)=(1+\epsilon_u^f)\uu^s(e),\]
			thus,
			\begin{equation}
				\label{eq: slu-lu-u}
				\tau^s_u\leq \epsilon^f_u.
			\end{equation}
			%As we set $\epsilon^f_u\leq \epsilon^s_u$ in the reduction, it indicates that $\tau^s_u\leq\epsilon^s_u$.
			
			Next, we track the error of the lower bound of capacity. We only need to take selective fixed flow edges into consideration since there is no error of the lower bound of capacity for  non-fixed flow edges. Because of the error in demand of two commodities on vertex $xy$, by Definition \ref{def: 2cffa-new}, we have
			\[\left|\ff^f(e_1)+\ff^f(e_2)-\ff^f(e_4)\right|\leq \epsilon_{d1}^f+\epsilon_{d2}^f.\]
			Combined with error in congestion on edge $e_2$ and $e_4$, the minimum flow to be routed in $e=(x,y)$ is lower bounded by 
			\begin{equation}
				\label{eq: slu-lu-1}
				\begin{aligned}
					(1-\tau^s_l)\uu^s(e)=\ff^s(e)&=\ff^f(e_1)\\
					&\geq -\epsilon_{d1}^f-\epsilon_{d2}^f-\ff^f(e_2)+\ff^f(e_4)\\
					&\geq -\epsilon_{d1}^f-\epsilon_{d2}^f-(1+\epsilon_u^f)(\uu^s(e)-\uu^s(e))+(1-\epsilon_l^f)\uu^s(e),\\
					&\geq  -\epsilon_{d1}^f-\epsilon_{d2}^f+(1-\epsilon_l^f)\uu^s(e)\\
					&=(1-\epsilon_l^f-\frac{\epsilon_{d1}^f+\epsilon_{d2}^f}{\uu^s(e)})\uu^s(e),
				\end{aligned}
			\end{equation}
%			
%			As $\ll^s(e)=\uu^s(e)$ if $e$ is a fixed flow edge or $\ll^s(e)=0$ if $e$ is an non-fixed flow edge, it is noticed that the value of $\tau^s_l$ has no impact for the latter case. Therefore, we only need to take the former case into consideration.
%			Plugging $\ll^s(e)=\uu^s(e)$ back to Eq. \eqref{eq: slu-lu-1}, we have
%			\begin{align*}
%				(1-\tau^s_l)\uu^s(e)=\ff^s(e) &\geq  -\epsilon_{d1}^f-\epsilon_{d2}^f+(1-\epsilon_l^f)\uu^s(e)\\
%&=(1-\epsilon_l^f-\frac{\epsilon_{d1}^f+\epsilon_{d2}^f}{\uu^s(e)})\uu^s(e),
%			\end{align*}
			thus,
			\begin{equation}
				\label{eq: slu-lu-l}
				\tau_l^s\leq \epsilon_l^f+\frac{\epsilon_{d1}^f+\epsilon_{d2}^f}{\uu^s(e)}\leq \epsilon_l^f+\epsilon_{d1}^f+\epsilon_{d2}^f,
			\end{equation}
			where we use $\uu^s(e)\geq 1$ because of integer capacities.
			
			\item Error in demand.\\
			For simplicity, we denote $S=S_1\bigcup S_2$. By Eq. \eqref{eqn:sffa_error_demand} in Definition \ref{def: sffa-new}, error in demand of commodity $i$ that we can achieve for vertices other than $s_i, t_i$ in $G^s$ is computed as 
%				According to Definition \ref{def: sffa}, error in demand for commodity $i$ in $G^s$ can be computed as
			\begin{scriptsize}
			\begin{equation}
				\label{eq: slu-lu}
				\begin{aligned}
					\tau_{di}^s&=\max_{y\in V^s\backslash\{s_i,t_i\}}\abs{\sum_{(x,y)\in E^s}\ff^s_i(x,y)-\sum_{(y,z)\in E^s}\ff^s_i(y,z)}\\
					&\overset{(1)}{=} \max_{y\in V^s\backslash\{s_i,t_i\}}\abs{\left(\sum_{(x,y)\in S}\ff^s_i(x,y)+\sum_{(x,y)\in E^s\backslash S}\ff^s_i(x,y)\right)-\left(\sum_{(y,z)\in S}\ff^s_i(y,z)+\sum_{(y,z)\in E^s\backslash S}\ff^s_i(y,z)\right)}\\
					&\overset{(2)}{=} \max_{y\in V^s\backslash\{s_i,t_i\}}\abs{\left(\sum_{e=(x,y)\in S}\ff^f_i(e_1)+\sum_{(x,y)\in E^s\backslash S}\ff^f_i(x,y)\right)-\left(\sum_{e=(y,z)\in S}\ff^f_i(e_1)+\sum_{(y,z)\in E^s\backslash S}\ff^f_i(y,z)\right)} \\
					&\overset{(3)}{\leq} \epsilon^f_{di}+\max_{y\in V^s\backslash\{s_i,t_i\}}\abs{\left(\sum_{e=(x,y)\in S}\ff^f_i(e_1)+\sum_{(x,y)\in E^s\backslash S}\ff^f_i(x,y)\right)-\left(\sum_{e=(x,y)\in S}\ff^f_i(e_3)+\sum_{(x,y)\in E^s\backslash S}\ff^f_i(x,y)\right)} \\
					&= \epsilon^f_{di}+\max_{y\in V^s\backslash\{s_i,t_i\}}\abs{\sum_{e=(x,y)\in S}\ff^f_i(e_1)-\sum_{e=(x,y)\in S}\ff^f_i(e_3)}\\
					&=\epsilon^f_{di}+\max_{y\in V^s\backslash\{s_i,t_i\}}\abs{\sum_{e=(x,y)\in S}(\ff^f_i(e_1)-\ff^f_i(e_3))}\\
					&\leq \epsilon^f_{di}+\max_{y\in V^s\backslash\{s_i,t_i\}}\sum_{e=(x,y)\in S}\abs{\ff^f_i(e_1)-\ff^f_i(e_3)}\\
					&= \epsilon^f_{di}+\max_{y\in V^s\backslash\{s_i,t_i\}}\left\{\sum_{e=(x,y)\in S_1}\abs{\ff^f_i(e_1)-\ff^f_i(e_3)}+\sum_{\hat{e}=(x,y)\in S_2}\abs{\ff^f_i(\hat{e}_1)-\ff^f_i(\hat{e}_3)}\right\}.
				\end{aligned}
			\end{equation}
			\end{scriptsize}
		
			For step (1), we separate selective edges from non-selective edges that are incident to vertex $y$.
			For step (2), we apply the rule of mapping $\ff^f$ back to $\ff^s$.
			For step (3), we apply Eq. \eqref{eqn:2cffa_error_demand} in Definition \ref{def: 2cffa-new} with respect to vertex $y$, so that we can replace the sum of outgoing flows of $y$ by the sum of incoming flows, where an error of $\epsilon^f_{di}$ is introduced because of the error in demand of vertex $y$ in $G^f$, i.e., 
			\begin{scriptsize}
			\[\abs{\left(\sum_{e=(y,z)\in S}\ff^f_i(e_1)+\sum_{(y,z)\in E^s\backslash S}\ff^f_i(y,z)\right)-\left(\sum_{e=(x,y)\in S}\ff^f_i(e_3)+\sum_{(x,y)\in E^s\backslash S}\ff^f_i(x,y)\right)}\leq \epsilon^f_{di}.\]					
			\end{scriptsize}
		
			Now, we try to bound $\abs{\ff^f_i(e_1)-\ff^f_i(e_3)}$. We apply Eq. \eqref{eqn:2cffa_error_demand} again with respect to vertex $xy$. Since $xy$ is only incident to $e_1, e_2, e_4$, we have			
			\[\left|\ff^f_i(e_1)+\ff^f_i(e_2)-\ff^f_i(e_4)\right|\leq \epsilon_{di}^f.\]
%				hence,
%				\begin{equation}
%					\label{eq: slu-lu-xy}
%					-\epsilon_{di}^f-\ff^f_i(e_2)+\ff^f_i(e_4)\leq \ff^f_i(e_1)\leq \epsilon_{di}^f -\ff^f_i(e_2)+\ff^f_i(e_4).
%				\end{equation}
			Similarly, by the error in demand of vertex $xy'$, we have
			\[\left|\ff^f_i(e_3)+\ff^f_i(e_2)-\ff^f_i(e_5)\right|\leq \epsilon_{di}^f.\]
%				hence,
%				\begin{equation}
%					\label{eq: slu-lu-xy'}
%					-\epsilon_{di}^f-\ff^f_i(e_2)+\ff^f_i(e_5)\leq \ff^f_i(e_3)\leq \epsilon_{di}^f-\ff^f_i(e_2)+\ff^f_i(e_5).
%				\end{equation}
			Combining the above two inequalities, we have
			\[-2\epsilon_{di}^f+\ff^f_i(e_4)-\ff^f_i(e_5)\leq\ff^f_i(e_1)-\ff^f_i(e_3)\leq 2\epsilon_{di}^f+\ff^f_i(e_4)-\ff^f_i(e_5),\]
			which can be rewritten as
			\begin{equation}
				\label{eq: slu-lu-s1}
				\begin{aligned}
					\left|\ff^f_i(e_1)-\ff^f_i(e_3)\right|&\leq2\epsilon_{di}^f+\left|\ff^f_i(e_4)-\ff^f_i(e_5)\right|.
				\end{aligned}
			\end{equation}	
		
			Since $e_4$ and $e_5$ are incident to $t_i$ and $s_i$, respectively, we now analyze by separating the cases of $e\in S_1$ and $e\in S_2$. 
			\paragraph{Case 1:}
			In the case of $e\in S_1$, $e_4$ and $e_5$ are incident to $t_1$ and $s_1$, respectively. Then, for flow of commodity 1, i.e., $i=1$, Eq. \eqref{eq: slu-lu-s1} can be further bounded by
			\begin{equation}
				\label{eq: slu-lu-s1(1)}
				\begin{aligned}
					\left|\ff^f_1(e_1)-\ff^f_1(e_3)\right|&\leq2\epsilon_{d1}^f+\left|\ff^f_1(e_4)-\ff^f_1(e_5)\right|\\
					&=2\epsilon_{d1}^f+\left|(\ff^f(e_4)-\ff^f_{2}(e_4))-(\ff^f(e_5)-\ff^f_{2}(e_5))\right|\\
					&\leq2\epsilon_{d1}^f+\left|\ff^f(e_4)-\ff^f(e_5)\right|+\left|\ff^f_{2}(e_4)-\ff^f_{2}(e_5)\right|\\
					&\overset{(1)}{=}2\epsilon_{d1}^f+\left|\ff^f(e_4)-\ff^f(e_5)\right|+\ff^f_{2}(e_4)\\
					&\overset{(2)}{\leq}2\epsilon_{d1}^f+\left|\ff^f(e_4)-\ff^f(e_5)\right|+\epsilon_{d2}^f\\
					&\overset{(3)}{\leq} 2\epsilon_{d1}^f+(\epsilon_l^f+\epsilon_u^f)\uu^s(e)+\epsilon_{d2}^f.
				\end{aligned}
			\end{equation}	
			
			For step (1), we use $\ff^f_{2}(e_5)=0$ because there is no error in demand for $s_1$ in $G^f$ by Eq. \eqref{eqn:2cffa_error_demand_s_t} in Definition \ref{def: 2cffa-new}.
			For step (2), we use $\ff^f_{2}(e_4)\leq \epsilon_{d2}^f$ because of the error in demand for $t_1$ in $G^f$ again by Eq. \eqref{eqn:2cffa_error_demand_s_t} in Definition \ref{def: 2cffa-new}.
			For step (3), we use the error in congestion for $e_4$ and $e_5$ in $G^f$.
			
			Next, for flow of commodity 2, i.e., $i=2$, Eq. \eqref{eq: slu-lu-s1} can be further bounded as
			\begin{equation}
				\label{eq: slu-lu-s1(2)}
				\begin{aligned}
					\left|\ff^f_2(e_1)-\ff^f_2(e_3)\right|&\leq2\epsilon_{d2}^f+\left|\ff^f_2(e_4)-\ff^f_2(e_5)\right|\\
					&\overset{(1)}{\leq} 2\epsilon_{d2}^f+\epsilon_{d2}^f \\
					&=3\epsilon_{d2}^f.
				\end{aligned}
			\end{equation}
			
			For step (1), we use $\ff^f_{2}(e_4)\leq \epsilon_{d2}^f, \ff^f_{2}(e_5)=0$ with the same reasons as explained before.
		
			\paragraph{Case 2:} 
			In the case of $\hat{e}\in S_2$, $\hat{e}_4$ and $\hat{e}_5$ are incident to $t_2$ and $s_2$, respectively. Using the same strategy as that of case 1, we can obtain the following bounds directly by symmetry:
			\begin{equation}
				\label{eq: slu-lu-s2(1)}
				\abs{\ff^f_1(\hat{e}_1)-\ff^f_1(\hat{e}_3)}\leq 3\epsilon_{d1}^f,
			\end{equation}			
			\begin{equation}
				\label{eq: slu-lu-s2(2)}
				\abs{\ff^f_2(\hat{e}_1)-\ff^f_2(\hat{e}_3)}\leq2\epsilon_{d2}^f+(\epsilon_l^f+\epsilon_u^f)\uu^s(\hat{e})+\epsilon_{d1}^f.
			\end{equation}

			Finally, applying Eq. \eqref{eq: slu-lu-s1(1)} and Eq. \eqref{eq: slu-lu-s2(1)} to Eq. \eqref{eq: slu-lu}, we obtain
			\begin{equation}
				\label{eq: slu-lu-d1}
				\begin{aligned}
					\tau_{d1}^s&\leq \epsilon_{d1}^f+\max_{y\in V^s\backslash\{s_1,t_1\}}\left\{\sum_{e=(x,y)\in S_1}\abs{\ff^f_1(e_1)-\ff^f_1(e_3)}+\sum_{\hat{e}=(x,y)\in S_2}\abs{\ff^f_1(\hat{e}_1)-\ff^f_1(\hat{e}_3)}\right\}\\
					&\leq \epsilon_{d1}^f+\max_{y\in V^s\backslash\{s_1,t_1\}}\left\{\sum_{e=(x,y)\in S_1}\left(2\epsilon_{d1}^f+(\epsilon_l^f+\epsilon_u^f)\uu^s(e)+\epsilon_{d2}^f\right)+\sum_{\hat{e}=(x,y)\in S_2}3\epsilon_{d1}^f\right\}\\
					&\leq \epsilon_{d1}^f+|S_1|(2\epsilon_{d1}^f+\epsilon_{d2}^f+(\epsilon_l^f+\epsilon_u^f)\norm{\uu^s}_{max})+|S_2|\cdot 3\epsilon_{d1}^f\\
					&=(2|S_1|+3|S_2|+1)\epsilon_{d1}^f+|S_1|\epsilon_{d2}^f+|S_1|\norm{\uu^s}_{max}(\epsilon_l^f+\epsilon_u^f)\\
					&\leq 3(|S_1|+|S_2|)\left(\epsilon^f_{d1}+\epsilon^f_{d2}+\norm{\uu^s}_{max}(\epsilon_l^f+\epsilon_u^f)\right),
				\end{aligned}
			\end{equation}			
			where we use $|S_1|\geq 1$ in the last inequality.	
%				where $u^s_{max}=\max_{e\in S} \uu^s(e)$.			
			
		 Similarly, applying Eq. \eqref{eq: slu-lu-s1(2)} and Eq. \eqref{eq: slu-lu-s2(2)} to Eq. \eqref{eq: slu-lu}, we obtain
		 \begin{equation}
			 	\label{eq: slu-lu-d2}
			 	\begin{aligned}
			 		\tau_{d2}^s&\leq \epsilon_{d2}^f+\max_{y\in V^s\backslash\{s_2,t_2\}}\left\{\sum_{e=(x,y)\in S_1}\abs{\ff^f_2(e_1)-\ff^f_2(e_3)}+\sum_{\hat{e}=(x,y)\in S_2}\abs{\ff^f_2(\hat{e}_1)-\ff^f_2(\hat{e}_3)}\right\}\\
			 		&\leq \epsilon_{d2}^f+\max_{y\in V^s\backslash\{s_2,t_2\}}\left\{\sum_{e=(x,y)\in S_1}3\epsilon_{d2}^f+\sum_{\hat{e}=(x,y)\in S_2}\left(2\epsilon_{d2}^f+(\epsilon_l^f+\epsilon_u^f)\uu^s(e)+\epsilon_{d1}^f\right)\right\}\\
			 		&\leq \epsilon_{d2}^f+|S_1|\cdot 3\epsilon_{d2}^f+|S_2|(2\epsilon_{d2}^f+\epsilon_{d1}^f+(\epsilon_l^f+\epsilon_u^f)\norm{\uu^s}_{max})\\
			 		&=(2|S_2|+3|S_1|+1)\epsilon_{d2}^f+|S_2|\epsilon_{d1}^f+|S_2|\norm{\uu^s}_{max}(\epsilon_l^f+\epsilon_u^f)\\
			 		&\leq 3(|S_1|+|S_2|)\left(\epsilon^f_{d1}+\epsilon^f_{d2}+\norm{\uu^s}_{max}(\epsilon_l^f+\epsilon_u^f)\right), 
			 	\end{aligned}
		 \end{equation}
		 	where we use $|S_2|\geq 1$ in the last inequality.
		 	\\
		 	\\
		 	Having computed the error in demand for vertices other than $s_i, t_i$, now we compute the error in demand for the sources and sinks in $G^s$.
		 	
		 	%For sources $s_1$ and $s_2$, as there is no error in demand for $s_1$ and $s_2$ in $G^f$ by definition \ref{def: 2cffa}, there is also no error in demand for $s_1$ and $s_2$ in $G^s$, which validates definition \ref{def: sffa} of \textsc{sffa}. 
		 	\ming{check} 
		 	For source $s_1$, it is noticed that all outgoing flows of $s_1$ in $G^f$ cannot route commodity 2 because there is no error in demand for $s_1$ in $G^f$ by Eq. \eqref{eqn:2cffa_error_demand_s_t} in Definition \ref{def: 2cffa-new}. As we map back by setting $\ff^s(e)=\ff^f(e_1)$ for a selective edge $e$ and map back trivially for non-selective edges, there is no error in demand for $s_1$, which validates Eq. \eqref{eqn:sffa_error_demand_s_t} in Definition \ref{def: sffa-new} about \textsc{sffa}. Similarly, there is no error in demand for $s_2$.
			
			For sinks $t_1$ and $t_2$, we compute the error in demand for $t_1$ first, and that of $t_2$ can be obtained directly by symmetry. 
			We denote the error in demand for sink $t_1$ by $\bar{\tau}_{d2}^s$, and by Eq. \eqref{eqn:sffa_error_demand_s_t} in Definition \ref{def: sffa-new}, it can be computed as
				\begin{equation}
					\label{eq: lslu-lu-t}
					\begin{aligned}
						\bar{\tau}_{d2}^s=&\sum_{(x,t_1) \in E^s}\ff^s_2(x,t_1)\\
						\overset{(1)}{=}&\sum_{(x,t_1) \in S}\ff^s_2(x,t_1)+\sum_{(x,t_1) \in E^s\backslash S}\ff^s_2(x,t_1)\\
						\overset{(2)}{=}&\sum_{e=(x,t_1) \in S}\ff^f_2(e_1)+\sum_{(x,t_1) \in E^s\backslash S}\ff^f_2(x,t_1)\\
						\overset{(3)}{\leq}&\sum_{e=(x,t_1) \in S}\ff^f_2(e_1)+\left(\epsilon^f_{d2}-\sum_{e=(x,t_1) \in S}\ff^f_2(e_3)-\sum_{e \in S_1}\ff^f_2(e_4)\right)\\
						\overset{(4)}{\leq}&\epsilon^f_{d2}+\abs{\sum_{e=(x,t_1) \in S}(\ff^f_2(e_1)-\ff^f_2(e_3))}\\ 
						\overset{(5)}{\leq}& \tau_{d2}^s.
					\end{aligned}
				\end{equation}
			For step (1), we separate non-selective incoming edges from selective incoming edges of sink $t_1$.
			For step (2), we apply the rule of mapping $\ff^f$ back to $\ff^s$.
			For step (3), it comes from the error in demand of $t_1$ in $G^f$, where the incoming edges of $t_1$ include: $e_4$ of all selective edges for commodity 1; $e_3$ of all selective edges that incident to $t_1$; all non-selective edges that incident to $t_1$, i.e.,
			\ming{check}
			\[\sum_{(x,t_1)\in E^f}\ff^f_2(x,t_1)=\sum_{e \in S_1}\ff^f_2(e_4)+\sum_{e=(x,t_1) \in S}\ff^f_2(e_3)+\sum_{(x,t_1) \in E^s\backslash S}\ff^f_2(x,t_1)\leq \epsilon^f_{d2}.\]
			For step (4), we use $\sum_{e \in S_1}\ff^f_2(e_4)\geq 0$.
			For step (5), we apply Eq. \eqref{eq: slu-lu-d2}, where we have
			\[\tau^s_{d2}=\epsilon^f_{d2}+\max_{y\in V^s\backslash\{s_2,t_2\}}\abs{\sum_{e=(x,y)\in S}(\ff^f_2(e_1)-\ff^f_2(e_3))}.\]
			
			Therefore, Eq. \eqref{eq: lslu-lu-t} indicates that error in demand of $t_1$ that can be achieved can be bounded by $\tau^s_{d2}$. 				
			By symmetry, we have error in demand of $t_2$ that can be achieved can also be bounded $\tau^s_{d1}$, i.e., $\bar{\tau}^s_{d1}\leq \tau^s_{d1}$. Thus, we can unify the error in demand for sinks and other non-fixed flow vertices. 
			
			
			\item Error in type.\\
			%According to Definition \ref{def: sffa}, 
			By Eq. \eqref{eqn:sffa_error_type} in Definition \ref{def: sffa-new}, error in type for edges selecting commodity $i$ that we can achieve is computed as 
			\begin{equation*}
				\label{eq: slu-t}
				\begin{aligned}
					\tau_{ti}^s=\max_{e\in S_i}\ff^s_{\bar{i}}(e)&=\max_{e\in S_i}\ff^f_{\bar{i}}(e_1)\\
					&\leq \max_{e\in S_i}(\ff^f_{\bar{i}}(e_1)+\ff^f_{\bar{i}}(e_2)) && \text{Becasue $\ff^f_{\bar{i}}(e_2)\geq 0$}
				\end{aligned}
			\end{equation*}
			Again, we first compute $\tau^s_{t1}$, $\tau^s_{t2}$ can be obtained directly by symmetry. 
			For an arbitrary edge $e=(x,y)\in S_1$, it is known that $e_4$ and $e_5$ are incident to $t_1$ and $s_1$.
			By error in demand on vertex $xy$, we have
			\[\abs{\ff^f_2(e_1)+\ff^f_2(e_2)-\ff^f_2(e_4)}\leq \epsilon_{d2}^f.\]
			As $\ff^f_2(e_4)\leq \epsilon_{d2}^f$ because of error in demand for $t_1$ in $G^f$, then we can bound
			\[\ff^f_2(e_1)+\ff^f_2(e_2)\leq 2\epsilon_{d2}^f.\]
			Since $e$ is an arbitrary edge in $S_1$, thus
			\begin{equation}
				\label{eq: slu-lu-t1}
				\tau_{t1}^s\leq 2\epsilon_{d2}^f.
			\end{equation}
			
			By symmetry, we also have
			\begin{equation}
				\label{eq: slu-lu-t2}
				\tau_{t2}^s\leq 2\epsilon_{d1}^f.
			\end{equation}		
			
		\end{enumerate}
	
		Now, we prove that $\ff^s$ solves the \textsc{sffa} instance by showing the the error achieved by $\ff^s$ is less than the error target set in the \textsc{sffa} instance.
		Combining Eq. \eqref{eq: slu-lu-u}, \eqref{eq: slu-lu-l}, \eqref{eq: slu-lu-d1}, \eqref{eq: slu-lu-d2}, \eqref{eq: slu-lu-t1}, \eqref{eq: slu-lu-t2}, we have
		\begin{align*}
				\tau^s_u&\leq \epsilon^f_u,\\
				\tau_l^s&\leq \epsilon_l^f+\epsilon_{d1}^f+\epsilon_{d2}^f,\\
				\tau^s_{d1}, \tau^s_{d2}&\leq 3(|S_1|+|S_2|)\left(\epsilon_{d1}^f+\epsilon_{d2}^f+\norm{\uu^s}_{max}(\epsilon_l^f+\epsilon_u^f)\right),\\
				\tau^s_{t1}&\leq 2\epsilon^f_{d2},\\
				\tau^s_{t2}&\leq 2\epsilon^f_{d1}.
		\end{align*}
	
		As we set in the reduction that $\epsilon_l^f=\min\left\{\frac{\epsilon^s_l}{2}, \frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}\right\},
		\epsilon_u^f=\min\left\{\epsilon_u^s, \frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}\right\},\\
		\epsilon^f_{d1}= \min\left\{\frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)},\frac{\epsilon^s_l}{4}, \frac{\epsilon^s_{t2}}{2}\right\},
		\epsilon^f_{d2}= \min\left\{\frac{\min\{\epsilon^s_{d1},\epsilon^s_{d2}\}}{12(|S_1|+|S_2|)}, \frac{\epsilon^s_l}{4}, \frac{\epsilon^s_{t2}}{2}\right\}$, then we have			
		\[\tau^s_u\leq \epsilon^f_u\leq \epsilon^s_u,\]
		\begin{align*}
			\tau_l^s\leq \epsilon_l^f+\epsilon_{d1}^f+\epsilon_{d2}^f
			\leq \frac{\epsilon^s_l}{2}+\frac{\epsilon^s_l}{4}+\frac{\epsilon^s_l}{4}
			=\epsilon^s_l,
		\end{align*}
		\begin{small}
		\begin{multline*}
			\tau_{d1}^s\leq 3(|S_1|+|S_2|)\left(\frac{\epsilon^s_{d1}}{12(|S_1|+|S_2|)}+\frac{\epsilon^s_{d1}}{12(|S_1|+|S_2|)}\right.\\ 				
			\phantom{=\;\;}\left.  +\norm{\uu^s}_{max}\left(\frac{\epsilon^s_{d1}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}+\frac{\epsilon^s_{d1}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}\right)\right)
			\leq \epsilon_{d1}^s,
		\end{multline*}
		\end{small}
		\begin{small}
			\begin{multline*}
				\tau_{d2}^s\leq 3(|S_1|+|S_2|)\left(\frac{\epsilon^s_{d2}}{12(|S_1|+|S_2|)}+\frac{\epsilon^s_{d2}}{12(|S_1|+|S_2|)}\right.\\ 				
				\phantom{=\;\;}\left. +\norm{\uu^s}_{max}\left(\frac{\epsilon^s_{d2}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}+\frac{\epsilon^s_{d2}}{12(|S_1|+|S_2|)\norm{\uu^s}_{max}}\right)\right)
				\leq \epsilon_{d2}^s,
			\end{multline*}
		\end{small}
		\[\tau^s_{t1}\leq\epsilon^s_{t1}, \qquad \tau^s_{t2}\leq\epsilon^s_{t2}.\]
		
		Thus, we can conclude that if $\ff^f$ is a solution to the \textsc{2cffa} instance with the error $\epsilon^f_l,\epsilon^f_u,\epsilon^f_{d1}, \epsilon^f_{d2}$ as set in the reduction, we can map it back to a solution $\ff^s$ to the \textsc{sffa} instance with its error target achieved.
\end{proof}

\subsection{2CFF(A) to 2CFR(A)}
\label{sect: 2cffa-2cfra}
\subsubsection{2CFF to 2CFR}
We show the reduction from a \textsc{2cff} instance $(G^f, F^f, \uu^f, s_1,t_1, s_2,t_2)$ to a \textsc{2cfr} instance \\$(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2)$. 
First of all, we add two new sources $\bar{s}_1, \bar{s}_2$ and two new sinks $\bar{t}_1, \bar{t}_2$. Then, for each edge $e\in E^f$, we map it to a gadget consisting edges $\{e_1,e_2,e_3,e_4,e_5, e_6,e_7\}$ in $G^{r}$, as shown in the upper part of Figure \ref{fig: lu2cf-2cfr}. Additionally, there is another gadget with 5 edges in $G^r$ that connects the original sink $t_i$ and source $s_i$, as shown in the lower part of Figure \ref{fig: lu2cf-2cfr}. Capacity of these edges is the sum capacities of all edges in $G^f$, i.e., $M^f=\sum_{e\in E^f} \uu^f(e)$. 
Additionally, we set $R_1=R_2=2M^f$, indicating that at least $2M^f$ unit of flow should be routed from $\bar{s}_i$ to $\bar{t}_i$, $i\in\{1,2\}$. 
%Finally, as no reduction is performed on non-fixed flow edges in $E^f\backslash F^f$, we trivially copy these edges to $G^r$.

The key idea to remove the fixed flow constraint is utilizing edge directions and the requirements that $2M^f$ units of flow of commodity $i$ to be routed from the new source $\bar{s}_i$ to the new sink $\bar{t}_i$, $i\in\{1,2\}$.
It is noticed that all edges that are incident to the new sources and sinks should be saturated to fulfill the requirements. Therefore, in the first gadget for a fixed flow edge $e$, the incoming flow of vertex $xy'$ and the outgoing flow of vertex $xy$ must be $2u$. Since the capacity of $e_2$ is $2u-u=u$, then the flow of $e_1, e_2, e_3$ are forced to be $u$. As such, the fixed flow constraint can be simulated. 
Note that instead of simply copying non-fixed flow edges to $G^r$, we also need to map non-fixed flow edges to the designed gadget in this step. \ming{more explanation?}


\begin{figure}[t]
	\centering
	\includegraphics[width=\textwidth]{image/lu2CF-2CFR}
	\caption{The reduction from \textsc{2cff} to \textsc{2cfr}. $l=u$ if $e$ is a fixed flow edge, and $l=0$ if $e$ is a non fixed flow edge.} 
	\label{fig: lu2cf-2cfr}
\end{figure}

If a \textsc{2cfr} solver returns $\ff^r$ for the \textsc{2cfr} instance $(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2)$, then we return $\ff^f$ for the \textsc{2cff} instance $(G^f, F^f, \uu^f, s_1,t_1, s_2,t_2)$ by setting $\ff_i^f(e)=\ff^r_i(e_1), \forall e\in E^f, i\in\{1,2\}$.


\begin{lemma}[\textsc{2cff} to \textsc{2cfr}]
	\label{lm: 2cff-2cfr}
	Given a \textsc{2cff} instance $(G^f, F^f, \uu^f, s_1,t_1, s_2,t_2)$,
	we can construct, in time $O(|E^f|)$, a \textsc{2cfr} instance $(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2)$ such that
	\[|V^r|=|V^f|+2|E^f|+8,\qquad |E^r|=7|E^f|+10,\qquad \norm{\uu^r}_{max}= \max\left\{2\norm{\uu^f}_{max}, M^f\right\},\] 
	\[R_1=R_2=2M^f,\]
	where $M^f=\sum_{e\in E^f} \uu^f(e)$. 
	If the \textsc{2cff} instance has a solution, then the \textsc{2cfr} instance has a solution.
	%	and if $\ff^h$ is a solution to the FHF instance, then in time $O(\hat{n})$, we can compute a solution $\hat{\xx}$ to the 1-LEN instance.
\end{lemma}	
\begin{proof}
	According to the reduction described above, from any solution $\ff^f$ to the \textsc{2cff} instance, it is easy to derive a solution $\ff^r$ to the \textsc{2cfr} instance. Concretely, we define a feasible flow $\ff^r$ as follows. For any edge $e\in E^f$, we set:

		\[\ff^r_i(e_1)=\ff^r_i(e_3)=\ff^f_i(e), \qquad i\in\{1,2\},\]
		\[\ff^r_i(e_2)=u-\ff^f_i(e), \qquad i\in\{1,2\},\]
		\[\ff^r_1(e_4)=\ff^r_1(e_6)=u, \qquad \ff^r_2(e_5)=\ff^r_2(e_7)=u,\]
		\[\ff^r_2(e_4)=\ff^r_2(e_6)= \ff^r_1(e_5)=\ff^r_1(e_7)=0,\]
		where $u=\uu^f(e)$.
		And we set
		\[\ff^r_i(t_i, z_i)=\ff^r_i(z'_i,s_i)=\sum_{\begin{subarray}{c}
				w:
				(s_i, w)\in E^f
		\end{subarray}}\ff_i^f(s_i, w)\leq M^f,\qquad i\in\{1,2\},\]
		\[\ff^r_i(z'_i, z_i)=M^f-\sum_{\begin{subarray}{c}
				w:
				(s_i, w)\in E^f
		\end{subarray}}\ff_i^f(s_i, w),\qquad i\in\{1,2\},\]
		\[\ff^r_i(\bar{s}_i,z'_i)=\ff^r_i(z_i,\bar{t}_i)=M^f, \qquad i\in\{1,2\},\]
		\[\ff^r_{\bar{i}}(t_i, z_i)=\ff^r_{\bar{i}}(z'_i,s_i)=\ff^r_{\bar{i}}(z'_i, z_i)=\ff^r_{\bar{i}}(\bar{s}_i,z'_i)=\ff^r_{\bar{i}}(z_i,\bar{t}_i)=0,\qquad \bar{i}\in\{1,2\}\backslash i.\]
		
		Now, we prove that $\ff^r$ is a solution to the \textsc{2cfr} instance. 
		\begin{enumerate}
			\item Capacity constraint.\\
			Only the capacity constraint on edge $e_2$ is nontrivial. 
			\begin{itemize}
				\item If $e$ is a fixed flow edge, then we have $l=u$, thus the capacity of $e_2$ is $u$. By construction, we have 
				\[\sum_{i=\{1,2\}}\ff^r_i(e_2)=2u-\sum_{i=\{1,2\}}\ff^f_i(e)=2u-u=u,\]
				where we use $\sum_{i=\{1,2\}}\ff^f_i(e)=u$.
				
				\item If $e$ is a non-fixed flow edge, then we have $l=0$, thus the capacity of $e_2$ is $2u$.
				By construction, we have
				\[\sum_{i=\{1,2\}}\ff^r_i(e_2)=2u-\sum_{i=\{1,2\}}\ff^f_i(e)\leq 2u,\]
				where we use $\sum_{i=\{1,2\}}\ff^f_i(e)\geq 0$.
			\end{itemize}
			Therefore, we conclude that $\ff^r$ fulfills the capacity constraint.	
			
			\item Flow conservation constraint.\\
			Only the flow conservation constraint on vertices $xy, xy', z_i, z'_i$ are nontrivial.
			\begin{itemize}
				\item For vertex $xy$, we have
				\[\ff^r_1(e_1)+\ff^r_1(e_2)=\ff^f_1(e)+(u-\ff^f_1(e))=u=\ff^r_1(e_4),\]
				and 
				\[\ff^r_2(e_1)+\ff^r_2(e_2)=\ff^f_2(e)+(u-\ff^f_2(e))=u=\ff^r_2(e_5).\]
				We can prove for vertex $xy'$ similarly.
				\item For vertex $z_i, i\in\{1,2\}$, we have
				\begin{align*}
					\ff^r_i(t_i, z_i)+\ff^r_i(z'_i, z_i)&=\sum_{\begin{subarray}{c}
							w:
							(s_i, w)\in E^f
					\end{subarray}}\ff_i^f(s_i, w)+\left(M^f-\sum_{\begin{subarray}{c}
							w:
							(s_i, w)\in E^f
					\end{subarray}}\ff_i^f(s_i, w)\right)\\
					&=M^f=\ff^r_i(z_i,\bar{t}_i).
				\end{align*}
				We can prove for vertex $z'_i$ similarly.
			\end{itemize}
			Therefore, we conclude that $\ff^r$ fulfills the flow conservation constraint.	
			
			\item Requirement $R_1=R_2=2M^f$.\\
			For commodity 1, we have
			\[R_1=\sum_{\begin{subarray}{c}
					w:
					(\bar{s}_1, w)\in E^r
			\end{subarray}}\ff_1^r(\bar{s}_1, w)=\ff^r(\bar{s}_1, z'_1)+\sum_{e\in E^f}\ff^r_1(e_6)=M^f+\sum_{e\in E^f}\uu^f(e)=2M^f,\]
			\[R_1=\sum_{\begin{subarray}{c}
					u:
					(u,\bar{t}_1)\in E^r
			\end{subarray}}\ff_1^r(u,\bar{t}_1)=\ff^r(z_1, \bar{t}_1)+\sum_{e\in E^f}\ff^r_1(e_4)=M^f+\sum_{e\in E^f}\uu^f(e)=2M^f.\]
			We can prove that the requirement $R_2=2M^f$ is satisfied similarly.
		\end{enumerate}
	To conclude, $\ff^r$ is a feasible flow to the \textsc{2cfr} instance.
	\\
	\\
	Now, we track the change of problem size after reduction. Based on the reduction method, given a \textsc{2cff} instance with $|V^f|$ vertices and $|E^f|$ edges (including $|F^f|$ fixed flow edges), we can compute the size of the reduced \textsc{2cfr} instance as follows.
	\begin{enumerate}
		\item $|V^r|$ vertices. First, all vertices in $V^f$ are maintained.
		Then, for each edge $e=(x,y)$, two new auxiliary vertices $xy, xy'$ are added.
		And finally, in the second gadget, $\{\bar{s}_i, \bar{t}_i, z_i, z_i'\}, i\in\{1,2\}$ are added. Hence, we have
		\[|V^r|=|V^f|+2|E^f|+8.\]
		
		\item $|E^r|$ edges. First, each edge $e\in E^f$ is replaced by the first gadget in Figure \ref{fig: lu2cf-2cfr} with 7 edges $(e_1, \ldots, e_7)$.
		Then, 5 edges are added between $t_i$ and $s_i$ according to the second gadget in Figure \ref{fig: lu2cf-2cfr}, $i\in\{1,2\}$. Thus, we have
		\[|E^r|=7|E^f|+10.\]
		
		\item The maximum edge capacity is bounded by
		\[\norm{\uu^r}_{max}=\max\left\{2\norm{\uu^f}_{max}, M^f\right\}.\]			
		For all fixed flow edges $e\in F^f$ with fixed flow $\uu^f(e)$, the 7 edges $(e_1, \ldots, e_7)$ in the first gadget are all with capacity $\uu^f(e)$.
		For all non-fixed flow edges in $e\in E^f\backslash F^f$ with capacity $\uu^f(e)$, the capacity of $e_2$ becomes $2\uu^f(e)$ and the capacity of the rest 6 edges in the first gadget remains $\uu^f(e)$. 
		Moreover, the 5 edges in the second gadget are all with capacity $M^f$, which is the sum of the capacity of all edges.
	\end{enumerate}
	To estimate the reduction time, it is observed that it takes constant time to reduce each edge in $E^f$ since only a constant number of vertices and edges are added. Thus, the reduction of this step takes $O(|E^f|)$ time.
\end{proof}	

\subsubsection{2CFFA to 2CFRA}
The above lemma shows the reduction between exactly solving a \textsc{2cff} instance and exactly solving a \textsc{2cfr} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.
First of all, we give a definition of the approximate version of \textsc{2cfr}.


\begin{definition}[2CFR Approximate Problem (\textsc{2cfra})]
	\label{def: 2cfra-new}
	A \textsc{2cfra} instance is given by a \textsc{2cfr} instance $(G, \uu, s_1,t_1, s_2,t_2,R_1,R_2)$ as in Definition \ref{def: 2cfr}, and error parameters $\epsilon \in[0,1]$, $\epsilon_1, \epsilon_2\geq 0$, which we collect in a tuple $\left(G, \uu, s_1,t_1, s_2,t_2,R_1,R_2,\epsilon, \epsilon_1, \epsilon_2 \right)$.
	We say an algorithm solves the \textsc{2cfra} problem, if, given any \textsc{2cfra} instance, it returns a pair of flows $\ff_1, \ff_2\geq\bf{0}$ (denote $\ff=\ff_1+\ff_2$) that satisfies
	\begin{align}
		&0\leq \ff_1(e)+\ff_2(e)\leq(1+\epsilon)\uu(e), ~~ \forall e \in E \label{eqn:2cfra_error_congestion} \\
		&F_i\geq R_i-\epsilon_i, ~~ i\in\{1,2\} \label{eqn:2cfra_requirement}
%		&F_1+F_2=R_1+R_2 \label{eqn:2cfra_requirement_2} 
	\end{align}
	\ming{check}
	or it correctly declares that the associated \textsc{2cfr} instance is infeasible. We refer to the error in \eqref{eqn:2cfra_error_congestion} as error in congestion, and the error in \eqref{eqn:2cfra_requirement} as error in requirement.
\end{definition}	

We can use the same reduction method and solution mapping method in the exact case to the approximate case.


\begin{lemma}[\textsc{2cffa} to \textsc{2cfra}]
	\label{lm: lu2cfa-2cfra}
	Given a \textsc{2cffa} instance $\left(G^f,F^f, \uu^f, s_1,t_1,s_2,t_2, \epsilon^f_l, \epsilon^f_u,\epsilon^f_{d1},\epsilon^f_{d2}\right)$, we can construct, in $O(|E^s|)$ time, a \textsc{2cfra} instance $\left(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2,\bar{t}_2,R_1,R_2,\epsilon^r,\epsilon_1^r, \epsilon_2^r \right)$ such that
	\[|V^r|=|V^f|+2|E^f|+8,\qquad |E^r|=7|E^f|+10,\qquad \norm{\uu^r}_{max}= \max\left\{2\norm{\uu^f}_{max}, M^f\right\},\] 
	\[R_1=R_2=2M^f,\]
	and	
	\[\epsilon^r= \min\left\{ \frac{\epsilon^f_l}{12M^f}, ~\epsilon^f_u,~ \frac{\epsilon^f_{d1}}{8M^f}, ~\frac{\epsilon^f_{d2}}{8M^f}\right\},\qquad \epsilon^r_1=\min\left\{ \frac{\epsilon^f_l}{3}, ~ \frac{\epsilon^f_{d1}}{4}\right\},\qquad \epsilon^r_2=\min\left\{ \frac{\epsilon^f_l}{3}, ~ \frac{\epsilon^f_{d2}}{4}\right\},\]
	where $M^f=\sum_{e\in E^f} \uu^f(e)$.	
	If the \textsc{2cff} instance $\left(G^f,F^f, \uu^f, s_1,t_1,s_2,t_2\right)$  has a solution, then the \textsc{2cfra} instance $\left(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2,\bar{t}_2,R_1,R_2\right)$ has a solution.
	Furthermore, if $\ff^r$ is a solution to the \textsc{2cfra} instance, then in time $O(|E^f|)$, we can compute a solution $\ff^f$ to the \textsc{2cffa} instance.

%	Given a \textsc{2cffa} instance $(G^f,\ll^f,\uu^f,\epsilon_l^f,\epsilon_u^f,\epsilon_{d1}^f,\epsilon_{d2}^f)$, it can be reduced to a \textsc{2cfra} instance $(G^r, \uu^r, R_1,R_2, \epsilon^r)$ in $O(|E^f|)$ time, such that $G^r$ has $|V^r|=O(|V^r|+|E^f|)$ vertices and $|E^r|=O(|E^f|)$ edges.
%	If there is a \textsc{2cfra} solver with $\epsilon^r$ error in congestion, then it can be translated into a \textsc{2cffa} solver with 
%	\begin{itemize}
%		\item $((1-\epsilon_l)l, (1+\epsilon_u)u)$ error in congestion, where
%		\[\epsilon_l=O\left(\frac{M^f}{u_{min}^f}\epsilon^r\right),\qquad \epsilon_u=\epsilon^r;\]
%		\item $\epsilon_{di}, i\in\{1,2\}$ error in demand for commodity $i$, where
%		\[\epsilon_{di}=O(M^f\epsilon^r).\]
%	\end{itemize}
\end{lemma}	

\begin{proof}
	Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: 2cff-2cfr} also apply here, including the reduction time, problem size, and that \textsc{2cfr} has a feasible solution when \textsc{2cff} has one. 
	It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{2cfra} back to an approximate solution to \textsc{2cffa}.
	
	Based on the solution mapping method described above, it takes constant time to set the value of each of $\ff^f$, and $\ff^f$ has $|E^f|$ entries, such a solution mapping takes $O(|E^f|)$ time.	
	
%		Based on the reduction described above, we observe that given a \textsc{2cffa} instance with $|V^f|$ vertices and $|E^f|$ edges (including $|F^f|$ fixed flow edges), it can be reduced to a \textsc{2cfra} instance with
		
%		\item \textbf{Reduction time}\\
%		It takes a constant time to reduce each fixed flow edge in $F^f$, and constant time to connect $t_i$ and $s_i$ since only a constant number of vertices and edges are added. And it also takes constant time to copy each of the other edges. Therefore, the reduction of this step takes $O(|E^f|)$ time.
		
%		\item \textbf{Solution mapping and error analysis}\\
%		Given a solution $\ff^r$ returned by the \textsc{2cfra} solver, we map the solution back to $G^f$ by the following rule: for any fixed flow edge $e\in F^f$, we set $\ff_i^f(e)=\ff^r_i(e_1), i\in\{1,2\}$; and for any non-fixed flow edge $e\in E^f\backslash F^f$, we map back trivially by setting $\ff^f_i(e)=\ff^r_i(e), i\in\{1,2\}$.
%		As there are $|E^f|$ entries to set value, it takes $O(|E^{f}|)$ time to map $\ff^{r}$ back to $\ff^f$. 
		Now, we conduct error analysis. The mapping will generate two types of error: (1) error in congestion; (2) error in demand.
		
		\begin{enumerate}
			\item Error in congestion.\\ 
%			Since we map solution back trivially for non-fixed flow edges in $E^f\backslash F^f$, error in congestion of $G^r$ (i.e., $\epsilon^r_l, \epsilon^r_u$) still hold for $G^f$. Therefore, we focus on how error in congestion changes when mapping solution back to fixed flow edges in $F^f$.			
			We first track the error of the upper bound of capacity. For any edge $e\in E^f$, the maximum flow to be routed in $e$ is
			\[(1+\tau_u^f)\uu^f(e)=\sum_{i=\{1,2\}}\ff_i^f(e)=\sum_{i=\{1,2\}}\ff^r_i(e_1)\leq (1+\epsilon^r)\uu^r(e_1)=(1+\epsilon^r)\uu^f(e),\]
			thus, 
			\[\tau_u^f\leq \epsilon^r.\]
%			As error in congestion for $G^r$ is bounded by $\epsilon^r$, we have
%			\[\sum_{i=\{1,2\}}\ff^r_i(e_1)\leq (1+\epsilon^r)\uu^r(e_1)=(1+\epsilon^r)\uu^f(e),\]
%			Hence, the upper error $\tau_u^f$ in $G^f$ can be bounded by
%			\[\sum_{i=\{1,2\}}\ff_i^f(e)=(1+\tau_u^f)\uu^f(e)\leq (1+\epsilon^r)\uu^f(e) \Rightarrow \tau_u^f\leq \epsilon^r.\]
			As we set $\epsilon^r\leq \epsilon_u^f$ in the reduction, it indicates that $\tau_u^f\leq \epsilon_u^f$.
			
			
			Next, we track the error of the lower bound of capacity. Note that we only need to take fixed flow edges into account since the lower capacity bound for non-fixed flow edges is 0. 
%			To satisfy the demand requirements in $G^r$, the incoming flow of $\bar{t}_1$ and $\bar{t}_2$ should equal to $2M^f$ because it is the maximum flow that can be routed for each commodity, i.e.,
			By error in congestion as shown in Eq. \eqref{eqn:2cfra_error_congestion} and error in requirement as shown in Eq. \eqref{eqn:2cfra_requirement}, as well as $R_1=R_2=2M^f$, we have
			\[2M^f-\epsilon^r_1\leq \sum_{e\in E^f}\ff^r_1(e_4)+\ff^r(z_1, \bar{t}_1)\leq 2(1+\epsilon^r)M^f,\]
			\[2M^f-\epsilon^r_2\leq \sum_{e\in E^f}\ff^r_2(e_5)+\ff^r(z_2, \bar{t}_2)\leq2(1+\epsilon^r)M^f,\]
			%		\[\sum_{e\in E^f}\ff^r_1(e_6)+\ff^r(\bar{s}_1,z_1')=2M^f,\]
			%		\[\sum_{e\in E^f}\ff^r_2(e_7)+\ff^r(\bar{s}_2,z_2')=2M^f.\]
			
			We now try to compute the minimum flow that can be routed through any fixed flow edge in $F^f$. For an arbitrary $\hat{e}\in F^f$, we can rearrange the above equations and have
			\begin{align*}
				\ff^r_1(\hat{e}_4)&\geq 2M^f-\epsilon^r_1-\sum_{e\in E^f\backslash\hat{e}}\ff^r_1(e_4)-\ff^r(z_1, \bar{t}_1)\\
				&\geq \max\left\{0, 2M^f-\epsilon^r_1-\sum_{e\in E^f\backslash\hat{e}}(1+\epsilon^r)\uu^f(e)-(1+\epsilon^r)M^f\right\} && \text{$\epsilon^r$ error in congestion in $G^r$}\\
				&=\max\left\{0, 2M^f-\epsilon^r_1-(1+\epsilon^r)(2M^f-\uu^f(\hat{e}))\right\} && \text{Because $M^f=\sum_{e\in E^f}\uu^f(e)$}\\
				&=\max\left\{0,(1+\epsilon^r)\uu^f(\hat{e})-2M^f\epsilon^r-\epsilon^r_1\right\} 
			%	&=\max\left\{0,\uu^f(\hat{e})-\epsilon^r(2M^f-\uu^f(\hat{e}))\right\}
			\end{align*}
%			Here, since $G^r$ is a directed graph and edge direction should be respected to make flow feasible, then we can get a primary upper bound of $\epsilon^r$:
%			\[\epsilon^r\leq\frac{u_{min}^f}{2M^f-u_{min}^f},\]
%			where $u_{min}^f=\min_{e\in E^f}\uu(e)$.
			
			Similarly, we have
			\begin{align*}
				\ff^r_2(\hat{e}_5)&\geq2M^f-\epsilon^r_2-\sum_{e\in E^f\backslash\hat{e}}\ff^r_1(e_5)-\ff^r(z_2, \bar{t}_2) \\
				&\geq \max\left\{0,(1+\epsilon^r)\uu^f(\hat{e})-2M^f\epsilon^r-\epsilon^r_2\right\}.
			\end{align*}
			Therefore, for any fixed flow edge $\hat{e}=(x,y) \in F^f$, the minimum flow to be routed can be lower bounded by
			\begin{equation}
				\label{eq: lu2cf_1}
				\begin{aligned}
					(1-\tau_l^f)\uu^f(\hat{e})=\ff^f(\hat{e})&=\ff^r(\hat{e}_1)\\
					&\overset{(1)}{=}\ff^r_1(\hat{e}_4)+\ff^r_2(\hat{e}_5)-\ff^r(\hat{e}_2)\\
					&\overset{(2)}{\geq} \max\{0,2(1+\epsilon^r)\uu^f(\hat{e})-4M^f\epsilon^r-\epsilon^r_1-\epsilon^r_2-(1+\epsilon^r)\uu^f(\hat{e})\}\\
					&=\max\{0,(1+\epsilon^r)\uu^{f}(\hat{e})-4M^f\epsilon^r -\epsilon^r_1-\epsilon^r_2\}\\
					&=\max\left\{0,\left(1+\epsilon^r-\frac{4 M^f\epsilon^r+\epsilon^r_1+\epsilon^r_2}{\uu^f(\hat{e})}\right)\uu^f(\hat{e})\right\}\\
					&=\max\left\{0,\left(1-\left(\left(\frac{4M^f}{\uu^f(\hat{e})}-1\right)\epsilon^r+\frac{\epsilon^r_1+\epsilon^r_2}{\uu^f(\hat{e})}\right)\right)\uu^f(\hat{e})\right\}.
				\end{aligned}
			\end{equation}
			For step (1), we apply the flow conservation constraint on vertex $xy$ since there is no error in demand in $G^r$.
			For step (2), we plug in the lower bound of $\ff^r_1(\hat{e}_4), \ff^r_2(\hat{e}_5)$ that are proved previously, and the upper bound of $\ff^r_1(\hat{e}_2)$.
 			Thus, we have
			\[\tau_l^f\leq\left(\frac{4M^f}{\uu^f(\hat{e})}-1\right)\epsilon^r+\frac{\epsilon^r_1+\epsilon^r_2}{\uu^f(\hat{e})}\leq 4M^f\epsilon^r+\epsilon^r_1+\epsilon^r_2,\]
			where we use $\uu^f(\hat{e})\geq 1$ because of integer capacities.
			
			As we set in the reduction that
			\[\epsilon^r\leq \frac{\epsilon^f_l}{12M^f},~~\epsilon^r_1\leq \frac{\epsilon^f_l}{3}, ~~\epsilon^r_2\leq \frac{\epsilon^f_l}{3},\]
			thus we have 
			\[\tau_l^f\leq 4M^f\frac{\epsilon^f_l}{12M^f}+\frac{\epsilon^f_l}{3}+\frac{\epsilon^f_l}{3}\leq \epsilon^f_l.\]
			
			\item Error in demand.\\
			We focus on the error in demand for commodity 1 first, and then the error in demand for commodity 2 can be achieved directly by symmetry. 
			By Eq. \eqref{eqn:2cffa_error_demand} in Definition \ref{def: 2cffa-new}, error in demand of commodity 1 that we can achieve for vertices other than $s_1, t_1$ in $G^f$ is computed as	
			\begin{small}
			\begin{equation}
				\label{eq: lu-2cfa}
				\begin{aligned}
					\tau_{d1}^f=&\max_{y\in V^f\backslash\{s_1,t_1\}}\abs{\sum_{(x,y) \in E^f}\ff^f_1(x,y)-\sum_{(y,z) \in E^f}\ff^f_1(y,z)}\\
%					\overset{(1)}{=}&\max_{y\in V^f\backslash\{s_1,t_1\}}\abs{\left(\sum_{(x,y) \in F^f}\ff^f_1(x,y)+\sum_{(x,y) \in E^f\backslash F^f}\ff^f_1(x,y)\right)-\left(\sum_{(y,z) \in F^f}\ff^f_1(y,z)+\sum_{(y,z) \in E^f\backslash F^f}\ff^f_1(y,z)\right)}\\
					\overset{(1)}{=}&\max_{y\in V^f\backslash\{s_1,t_1\}}\abs{\sum_{e=(x,y) \in E^f}\ff^r_1(e_1)-\sum_{e=(y,z) \in E^f}\ff^r_1(e_1)}\\
%					\overset{(3)}{=}&\max_{y\in V^f\backslash\{s_1,t_1\}}\abs{\left(\sum_{e=(x,y) \in F^f}\ff^r_1(e_1)+\sum_{(x,y) \in E^f\backslash F^f}\ff^r_1(x,y)\right)-\left(\sum_{e=(x,y) \in F^f}\ff^r_1(e_3)+\sum_{(x,y) \in E^f\backslash F^f}\ff^r_1(x,y)\right)}\\
					\overset{(2)}{=}&\max_{y\in V^f\backslash\{s_1,t_1\}}\abs{\sum_{e=(x,y) \in E^f}\ff^r_1(e_1)-\sum_{e=(x,y) \in E^f}\ff^r_1(e_3)}\\
					=&\max_{y\in V^f\backslash\{s_1,t_1\}}\abs{\sum_{e=(x,y) \in E^f}\left(\ff^r_1(e_1)-\ff^r_1(e_3)\right)} \\
					\leq& \max_{y\in V^f\backslash\{s_1,t_1\}}\sum_{e=(x,y) \in E^f}\left|\ff^r_1(e_1)-\ff^r_1(e_3)\right|. 
				\end{aligned}
			\end{equation}
			\end{small}
			
			For step (1), we apply the rule of mapping $\ff^r$ back to $\ff^f$.
			For step (2), we replace the sum of outgoing flows of $y$ by the sum of its incoming flows without introducing any error because there is no error in demand in $G^r$, i.e., 
			\[\sum_{e=(y,z) \in E^f}\ff^r_1(e_1)=\sum_{e=(x,y) \in E^f}\ff^r_1(e_3).\] 
			%since $G^r$ has no demand error for vertices other than $(\bar{s}_1, \bar{s}_2,\bar{t}_1, \bar{t}_2)$.
						
			Now, we try to bound $\left|\ff^r_1(e_1)-\ff^r_1(e_3)\right|$.
			By the flow conservation constraint of vertex $xy$ and $xy'$ with respect to commodity 1, we have
			\[\ff^r_1(e_1)+\ff^r_1(e_2)=\ff^r_1(e_4),\]
			\[\ff^r_1(e_3)+\ff^r_1(e_2)=\ff^r_1(e_6).\]
			Subtracting these two equations gives
			\begin{align*}
				\left|\ff^r_1(e_1)-\ff^r_1(e_3)\right|
				=\left|\ff^r_1(e_4)-\ff^r_1(e_6)\right|,
			\end{align*}
			which can be plugged back into Eq. \eqref{eq: lu-2cfa} to give
			\[\tau_{d1}^f\leq \max_{y\in V^f\backslash\{s_1,t_1\}}\sum_{e=(x,y) \in E^f}\left|\ff^r_1(e_4)-\ff^r_1(e_6)\right|.\]
			
			The following is a claim that shows the sum of $\abs{\ff^r_1(e_4)-\ff^r_1(e_6)}$ for all edges $e\in E^f$ can be upper bounded.
			
			\begin{claim}
				\label{cl: 2cfra}
				\[\sum_{e\in E^f} \abs{\ff^r_1(e_4)-\ff^r_1(e_6)}\leq 4M^f\epsilon^r+2\epsilon^r_1.\]
			\end{claim}	

			By Claim \ref{cl: 2cfra}, we have 
			\begin{align*}
				 \tau_{d1}^f&\leq \max_{y\in V^f\backslash\{s_1,t_1\}}\sum_{e=(x,y) \in E^f}\left|\ff^r_1(e_4)-\ff^r_1(e_6)\right|\\
				&\leq \sum_{e\in E^f} \abs{\ff^r_1(e_4)-\ff^r_1(e_6)} \leq4M^f\epsilon^r+2\epsilon^r_1.
			\end{align*}
			As we set in the reduction 
			$\epsilon^r\leq \frac{\epsilon_{d1}^f}{8M^f}, \epsilon^r_1\leq \frac{\epsilon^f_{d1}}{4}$, it indicates that
			\begin{equation}
				\label{eq: lu-2cfa-d1}
				\tau_{d1}^f\leq 4M^f\frac{\epsilon_{d1}^f}{8M^f}+2\frac{\epsilon^f_{d1}}{4}=\epsilon_{d1}^f.
			\end{equation}
			
			By symmetry of the two commodities, we can also bound the error in demand for commodity 2 by
			\[\tau_{d2}^f\leq 4M^f\epsilon^r+2\epsilon^r_2.\]			
			As we set in the reduction 
			$\epsilon^r\leq \frac{\epsilon_{d2}^f}{8M^f}, \epsilon^r_2\leq \frac{\epsilon^f_{d2}}{4}$, it indicates that
			\begin{equation}
				\label{eq: lu-2cfa-d2}
				\tau_{d2}^f\leq 4M^f\frac{\epsilon_{d2}^f}{8M^f}+2\frac{\epsilon^f_{d2}}{4}=\epsilon_{d2}^f.
			\end{equation}
			\\
			Having computed the error in demand for vertices other than $s_i, t_i$, now we compute the error in demand for sources and sinks in $G^f$.
			
			For source $s_1$, it is noticed that all outgoing flows of $s_1$ in $G^r$ cannot route commodity 2 because the incoming flow of $s_1$ is only from $z'_1$ and thus from $\bar{s}_1$, where only flow of commodity 1 is allowed since there is no error in demand in $G^r$. As we map back by setting $\ff^f(e)=\ff^r(e_1)$ for a fixed flow edge $e$ and map back trivially for non-fixed flow edges, there is no error in demand for $s_1$, which validates Eq. \eqref{eqn:2cffa_error_demand_s_t} in Definition \ref{def: 2cffa-new} about \textsc{2cffa}. Similarly, there is no error in demand for $s_2$.
			
			For sinks $t_1$ and $t_2$, we compute the error in demand for $t_1$ first, and that of $t_2$ can be obtained directly by symmetry. We denote the error in demand for sink $t_1$ by $\bar{\tau}_{d2}^f$, and again by Eq. \eqref{eqn:2cffa_error_demand_s_t} in Definition \ref{def: 2cffa-new}, it can be computed as			
			\begin{small}
				\begin{equation}
					\label{eq: lu-2cfa-t}
					\begin{aligned}
						\bar{\tau}_{d2}^f=&\sum_{(x,t_1) \in E^f}\ff^f_2(x,t_1)\\
%						\overset{(1)}{=}&\sum_{(x,t_1) \in F^f}\ff^f_2(x,t_1)+\sum_{(x,t_1) \in E^f\backslash F^f}\ff^f_2(x,t_1)\\
%						\overset{(1)}{=}&\sum_{e=(x,t_1) \in F^f}\ff^r_2(e_1)+\sum_{(x,t_1) \in E^f\backslash F^f}\ff^r_2(x,t_1)\\
						\overset{(1)}{=}&\sum_{e=(x,t_1) \in E^f}\ff^r_2(e_1)\\
						\overset{(2)}{=}&\abs{\sum_{e=(x,t_1) \in E^f}(\ff^r_2(e_1)-\ff^r_2(e_3))}\\ 
						\overset{(3)}{\leq}& \tau_{d2}^f.
					\end{aligned}
				\end{equation}
			\end{small}

			For step (1), we apply the rule of mapping $\ff^r$ back to $\ff^f$.
			For step (2), we utilize the property that all incoming flows of $t_1$ in $G^r$ cannot route commodity 2, i.e., $\ff^r_2(e_3)=0$,
			because the outgoing flow of $t_1$ is only to $z_1$ and then $\bar{t}_1$, where only flow of commodity 1 is allowed. 
			For step (3), we apply the conclusion of Eq. \eqref{eq: lu-2cfa} by symmetry that $\tau_{d2}^f=\max_{y\in V^f\backslash\{s_2,t_2\}}\abs{\sum_{e=(x,y) \in E^f}\left(\ff^r_2(e_1)-\ff^r_2(e_3)\right)}$.
			Therefore, Eq. \eqref{eq: lu-2cfa-t} indicates that error in demand of $t_1$ that can be achieved can be bounded by $\tau_{d2}^f$.
			
			By symmetry, we have error in demand of $t_2$ that can be achieved is upper bounded by $\tau^f_{d1}$, i.e., $\bar{\tau}^f_{d1}\leq \tau^f_{d1}$. Thus, we can unify the error in demand for sinks and other non-fixed flow vertices. And Eq. \eqref{eq: lu-2cfa-d1} and \eqref{eq: lu-2cfa-d2} also implies
			\[\bar{\tau}^f_{d1}\leq \epsilon^f_{d1}, \qquad \bar{\tau}^f_{d2}\leq \epsilon^f_{d2}.\]
		
			To summarize, if $\ff^r$ is a solution to the \textsc{2cfra} instance with the error $\epsilon^r$ as set in the reduction, we can map it back to a solution $\ff^f$ to the \textsc{2cffa} instance with its error target achieved.
		\end{enumerate}
\end{proof}

Now, we provide a proof to Claim \ref{cl: 2cfra}.
\begin{proof}
	We divide all edges in $E^f$ into two groups: 
	\[E_I=\{e\in E^f ~s.t. ~\ff^r_1(e_4)\leq \ff^r_1(e_6)\},\]
	\[E_{II}=\{e\in E^f~ s.t.~ \ff^r_1(e_4)> \ff^r_1(e_6)\}.\]
	Then, we denote
	\[T_I=\sum_{e\in E_I}\ff^r_1(e_4), \qquad S_I=\sum_{e\in E_I}\ff^r_1(e_6);\]
	\[T_{II}=\sum_{e\in E_{II}}\ff^r_1(e_4), \qquad S_{II}=\sum_{e\in E_{II}}\ff^r_1(e_6).\]
	On the one hand, by the capacity constraints, we have
	\begin{equation}
		\label{eq: lu2cf}
		S_I+T_{II}\leq (1+\epsilon^r)\sum_{e\in E^f} \uu^f(e)=(1+\epsilon^r)M^f.
	\end{equation}
	On the other hand, applying error in requirement, we have
	\[T_I+T_{II}\geq (2M^f-\eps^r_1-)\ff^r_1(z_1,\bar{t}_1)\geq 2M^f-\eps^r_1-(1+\epsilon^r)M^f=(1-\epsilon^r)M^f-\epsilon^r_1,\]
	\[S_I+S_{II}=(2M^f-\eps^r_1)-\ff^r_1(\bar{s}_1, z_1')\geq2M^f-\eps^r_1-(1+\epsilon^r)M^f=(1-\epsilon^r)M^f-\epsilon^r_1.\]
	Thus,
	\[S_I+T_{II}=S_I+(T_I+T_{II})-T_{I}\geq (1-\epsilon^r)M^f-\epsilon^r_1+(S_I-T_{I}),\]
	\[S_I+T_{II}=(S_I+S_{II})+T_{II}-S_{II}\geq (1-\epsilon^r)M^f-\epsilon^r_1+(T_{II}-S_{II}).\]
	Together with Eq. \eqref{eq: lu2cf}, we obtain
	\[S_I-T_I\leq S_I+T_{II}+\epsilon^r_1-(1-\epsilon^r)M^f\leq (1+\epsilon^r)M^f+\epsilon^r_1-(1-\epsilon^r)M^f=2M^f\epsilon^r+\epsilon^r_1,\]
	\[T_{II}-S_{II}\leq S_I+T_{II}+\epsilon^r_1-(1-\epsilon^r)M^f\leq (1+\epsilon^r)M^f+\epsilon^r_1-(1-\epsilon^r)M^f=2M^f\epsilon^r+\epsilon^r_1.\]
	Hence, we have
	\[\sum_{e\in E^f} \abs{\ff^r_1(e_4)-\ff^r_1(e_6)}=(S_I-T_I)+(T_{II}-S_{II})\leq 4M^f\epsilon^r+2\epsilon^r_1,\]
	which finishes the proof.
\end{proof}
%\textbf{Remark:}
%
%We can investigate further in flows routed in edges that are incident to $s_i$ and $t_i$: 
%\begin{itemize}
%	\item For edges $e=(s_i,y)$, it is noted that $\ff^r_{\bar{i}}(e_1)=0, \bar{i}=\{1,2\}\backslash i$, since the incoming flow of $s_i$ only comes from $\bar{s}_i$ (refer to the second part of Figure \ref{fig: lu2cf-2cfr}). As we map back by setting $\ff^f(e)=\ff^r(e_1)$, we have 
%	\[\ff^f_{\bar{i}}(s_i,y)=0,\]
%	indicating that only flows of the $i$th commodity can be routed through edges incident to $s_i$.
%	
%	\item For edges $e=(x,t_i)$, it is noted that $\ff^r_{\bar{i}}(e_3)=0, \bar{i}=\{1,2\}\backslash i$, since the outgoing flow of $t_i$ only goes to $\bar{t}_i$ (refer to the second part of Figure \ref{fig: lu2cf-2cfr}). As we map back by setting $\ff^f(e)=\ff^r(e_1)$, we have 
%	\[\ff^f_{\bar{i}}(x,t_i)\leq \epsilon_{d\bar{i}}^f,\]
%	indicating that flows of the other commodity routed through edges incident to $t_i$ can be upper bounded by $O(M^f\epsilon^r)$.
%\end{itemize}

\subsection{2CFR(A) to 2CF(A)}
\label{sect: 2cfra-2cfa}
\subsubsection{2CFR to 2CF}
We show the reduction from a \textsc{2cfr} instance $(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2)$ to a \textsc{2cf} instance\\ $(G^{2cf}, \uu^{2cf}, \bar{\bar{s}}_1,\bar{t}_1, \bar{\bar{s}}_2, \bar{t}_2, R^{2cf})$. 
We copy the entire graph structure of $G^r$ to $G^{2cf}$. In addition, we add to $G^{2cf}$ with two new sources $\bar{\bar{s}}_1, \bar{\bar{s}}_2$ and two new edges $(\bar{\bar{s}}_1,\bar{s}_1), (\bar{\bar{s}}_2, \bar{s}_2)$ with capacity $R_1, R_2$, respectively. We set $R^{2cf}=R_1+R_2$. 

If a \textsc{2cf} solver returns $\ff^{2cf}$ for the \textsc{2cf} instance $(G^{2cf}, \uu^{2cf}, \bar{\bar{s}}_1,\bar{t}_1, \bar{\bar{s}}_2, \bar{t}_2, R^{2cf})$, then we return $\ff^r$ for the \textsc{2cfr} instance $(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2)$ by
setting $\ff_i^{r}(e)=\ff^{2cf}_i(e), \forall e\in E^r, i\in\{1,2\}$.

%To reduce a \textsc{2cfra} instance to a \textsc{2cfa} instance, besides maintaining the entire graph structure of $G^r$, we add to $G^r$ with two new sources $\bar{\bar{s}}_1, \bar{\bar{s}}_2$ and two new edges $(\bar{\bar{s}}_1,\bar{s}_1), (\bar{\bar{s}}_2, \bar{s}_2)$ with capacity $R_1, R_2$, respectively. 

\begin{lemma}[\textsc{2cfr} to \textsc{2cf}]
	\label{lm: 2cfr-2cf}
	Given a \textsc{2cfr} instance $(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2)$,
	we can construct, in time $O(|E^r|)$, a \textsc{2cf} instance $(G^{2cf}, \uu^{2cf}, \bar{\bar{s}}_1,\bar{t}_1, \bar{\bar{s}}_2, \bar{t}_2, R^{2cf})$ such that
	\[|V^{2cf}|= |V^r|+2, \qquad |E^{2cf}|=|E^r|+2, \qquad \norm{\uu^{2cf}}_{max}=\max\{R_1, R_2\}, \]
	\[R^{2cf}=R_1+R_2,\]
	and if the \textsc{2cfr} instance has a solution, then the \textsc{2cf} instance has a solution.
	%	and if $\ff^h$ is a solution to the FHF instance, then in time $O(\hat{n})$, we can compute a solution $\hat{\xx}$ to the 1-LEN instance.
\end{lemma}	
\begin{proof}
	According to the reduction described above, if there exists a solution $\ff^{r}$ to the \textsc{2cfr} instance such that $F_1^r\geq R_1, F_2^r\geq R_2$, then there also exists a solution $\ff^{2cf}$ to the \textsc{2cf} instance because $F_1^{2cf}=R_1, F_2^{2cf}=R_2$, and thus $F_1^{2cf}+F_2^{2cf}=R^{2cf}$.
	
	For the problem size after reduction, it is obvious that
	\[|V^{2cf}|=|V^r|+2, \qquad |E^{2cf}|=|E^r|+2, \qquad \norm{\uu^{2cf}}_{max}=\max\{R_1, R_2\}.\] 
	%		\item \textbf{Reduction time}\\
	For the reduction time, it takes constant time to add two new vertices and edges, and it take $O(|E^r|)$ time to copy the rest edges. Thus, the reduction of this step can be performed in $O(|E^r|)$ time.	
\end{proof}

\subsubsection{2CFRA to 2CFA}
The above lemma shows the reduction between exactly solving a \textsc{2cfr} instance and exactly solving a \textsc{2cf} instance. 
Next, we generalize the case with exact solutions to the case that allows approximate solutions.

To start with, we use the same reduction method and solution mapping method in the exact case to the approximate case.

\begin{lemma}[\textsc{2cfra} to \textsc{2cfa}]	
	Given a \textsc{2cfra} instance $(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2, \epsilon^r, \epsilon^r_1, \epsilon^r_2)$, we can construct, in time $O(|E^r|)$, a \textsc{2cfa} instance $(G^{2cf}, \uu^{2cf}, \bar{\bar{s}}_1,\bar{t}_1, \bar{\bar{s}}_2, \bar{t}_2, R^{2cf}, \epsilon^{2cf})$ such that
	\[|V^{2cf}|= |V^r|+2, \qquad |E^{2cf}|=|E^r|+2, \qquad \norm{\uu^{2cf}}_{max}=\max\{R_1, R_2\}, \]
	\[R^{2cf}=R_1+R_2,\]
	and
	\[\epsilon^{2cf}=\min\left\{\epsilon^r, \frac{\epsilon^r_1}{R_2}, \frac{\epsilon^r_2}{R_1}\right\}.\]
	If the \textsc{2cfr} instance $(G^r, \uu^r, \bar{s}_1,\bar{t}_1, \bar{s}_2, \bar{t}_2, R_1, R_2)$ has a solution, then the \textsc{2cf} instance \\$(G^{2cf}, \uu^{2cf}, \bar{\bar{s}}_1,\bar{t}_1, \bar{\bar{s}}_2, \bar{t}_2, R^{2cf})$ has a solution.
	Furthermore, if $\ff^{2cf}$ is a solution to the \textsc{2cfa} instance, then in time $O(|E^{r}|)$, we can compute a solution $\ff^r$ to the \textsc{2cfra} instance.
	
%	Given a  \textsc{2cfra} instance $(G^r, \uu^r, R_1,R_2, \epsilon^r)$, it can be reduced to a \textsc{2cfa} instance $(G^{2cf}, \uu^{2cf}, \epsilon^{2cf})$ in constant time, such that $G^{2cf}$ has $|V^{2cf}|=O(|V^r|)$ vertices and $|E^{2cf}|=O(|E^r|)$ edges.
%	If there is a  \textsc{2cfa} solver with $\epsilon^{2cf}$ error in congestion, then it can be translated into a  \textsc{2cfra} solver with $\epsilon^r$ error in congestion, where 
%	\[\epsilon^r=\epsilon^{2cf}.\]	
\end{lemma}	
\begin{proof}

%		\item \textbf{Problem size and reduction time}\\
%		According to the reduction approach described above, there are only two additional vertices $\bar{\bar{s}}_1, \bar{\bar{s}}_2$ and two additional edges $(\bar{\bar{s}}_1,\bar{s}_1), (\bar{\bar{s}}_2, \bar{s}_2)$ with capacity $R_1, R_2$ are added.
%		Therefore, we have for graph $G^{2cf}$ with
%		\[|V^{2cf}|=|V^r|+2, \qquad |E^{2cf}|=|E^r|+2, \qquad \norm{\uu^{2cf}}_{max}=\max\{R_1, R_2\}.\] 
%%		\item \textbf{Reduction time}\\
%		It takes constant time to add a constant number of vertices and edges. And it take $O(|E^r|)$ time to copy the rest edges. Thus, the reduction of this step can be performed in $O(|E^r|)$ time.
		
% 		\item \textbf{Solution mapping and error analysis}\\
% 		\ming{check}
% 		By the construction of $G^{2cf}$, its maximum flow value is $R_1, R_2$ if and only if there exists a flow with $\epsilon^r$ error in congestion in $G^r$ such that $F_1^r\geq R_1$ and $F_2^r\geq R_2$. 
% 		%As it is true if the LP at the beginning has a feasible solution, then 
% 		According to Definition \ref{def: 2cfa} and Lemma \ref{lm: 2cf_simp}, a \textsc{2cfa} solver can return a flow $\ff^{2cf}=\ff^{2cf}_1+\ff^{2cf}_2$, which satisfies:
% 		\begin{itemize}
% 			\item optimality: $F_1^{2cf}=R_1$, $F_2^{2cf}=R_2$;
% 			\item direction constraint: $\ff_1^{2cf}, \ff_2^{2cf}\geq\boldsymbol{0}$;
% 			\item capacity constraint with error in congestion: $\ff^{2cf}\leq (1+\epsilon^{2cf})\uu^{2cf}$;
% 			\item flow conservation constraint: $\sum\limits_{\begin{subarray}{c} 
% 					u\in V \\ 
% 					(u,v)\in E 
% 			\end{subarray}} \ff^{2cf}_i(u,v)=\sum\limits_{\begin{subarray}{c} 
% 					w\in V \\ 
% 					(v,w)\in E 
% 			\end{subarray}} \ff^{2cf}_i(v,w), ~\forall v\in V^{2cf}\backslash\{s_i,t_i\}, i\in\{1,2\}$.
% 		\end{itemize}
% %		\begin{align*}
% %			\BB\ff_1&=R_1\dd_1\\
% %			\BB\ff_2&=R_2\dd_2\\
% %			\ff_1+\ff_2&\leq (1+\epsilon^{2cf})\uu\\
% %			\ff_1,\ff_2&\geq\boldsymbol{0}
% %		\end{align*}
% 		Then, we can map $\ff^{2cf}$ back to $\ff^r$ by setting $\ff^{r}(e)=\ff^{2cf}(e), e\in E^r$. The two entries that correspond to the edges $(\bar{\bar{s}}_1,\bar{s}_1)$ and $(\bar{\bar{s}}_2, \bar{s}_2)$ are discarded. As there are $|E^r|$ entries to map, it takes $O(|E^{r}|)$ time to map $\ff^{2cf}$ back to $\ff^r$. Hence, the above constraints still hold for $\ff^{r}$. Thus,
% 		\[\tau^r= \epsilon^{2cf}.\]
% 		As we also set $\epsilon^{2cf}=\epsilon^r$ in the reduction, it indicates that $\tau^r=\epsilon^r$.

%\item \textbf{Solution mapping and error analysis}\\

		Since we use the same reduction method in the exact case to the approximate case, the conclusions in Lemma \ref{lm: 2cfr-2cf} also apply here, including the reduction time, problem size, and that \textsc{2cf} has a feasible solution when \textsc{2cfr} has one. 
		It remains to show the solution mapping time, as well as how the problem error changes by mapping an approximate solution to \textsc{2cfa} back to an approximate solution to \textsc{2cfra}.
		
		Based on the solution mapping method described above, it takes constant time to set the value of each of $\ff^r$, and $\ff^r$ has $|E^r|$ entries, such a solution mapping takes $O(|E^r|)$ time.	
		
		\ming{check}
		Now, we conduct error analysis.	If $\ff^{2cf}$ is a solution to the \textsc{2cfa} instance $(G^{2cf}, \uu^{2cf}, \bar{\bar{s}}_1,\bar{t}_1, \bar{\bar{s}}_2, \bar{t}_2, R^{2cf}, \epsilon^{2cf})$, then by Definition \ref{def: 2cfa} and Lemma \ref{lm: 2cf_simp}, we have
		\begin{enumerate}
			\item flow value: $F_1^{2cf} + F_2^{2cf} \geq R^{2cf}$;
			\item direction constraint: $\ff_1^{2cf}, \ff_2^{2cf}\geq\boldsymbol{0}$;
			\item capacity constraint with error in congestion: $\ff^{2cf}_1 + \ff^{2cf}_2 \leq (1+\epsilon^{2cf})\uu^{2cf}$;
			\item flow conservation constraint: $\sum\limits_{\begin{subarray}{c} 
					u\in V \\ 
					(u,v)\in E 
			\end{subarray}} \ff^{2cf}_i(u,v)=\sum\limits_{\begin{subarray}{c} 
					w\in V \\ 
					(v,w)\in E 
			\end{subarray}} \ff^{2cf}_i(v,w), ~\forall v\in V^{2cf}\backslash\{s_i,t_i\}, i\in\{1,2\}$.
		\end{enumerate}
		We observe that by the construction of $G^{2cf}$, the optimal flow values satisfy 
		$$F_1^{2cf*} \le R_1, \qquad F_2^{2cf*} \le R_2.$$ 
		Thus, we must have 
		\begin{equation}
			\label{eq: 2cfa_1}
			F_1^{2cf} + F_2^{2cf} = R^{2cf}.
		\end{equation}
		In addition, by error in congestion, we have
		\begin{equation}
			\label{eq: 2cfa_2}
			F_i^{2cf}=\ff_1^{2cf}(\bar{\bar{s}}_i, \bar{s_i}) \leq (1+\epsilon^{2cf})R_i, \qquad i \in \{1,2\}.
		\end{equation}
		Combining Eq. \eqref{eq: 2cfa_1} and \eqref{eq: 2cfa_2}, we have
		\begin{equation}
			\label{eq: 2cfa_3}
			\begin{aligned}
				R_1-R_2\epsilon^{2cf} \leq F_1^{2cf}\leq (1+\epsilon^{2cf})R_1,\\
				R_2-R_1\epsilon^{2cf}\leq F_2^{2cf}\leq (1+\epsilon^{2cf})R_2.
			\end{aligned}
		\end{equation}		
		As we map $\ff^{2cf}$ back to $\ff^r$ by setting 
		$$\ff_i^{r}(e)=\ff_i^{2cf}(e), \qquad \forall e\in E^r, i \in \{1,2\},$$ 
		we have the error in congestion that can be achieved by $\ff^r$ is 
		\[\tau^r\leq \eps^{2cf}.\]
		As we set in the reduction that $\eps^{2cf} \leq \eps^r$, then we have
		\[\tau^r\leq \eps^{r}.\]		
		In addition, by the flow conservation constraint, we have
		\[
		F_i^r =  \sum_{(\bar{s}_i, v) \in E^{r}} \ff_i^{r} (\bar{s}_i, v) =
		\sum_{(\bar{s}_i, v) \in E^{2cf}} \ff_i^{2cf} (\bar{s}_i, v) 
		=  \ff_1^{2cf}(\bar{\bar{s}}_i, \bar{s_i})=F_i^{2cf}, \qquad i \in \{1,2\}.
		\] 	
		Hence, applying Eq. \eqref{eq: 2cfa_3}, we have the error in requirement that can be achieved by $\ff^r$ is 
		 \begin{equation}
		 	\label{eq: 2cfa_4}
		 	\begin{aligned}
				R_1-\tau^r_1=\min F_1^{r}=\min F_1^{2cf}\geq R_1-R_2\epsilon^{2cf},\\
		 		R_2-\tau^r_2=\min F_2^{r}=\min F_2^{2cf}\geq R_2-R_1\epsilon^{2cf}.
		 	\end{aligned}
		 \end{equation}
	 	As we set in the reduction that $\epsilon^{2cf}\leq \min\left\{\frac{\epsilon^r_1}{R_2}, \frac{\epsilon^r_2}{R_1}\right\}$, then we have
	 	\[\tau^r_1\leq R_2\frac{\epsilon^r_1}{R_2}=\epsilon^r_1,\qquad \tau^r_2\leq R_1\frac{\epsilon^r_2}{R_1}=\epsilon^r_2.\]
		
		Thus, we can conclude that if $\ff^{2cf}$ is a solution to the \textsc{2cfa} instance with the error $\epsilon^{2cf}$ as set in the reduction, we can map it back to a solution $\ff^r$ to the \textsc{2cfra} instance with its error target achieved.
%		We observe that by the construction of $G^{2cf}$, the optimal flow values satisfy 
%		$$F_1^{2cf*} \le R_1, \qquad F_2^{2cf*} \le R_2$$ 
%		and $F_1^{2cf*} + F_1^{2cf*} = R_1 + R_2=R^{2cf}$ if and only there exists flows in $G^r$ such that $F_1^r = R_1, F_2^r = R_2$.
%
%		Let $\ff_1^{2cf}, \ff_2^{2cf}$ be a solution to the \textsc{2cfa} instance,
%		then  
%		\begin{itemize}
%			\item optimality: $F_1^{2cf} + F_2^{2cf} = R^{2cf}$;
%			\item direction constraint: $\ff_1^{2cf}, \ff_2^{2cf}\geq\boldsymbol{0}$;
%			\item capacity constraint with error in congestion: $\ff^{2cf}_1 + \ff^{2cf}_2 \leq (1+\epsilon^{2cf})\uu^{2cf}$;
%			\item flow conservation constraint: $\sum\limits_{\begin{subarray}{c} 
%					u\in V \\ 
%					(u,v)\in E 
%			\end{subarray}} \ff^{2cf}_i(u,v)=\sum\limits_{\begin{subarray}{c} 
%					w\in V \\ 
%					(v,w)\in E 
%			\end{subarray}} \ff^{2cf}_i(v,w), ~\forall v\in V^{2cf}\backslash\{s_i,t_i\}, i\in\{1,2\}$.
%		\end{itemize}
%		As we map $\ff_1^{2cf}, \ff_2^{2cf}$ back to $\ff_1^r, \ff_2^r$ by setting 
%		$$\ff_i^{r}(e)=\ff_i^{2cf}(e), \forall e\in E^r, i \in \{1,2\}.$$ 
%		% The two entries that correspond to the edges $(\bar{\bar{s}}_1,\bar{s}_1)$ and $(\bar{\bar{s}}_2, \bar{s}_2)$ are discarded. 
%%		As there are $|E^r|$ entries to map, it takes $O(|E^{r}|)$ time to map $\ff^{2cf}$ back to $\ff^r$. 
%		The error in congestion for $\ff^r$ is at most $\eps^{2cf} = \eps^r$.
%		
%		In addition, by the conservation of flows, for each $i \in \{1,2\}$,
%		\[
%	 F_i^r =  \sum_{(\bar{s}_i, v) \in E^{r}} \ff_i^{r} (\bar{s}_i, v) =
%	  \sum_{(\bar{s}_i, v) \in E^{2cf}} \ff_i^{2cf} (\bar{s}_i, v) 
%	 =  \ff_1^{2cf}(\bar{\bar{s}}_i, \bar{s_i}) = F_i^{2cf}
%		\] 
%		
%		If there is a solution to the instance 2CFRA $(G^r, \uu^{r}, R_1, R_2, \eps^r)$, 
%		then there exists a solution to 2CFA $(G^{2cf}, \uu^{2cf}, \eps^{2cf})$ such that 
%		the sum of the two flow value is no less than $R_1 + R_2$. $F_i^{2cf} \ge R_i$ for each $i \in \{1,2\}$
%		and thus $\ff_1^r, \ff_2^r$ form a solution to $(G^r, \uu^{r}, R_1, R_2, \eps^r)$.
%		\peng{the proof is incomplete}

		% Hence, the above constraints still hold for $\ff^{r}$. Thus,
		% \[\tau^r= \epsilon^{2cf}.\]
		% As we also set $\epsilon^{2cf}=\epsilon^r$ in the reduction, it indicates that $\tau^r=\epsilon^r$.

\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
